Multitask Prompted Training Enables Zero-Shot Task Generalization

Large language models have recently been shown to attain reasonable zero-shot generalization on a diverse set of tasks (Brown et al., 2020). It has been hypothesized that this is a consequence of implicit multitask learning in language models' pretraining (Radford et al., 2019). Can zero-shot generalization instead be directly induced by explicit multitask learning? To test this question at scale, we develop a system for easily mapping any natural language tasks into a human-readable prompted form. We convert a large set of supervised datasets, each with multiple prompts with diverse wording. These prompted datasets allow for benchmarking the ability of a model to perform completely held-out tasks. We fine-tune a pretrained encoder-decoder model (Raffel et al., 2020; Lester et al., 2021) on this multitask mixture covering a wide variety of tasks. The model attains strong zero-shot performance on several standard datasets, often outperforming models up to 16x its size. Further, our approach attains strong performance on a subset of tasks from the BIG-bench benchmark, outperforming models up to 6x its size. All trained models are available at https://github.com/bigscience-workshop/t-zero and all prompts are available at https://github.com/bigscience-workshop/promptsource.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> promptgen.tex <==
\subsection{Coreference }
\subsubsection{super\_glue wsc.fixed}
\noindent Dataset from \citet{levesque2012winograd}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 idx & \verb+ 0 + \\
	 label & \verb+ 0 + \\
	 span1\_index & \verb+ 0 + \\
	 span1\_text & \verb+ Mark + \\
	 span2\_index & \verb+ 13 + \\
	 span2\_text & \verb+ He + \\
	 text & \verb+ Mark told Pete many lies about himself, which Pete... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ text }} In the previous sentence, does the pronoun "{{ span2_text.lower() }}" refer to {{ span1_text }}? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ text }} Here, by "{{ span2_text }}" they mean "{{ span1_text }}". Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ text }} 

In other words, {{ text.split(" ")[span2_index:] | join(" ") | replace(span2_text, span1_text) }} True or false?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ text }} I think they mean "{{ text.split(" ")[span2_index:] | join(" ") | replace(span2_text, span1_text) }}" Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ text }} Here, does "{{ span2_text.lower() }}" stand for {{ span1_text }}? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Passage: {{ text }} 

Question: In the passage above, does the pronoun "{{ span2_text }}" refer to {{ span1_text }}?

Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ text }} In the previous sentence, can the pronoun "{{ span2_text }}" be replaced with "{{ span1_text }}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Context: {{ text }} 

{% if span2_text.lower()  == "they" or span2_text.lower() == "them" %}
Question: "{{ span2_text }}" are {{ span1_text }}. True or false?
{% else %}
Question: "{{ span2_text }}" is {{ span1_text }}. True or false?
{% endif %}

Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ text }} 
In the passage above, the pronoun "{{ span2_text }}" refers to {{ span1_text }}. True or false?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ text }} 
{% if span2_text.lower()  == "they" or span2_text.lower() == "them" %}
Question: Who are "{{ span2_text.lower() }}"? {{ span1_text }}?
{% else %}
Question: Who is "{{ span2_text.lower() }}"? Is it {{ span1_text }}?
{% endif %}
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{winograd\_wsc wsc273}
\noindent Dataset from \citet{levesque2012winograd}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 label & \verb+ 0 + \\
	 options & \verb+ ['The city councilmen', 'The demonstrators'] + \\
	 pronoun & \verb+ they + \\
	 pronoun\_loc & \verb+ 63 + \\
	 quote & \verb+ they feared violence + \\
	 quote\_loc & \verb+ 63 + \\
	 source & \verb+ (Winograd 1972) + \\
	 text & \verb+ The city councilmen refused the demonstrators a pe... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Identify the pronoun in "{{text}}"
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{pronoun}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Identify the pronoun in "{{text}}" and the entity it is referring to
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
"{{pronoun}}" which refers to the "{{options[label]}}"
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Who does the pronoun "{{pronoun}}" in "{{text}}" refer to?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{options[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Who does the pronoun "{{pronoun}}" in "{{text}}" refer to?

The options are {{options | join(" and ")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{options[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Identify the phrase in "{{text}}" in which the key action or context surrounding the pronoun is described
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{quote}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{winogrande winogrande\_xl}
\noindent Dataset from \citet{ai2:winogrande}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ 2 + \\
	 option1 & \verb+ Ian + \\
	 option2 & \verb+ Dennis + \\
	 sentence & \verb+ Ian volunteered to eat Dennis's menudo after alrea... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ option1 }} ||| {{ option2 }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ sentence }} In the previous sentence, does _ refer to {{ option1 }} or  {{ option2 }}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer == '1' %} {{option1}} {% else %} {{ option2 }} {% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{option1}} ||| {{option2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
In the sentence below, does the _ stand for {{answer_choices[0]}} or {{answer_choices[1]}}?
{{sentence}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer | int - 1]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{option1}} ||| {{option2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{sentence}}
What does the _ in the above sentence refer to? {{ option1 }} or {{ option2 }}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer == '1' %} {{option1}} {% else %} {{ option2 }} {% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{option1}} ||| {{option2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Fill in the _ in the below sentence:
{{sentence}}

Choices:
- {{ option1 }}
- {{ option2 }}

Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer == '1' %} {{option1}} {% else %} {{ option2 }} {% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
The _ in the sentence below refers to {{option1}}. True or False?
{{sentence}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer|int - 1]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{option1}} ||| {{option2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{sentence}}
Replace the _ in the above sentence with the correct option: 
- {{option1}}
- {{option2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer == '1' %} {{option1}} {% else %} {{ option2 }} {% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{winogrande winogrande\_debiased}
\noindent Dataset from \citet{ai2:winogrande}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ 1 + \\
	 option1 & \verb+ garage + \\
	 option2 & \verb+ backyard + \\
	 sentence & \verb+ John moved the couch from the garage to the backya... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{option1}} ||| {{option2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{sentence}}
Replace the _ in the above sentence with the correct option: 
- {{option1}}
- {{option2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer == '1' %} {{option1}} {% else %} {{ option2 }} {% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{option1}} ||| {{option2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{sentence}}
What does the _ in the above sentence refer to? {{ option1 }} or {{ option2 }}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer == '1' %} {{option1}} {% else %} {{ option2 }} {% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ option1 }} ||| {{ option2 }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ sentence }} In the previous sentence, does _ refer to {{ option1 }} or  {{ option2 }}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer == '1' %} {{option1}} {% else %} {{ option2 }} {% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{option1}} ||| {{option2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
In the sentence below, does the _ stand for {{answer_choices[0]}} or {{answer_choices[1]}}?
{{sentence}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer | int - 1]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
The _ in the sentence below refers to {{option1}}. True or False?
{{sentence}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer|int - 1]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{option1}} ||| {{option2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Fill in the _ in the below sentence:
{{sentence}}

Choices:
- {{ option1 }}
- {{ option2 }}

Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer == '1' %} {{option1}} {% else %} {{ option2 }} {% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Grammatical Acceptability }
\subsubsection{glue cola}
\noindent Dataset from \citet{warstadt2018neural}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 idx & \verb+ 0 + \\
	 label & \verb+ 1 + \\
	 sentence & \verb+ Our friends won't buy this analysis, let alone the... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Does the following sentence make sense and use correct English? Please answer {{"yes"}} or {{"no"}}.
{{sentence}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{sentence}}
Is this example grammatically correct and sensible?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I'm copy-editing a story for publication. It has the following sentence in it:
{{sentence}}
Does this sentence make sense and is it grammatically correct? Please answer {{"yes or no"}}.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
The following sentence is either "{{"acceptable"}}", meaning it is grammatically correct and makes sense, or "{{"unacceptable"}}". Which is it?
{{sentence}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{sentence}}
I'm worried that sentence didn't make any sense, or was grammatically incorrect. Was it correct?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{NLI }
\subsubsection{super\_glue cb}
\noindent Dataset from \citet{de:marneff_simons_tonhauser_2019}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 hypothesis & \verb+ the language was peeled down + \\
	 idx & \verb+ 0 + \\
	 label & \verb+ 0 + \\
	 premise & \verb+ It was a complex language. Not written down but ha... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Suppose {{premise}} Can we infer that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} Based on the previous passage, is it true that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} Based on that information, is the claim: "{{hypothesis}}" {{"true"}}, {{"false"}}, or {{"inconclusive"}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given that {{premise}} Does it follow that {{hypothesis}} Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} Are we justified in saying that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Suppose it's true that {{premise}} Then, is "{{hypothesis}}" {{"always"}}, {{"sometimes"}}, or {{"never"}} true?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}}
Question: {{hypothesis}} True, False, or Neither?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} 

Keeping in mind the above text, consider: {{hypothesis}} Is this {{"always"}}, {{"sometimes"}}, or {{"never"}} correct?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given {{premise}} Is it guaranteed true that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given that {{premise}} Therefore, it must be true that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Assume it is true that {{premise}} 

Therefore, "{{hypothesis}}" is {{"guaranteed"}}, {{"possible"}}, or {{"impossible"}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} 

Question: Does this imply that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{N18-1101}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} Using only the above description and what you know about the world, "{{hypothesis}}" is definitely correct, incorrect, or inconclusive?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given {{premise}} Should we assume that "{{hypothesis}}" is true? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Take the following as truth: {{premise}}
Then the following statement: "{{hypothesis}}" is {{"true"}}, {{"false"}}, or {{"inconclusive"}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{super\_glue rte}
\noindent Dataset from \citet{dagan2005pascal}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 hypothesis & \verb+ Weapons of Mass Destruction Found in Iraq. + \\
	 idx & \verb+ 0 + \\
	 label & \verb+ 1 + \\
	 premise & \verb+ No Weapons of Mass Destruction Found in Iraq Yet. + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt from \cite{N18-1101}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} Using only the above description and what you know about the world, is "{{hypothesis}}" definitely correct? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given {{premise}} Is it guaranteed true that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Suppose {{premise}} Can we infer that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}}
Question: {{hypothesis}} True or False?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} 

Question: Does this imply that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given {{premise}} Should we assume that "{{hypothesis}}" is true? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given that {{premise}} Does it follow that {{hypothesis}} Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} Based on the previous passage, is it true that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} Are we justified in saying that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given that {{premise}} Therefore, it must be true that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{anli}
\noindent Dataset from \citet{nie2019adversarial}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 hypothesis & \verb+ The trolleybus system has over 2 urban routes + \\
	 label & \verb+ 0 + \\
	 premise & \verb+ The Parma trolleybus system (Italian: "Rete filovi... + \\
	 reason & \verb+  + \\
	 uid & \verb+ 0fd0abfb-659e-4453-b196-c3a64d2d8267 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt from \cite{N18-1101}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} Using only the above description and what you know about the world, "{{hypothesis}}" is definitely correct, incorrect, or inconclusive?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given {{premise}} Should we assume that "{{hypothesis}}" is true? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given that {{premise}} Does it follow that {{hypothesis}} Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}}
Question: {{hypothesis}} True, False, or Neither?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} Based on the previous passage, is it true that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} Are we justified in saying that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Take the following as truth: {{premise}}
Then the following statement: "{{hypothesis}}" is {{"true"}}, {{"false"}}, or {{"inconclusive"}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given that {{premise}} Therefore, it must be true that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Suppose {{premise}} Can we infer that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Assume it is true that {{premise}} 

Therefore, "{{hypothesis}}" is {{"guaranteed"}}, {{"possible"}}, or {{"impossible"}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Suppose it's true that {{premise}} Then, is "{{hypothesis}}" {{"always"}}, {{"sometimes"}}, or {{"never"}} true?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} 

Question: Does this imply that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} 

Keeping in mind the above text, consider: {{hypothesis}} Is this {{"always"}}, {{"sometimes"}}, or {{"never"}} correct?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} Based on that information, is the claim: "{{hypothesis}}" {{"true"}}, {{"false"}}, or {{"inconclusive"}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given {{premise}} Is it guaranteed true that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{hans}
\noindent Dataset from \citet{DBLP:journals/corr/abs-1902-01007}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 binary\_parse\_hypothesis & \verb+ ( ( The scientist ) ( ( supported ( the doctors ) ... + \\
	 binary\_parse\_premise & \verb+ ( ( The doctors ) ( ( supported ( the scientist ) ... + \\
	 heuristic & \verb+ lexical_overlap + \\
	 hypothesis & \verb+ The scientist supported the doctors . + \\
	 label & \verb+ 1 + \\
	 parse\_hypothesis & \verb+ (ROOT (S (NP (DT The) (NN scientist)) (VP (VBD sup... + \\
	 parse\_premise & \verb+ (ROOT (S (NP (DT The) (NNS doctors)) (VP (VBD supp... + \\
	 premise & \verb+ The doctors supported the scientist . + \\
	 subcase & \verb+ ln_subject/object_swap + \\
	 template & \verb+ temp1 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} 

Question: Does this imply that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given {{premise}} Should we assume that "{{hypothesis}}" is true? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} Based on the previous passage, is it true that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given that {{premise}} Does it follow that {{hypothesis}} Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given {{premise}} Is it guaranteed true that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given that {{premise}} Therefore, it must be true that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{N18-1101}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} Using only the above description and what you know about the world, is "{{hypothesis}}" definitely correct? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}} Are we justified in saying that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{premise}}
Question: {{hypothesis}} True or False?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Suppose {{premise}} Can we infer that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Paraphrase }
\subsubsection{glue mrpc}
\noindent Dataset from \citet{dolan2005automatically}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 idx & \verb+ 0 + \\
	 label & \verb+ 1 + \\
	 sentence1 & \verb+ Amrozi accused his brother , whom he called " the ... + \\
	 sentence2 & \verb+ Referring to him as only " the witness " , Amrozi ... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label == 1 %}
Paraphrase the following sentence: {{sentence1}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{sentence2}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I want to know whether the following two sentences mean the same thing.
{{sentence1}}
{{sentence2}}
Do they?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Does the sentence
{{sentence1}}
paraphrase (that is, mean the same thing as) this sentence?
{{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Are the following two sentences "{{"equivalent"}}" or "{{"not equivalent"}}"?
{{sentence1}}
{{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label == 1 %}
Generate a sentence that means the same thing as this one: {{sentence1}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{sentence2}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Can I replace the sentence
{{sentence1}}
with the sentence
{{sentence2}}
and have it mean the same thing?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Do the following two sentences mean the same thing?
{{sentence1}}
{{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{glue qqp}
\noindent Dataset from \citet{WinNT}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 idx & \verb+ 0 + \\
	 label & \verb+ 0 + \\
	 question1 & \verb+ How is the life of a math student? Could you descr... + \\
	 question2 & \verb+ Which level of prepration is enough for the exam j... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I'm an administrator on the website Quora. There are two posts, one that asks "{{question1}}" and another that asks "{{question2}}". I can merge questions if they are asking the same thing. Can I merge these two questions?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{question1}}
{{question2}}
Pick one: These questions are "{{"duplicates"}}" or "{{"not duplicates"}}".
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Are the questions "{{question1}}" and "{{question2}}" asking the same thing?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Can an answer to "{{question1}}" also be used to answer "{{question2}}"?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Question 1: {{question1}}
Question 2: {{question2}}

Do these two questions convey the same meaning? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I received the questions "{{question1}}" and "{{question2}}". Are they duplicates?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{paws labeled\_final}
\noindent Dataset from \citet{paws2019naacl}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ 1 + \\
	 label & \verb+ 0 + \\
	 sentence1 & \verb+ In Paris , in October 1560 , he secretly met the E... + \\
	 sentence2 & \verb+ In October 1560 , he secretly met with the English... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Determine if the following two sentences paraphrase each other or not.
Sent 1: {{sentence1}}
Sent 2: {{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}
Question: Do Sentence 1 and Sentence 2 express the same meaning? Yes or No?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{sentence1}}
Is that a paraphrase of the following sentence?
{{sentence2}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}
Question: Can we rewrite Sentence 1 to Sentence 2?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{sentence1}}
Is that a paraphrase of the following sentence?
{{sentence2}}?
Yes or No.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}
Question: Does Sentence 1 paraphrase Sentence 2? Yes or No?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label == 1 %} 
Paraphrase the sentence: {{sentence1}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{sentence2}} 
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}
Question: Does Sentence 1 paraphrase Sentence 2?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}
Question: Do Sentence 1 and Sentence 2 express the same meaning?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{sentence1}} Question: {{sentence2}} True or False?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}
Question: Can we rewrite Sentence 1 to Sentence 2? Yes or No?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{sentence1}} Question: {{sentence2}} Paraphrase or not?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{QA Closed Book }
\subsubsection{ai2\_arc ARC-Challenge}
\noindent Dataset from \citet{allenai:arc}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answerKey & \verb+ A + \\
	 choices & \verb+ {'label': ['A', 'B', 'C', 'D'], 'text': ['dry palm... + \\
	 id & \verb+ Mercury_SC_415702 + \\
	 question & \verb+ George wants to warm his hands quickly by rubbing ... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Pick and copy all the incorrect options for the following question:

{{question}}

Options:
- {{choices["text"] | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for i in range(choices["label"]|length) %}
{% if i != choices["label"].index(answerKey) %}
- {{choices["text"][i]}}
{% endif %}
{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Here's a problem to solve: {{question}}

Among the 4 following options, which is the correct answer?
{% for letter, t in zip(answer_choices, choices.text) %}
- {{letter}}: {{t}}
 {% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answerKey}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{question}}

Options:
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices["label"].index(answerKey)]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I am hesitating between 4 options to answer the following question, which option should I choose?
Question: {{question}}
Possibilities:
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices["label"].index(answerKey)]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I gave my students this multiple choice question: {{question}}

Only one answer is correct among these 4 choices:
- {{answer_choices | join("\n- ")}}

Could you tell me which one is correct?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices["label"].index(answerKey)]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Pick the most correct option to answer the following question.

{{question}}

Options:
{% for letter, t in zip(answer_choices, choices.text) %}
- {{letter}}: {{t}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answerKey}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{ai2\_arc ARC-Easy}
\noindent Dataset from \citet{allenai:arc}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answerKey & \verb+ B + \\
	 choices & \verb+ {'label': ['A', 'B', 'C', 'D'], 'text': ['a leg mu... + \\
	 id & \verb+ Mercury_7220990 + \\
	 question & \verb+ Which factor will most likely cause a person to de... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Pick the most correct option to answer the following question.

{{question}}

Options:
{% for letter, t in zip(answer_choices, choices.text) %}
- {{letter}}: {{t}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answerKey}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{question}}

Options:
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices["label"].index(answerKey)]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I am hesitating between 4 options to answer the following question, which option should I choose?
Question: {{question}}
Possibilities:
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices["label"].index(answerKey)]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I gave my students this multiple choice question: {{question}}

Only one answer is correct among these 4 choices:
- {{answer_choices | join("\n- ")}}

Could you tell me which one is correct?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices["label"].index(answerKey)]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Pick and copy all the incorrect options for the following question:

{{question}}

Options:
- {{choices["text"] | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for i in range(choices["label"]|length) %}
{% if i != choices["label"].index(answerKey) %}
- {{choices["text"][i]}}
{% endif %}
{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Here's a problem to solve: {{question}}

Among the 4 following options, which is the correct answer?
{% for letter, t in zip(answer_choices, choices.text) %}
- {{letter}}: {{t}}
 {% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answerKey}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{kilt\_tasks nq}
\noindent Dataset from \citet{kilt_tasks}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ 5328212470870865242 + \\
	 input & \verb+ how i.met your mother who is the mother + \\
	 meta & \verb+ {'left_context': '', 'mention': '', 'right_context... + \\
	 output & \verb+ [{'answer': 'Tracy McConnell', 'meta': {'score': -... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if output %}
The goal is to predict an English answer string for an input English question. All questions can be answered using the contents of English Wikipedia.
Question: {{input}}
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output|selectattr("answer")|map(attribute='answer')|reject("equalto", "")|list|choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if output %}
Search query: {{input}}
Response:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output|selectattr("answer")|map(attribute='answer')|reject("equalto", "")|list|choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if output %}
Question : {{input}}
Answer :
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output|selectattr("answer")|map(attribute='answer')|reject("equalto", "")|list|join(', ') }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if output %}
Guess a question that has the answer "{{output|selectattr("answer")|map(attribute='answer')|reject("equalto", "")|list|choice }}"
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{input}}?
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if output %}
Question : {{input}}
Answer :
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output|selectattr("answer")|map(attribute='answer')|reject("equalto", "")|list|choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if output %}
I've always wondered: {{input}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output|selectattr("answer")|map(attribute='answer')|reject("equalto", "")|list|choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if output %}
Answer the following question.
{{input}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output|selectattr("answer")|map(attribute='answer')|reject("equalto", "")|list|choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{kilt\_tasks hotpotqa}
\noindent Dataset from \citet{kilt_tasks}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ 5a7a06935542990198eaf050 + \\
	 input & \verb+ Which magazine was started first Arthur's Magazine... + \\
	 meta & \verb+ {'left_context': '', 'mention': '', 'right_context... + \\
	 output & \verb+ [{'answer': "Arthur's Magazine", 'meta': {'score':... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if output %}
Here's a complex question that requires someone to reason about the input, can you answer it?
{{input}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output | map(attribute="answer") | list | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if output %}
Combine facts and answer this: {{input}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output | map(attribute="answer") | list | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if output %}
Formulate an answer to this elaborate question: {{input}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output | map(attribute="answer") | list | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if output %}
FINAL EXAM

Question 1. {{input}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output | map(attribute="answer") | list | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if output %}
{{input}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output | map(attribute="answer") | list | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{trivia\_qa rc}
\noindent Dataset from \citet{2017arXivtriviaqa}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ {'aliases': ['(Harry) Sinclair Lewis', 'Harry Sinc... + \\
	 entity\_pages & \verb+ {'doc_source': [], 'filename': [], 'title': [], 'w... + \\
	 question & \verb+ Which American-born Sinclair won the Nobel Prize f... + \\
	 question\_id & \verb+ tc_1 + \\
	 question\_source & \verb+ http://www.triviacountry.com/ + \\
	 search\_results & \verb+ {'description': ['The Nobel Prize in Literature 19... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answer.aliases %} 
    Guess a question that has the answer "{{answer.aliases|choice}}"
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}} 
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answer.aliases %} 
    The goal is to predict an English answer string for an input English question. 
    Question : {{question}}
    Answer :
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer.aliases|choice}} 
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answer.aliases %} 
    Answer the following question.
    {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer.aliases|choice}} 
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answer.aliases %} 
   I've always wondered: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer.aliases|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answer.aliases %} 
    Question : {{question}}
    Answer :
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer.aliases|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{web\_questions}
\noindent Dataset from \citet{berant-etal-2013-semantic}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ ['Jazmyn Bieber', 'Jaxon Bieber'] + \\
	 question & \verb+ what is the name of justin bieber brother? + \\
	 url & \verb+ http://www.freebase.com/view/en/justin_bieber + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Give me the correct facts to answer this: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Give me a possible correct answer to the question "{{ question }}"
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers | choice }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
What's the answer to that question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Short general knowledge question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ question|capitalize }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers | choice }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{wiki\_qa}
\noindent Dataset from \citet{YangYihMeek:EMNLP2015:WikiQA}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ African immigration to the United States refers to... + \\
	 document\_title & \verb+ African immigration to the United States + \\
	 label & \verb+ 0 + \\
	 question & \verb+ HOW AFRICAN AMERICANS WERE IMMIGRATED TO THE US + \\
	 question\_id & \verb+ Q0 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Question: {{question}}?
Would "{{answer}}" be a reasonable answer?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I am verifying the answers generated by an automatic system to the following question: {{question}}
Suggested answer: {{answer}}
Should I validate this answer?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label == 1 %}
What is the question to: "{{answer}}"? The topic is {{document_title}}.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
"{{question}}?"
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label == 1 %}
Determine the topic of the question-answer pair.
Question: "{{question}}?";  Answer: "{{answer}}"? Topic:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{document_title}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label == 1 %}
Generate a question about the topic "{{document_title}}" whose answer would be: {{answer}}.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}?
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Question: {{question}}
I found the following answer on Google: {{answer}}
Is that a correct answer? Yes or no.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label == 1 %}
Determine the topic of the question.
Question: "{{question}}?"
Topic:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{document_title}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
False ||| True
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
The exercise is to decide whether the question accepts the proposed suggestion as a correct answer. If yes, write "{{answer_choices[1]}}", otherwise write "{{answer_choices[0]}}".
Question: {{question}}
Suggestion: {{answer}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
This is a correct answer to the following question about {{document_title}}. Yes or no?
Answer: {{answer}}
Question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label == 1 %}
Determine the topic of the passage.
"{{answer}}"
Topic:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{document_title}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label == 1 %}
Answer this question: {{question}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{QA Extractive }
\subsubsection{adversarial\_qa dbidaf}
\noindent Dataset from \citet{bartolo2020beat}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ 821607441c173838196c4d1500c2ab21a044e6b0 + \\
	 title & \verb+ Yale_University + \\
	 context & \verb+ Slack (2003) compares three groups that conducted ... + \\
	 question & \verb+ what year were the research groups compared + \\
	 answers & \verb+ {'text': ['2003'], 'answer_start': [7]} + \\
	 metadata & \verb+ {'split': 'train', 'model_in_the_loop': 'BiDAF'} + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if metadata.split != "test" %}
Extract the answer to the question from the following context.
Question: {{question}}
Context: {{context}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if metadata.split != "test" %}
Given the following passage

"{{context}}",

answer the following question. Note that the answer is present within the text.

Question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I want to test the ability of students to read a passage and answer questions about it. Could you please come up with a good question for the passage "{{context}}"?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if metadata.split != "test" %}
I know that the answer to the question "{{question}}" is in "{{context}}". Can you tell me what it is?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if metadata.split != "test" %}
Question: "{{question}}"

Context: "{{context}}"

Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{adversarial\_qa dbert}
\noindent Dataset from \citet{bartolo2020beat}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ dab017ed8a1c27c6afa2d8618abc3a477a4edffc + \\
	 title & \verb+ Empiricism + \\
	 context & \verb+ A generation later, the Irish Anglican bishop, Geo... + \\
	 question & \verb+ what concept is mentioned last? + \\
	 answers & \verb+ {'text': ['subjective idealism'], 'answer_start': ... + \\
	 metadata & \verb+ {'split': 'train', 'model_in_the_loop': 'BERT-Larg... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I want to test the ability of students to read a passage and answer questions about it. Could you please come up with a good question for the passage "{{context}}"?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if metadata.split != "test" %}
I know that the answer to the question "{{question}}" is in "{{context}}". Can you tell me what it is?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if metadata.split != "test" %}
Question: "{{question}}"

Context: "{{context}}"

Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if metadata.split != "test" %}
Extract the answer to the question from the following context.
Question: {{question}}
Context: {{context}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if metadata.split != "test" %}
Given the following passage

"{{context}}",

answer the following question. Note that the answer is present within the text.

Question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{adversarial\_qa droberta}
\noindent Dataset from \citet{bartolo2020beat}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ 12cf36866b656dc4f254081fe6796ea1be2f6d43 + \\
	 title & \verb+ Napoleon + \\
	 context & \verb+ When he became First Consul and later Emperor, Nap... + \\
	 question & \verb+ What jewelry like accessories did he wear? + \\
	 answers & \verb+ {'text': ["Légion d'honneur star, medal and ribbon... + \\
	 metadata & \verb+ {'split': 'train', 'model_in_the_loop': 'RoBERTa-L... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I want to test the ability of students to read a passage and answer questions about it. Could you please come up with a good question for the passage "{{context}}"?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if metadata.split != "test" %}
I know that the answer to the question "{{question}}" is in "{{context}}". Can you tell me what it is?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if metadata.split != "test" %}
Question: "{{question}}"

Context: "{{context}}"

Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if metadata.split != "test" %}
Extract the answer to the question from the following context.
Question: {{question}}
Context: {{context}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if metadata.split != "test" %}
Given the following passage

"{{context}}",

answer the following question. Note that the answer is present within the text.

Question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{coqa}
\noindent Dataset from \citet{SivaAndAl:Coca}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ {'answer_end': [179, 494, 511, 545, 879, 1127, 112... + \\
	 questions & \verb+ ['When was the Vat formally opened?', 'what is the... + \\
	 source & \verb+ wikipedia + \\
	 story & \verb+ The Vatican Apostolic Library (), more commonly ca... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Answer the question based on the information contained in the passage.
Q: {{questions[0]}} 

Passage: {{story}}

A:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers["input_text"][0]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Answer the last question based on the hint.
{% for question, answer in zip(questions[:-1], answers["input_text"][:-1]) %}
Q: {{question}}

A:{{answer}}
{%endfor %}

Q: {{questions[-1]}}

Hint: {{story}}

A:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers["input_text"][-1]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Can you form a set of {{questions | length}} question-answer pairs about the passage below?

Passage: {{story}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for question, answer in zip(questions, answers["input_text"]) %}
Q: {{question}}

A: {{answer}}

{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
In the passage below, extract the part which answers the question:

Q: {{questions[0]}}
Passage: {{story}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{story[answers["answer_start"][0] : answers["answer_end"][0] ]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set missing_idx = range(questions|length)|choice %}

{% for i in range(questions|length) %}
Q: {{questions[i] }}

A:  {% if i !=missing_idx %}
{{answers["input_text"][i]}}
{%endif%}
{%endfor%}

Given the above conversation, give a suitable response to the missing answer

Hint: {{story}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers["input_text"][missing_idx]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{duorc SelfRC}
\noindent Dataset from \citet{DuoRC}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ ['They arrived by train.'] + \\
	 no\_answer & \verb+ False + \\
	 plot & \verb+ 200 years in the future, Mars has been colonized b... + \\
	 plot\_id & \verb+ /m/03vyhn + \\
	 question & \verb+ How did the police arrive at the Mars mining camp? + \\
	 question\_id & \verb+ b440de7d-9c3f-841c-eaec-a14bdff950d1 + \\
	 title & \verb+ Ghosts of Mars + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if no_answer == false%}
Generate a question that has the following answer: 
{{answers|choice}} 
for the following movie plot: 
{{plot}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I am a movie director and I just received the following movie plot. Could you help me answer this question? If not, let me know by writing "{{"Not answerable"}}".

Plot title: {{title}}
Movie plot: {{plot}}
My question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
Not answerable
{% else %}
{{answers|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Extract the answer to the following question from the movie plot. If the question isn't answerable, please output "{{"Can't answer"}}".
Question: {{question}}
Title: {{title}}
Movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
Can't answer
{% else %}
{{answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Generate a question about the following movie plot: {{ plot }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ question }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Please answer the following question about this movie plot. If it's un-answerable, please output "{{"No answer"}}".

Question: {{question}}
Movie plot title: {{title}}
Movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
No answer
{% else %}
{{answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if no_answer == false%}
Build a movie plot around this: {{ question }} {{answers|choice}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ plot }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Question: {{question}}
If there is no answer, please output "{{"Insufficient information to provide an answer."}}".
Movie title: {{title}}
Context: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
Insufficient information to provide an answer.
{% else %}
{{answers|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Suggest a movie title for the following movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{title}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I am trying to decide whether it's worth it to invest in this film proposal. Can you help me answer a few questions? If you can't, please say "{{"No I can't"}}".

Question: {{question}}
Movie title: {{title}}
Movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
No I can't
{% else %}
{{answers|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{duorc ParaphraseRC}
\noindent Dataset from \citet{DuoRC}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ ['second in command Sergeant  Jericho and prisoner... + \\
	 no\_answer & \verb+ False + \\
	 plot & \verb+ Set in the second half of the 22nd century, Mars h... + \\
	 plot\_id & \verb+ /m/03vyhn + \\
	 question & \verb+ who is there with Melanie Ballard? + \\
	 question\_id & \verb+ 28ded42d-f6d5-aac6-cf6f-9e6e0820c5aa + \\
	 title & \verb+ Ghosts of Mars + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if no_answer == false%}
Build a movie plot around this: {{ question }} {{answers|choice}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ plot }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I am trying to decide whether it's worth it to invest in this film proposal. Can you help me answer a few questions? If you can't, please say "{{"No I can't"}}".

Question: {{question}}
Movie title: {{title}}
Movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
No I can't
{% else %}
{{answers|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Question: {{question}}
If there is no answer, please output "{{"Insufficient information to provide an answer."}}".
Movie title: {{title}}
Context: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
Insufficient information to provide an answer.
{% else %}
{{answers|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I am a movie director and I just received the following movie plot. Could you help me answer this question? If not, let me know by writing "{{"Not answerable"}}".

Plot title: {{title}}
Movie plot: {{plot}}
My question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
Not answerable
{% else %}
{{answers|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Generate a question about the following movie plot: {{ plot }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ question }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Extract the answer to the following question from the movie plot. If the question isn't answerable, please output "{{"Can't answer"}}".
Question: {{question}}
Title: {{title}}
Movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
Can't answer
{% else %}
{{answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Suggest a movie title for the following movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{title}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Please answer the following question about this movie plot. If it's un-answerable, please output "{{"No answer"}}".

Question: {{question}}
Movie plot title: {{title}}
Movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
No answer
{% else %}
{{answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if no_answer == false%}
Generate a question that has the following answer: 
{{answers|choice}} 
for the following movie plot: 
{{plot}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{ropes}
\noindent Dataset from \citet{Lin2019ReasoningOP}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ {'text': ['cup B']} + \\
	 background & \verb+ Passive transport occurs when a substance passes t... + \\
	 id & \verb+ 1971664873 + \\
	 question & \verb+ Which cup has a higher concentration of sugar? + \\
	 situation & \verb+ A man put two cups, cup A and cup B, filled with e... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text %}
Please answer correctly the following question related to the paragraph below. 

{{ question }}

{{ situation }}

Hint: {{ background }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text %}
{{ situation }}

Given the paragraph above, please answer correctly the following question: 

{{ question }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text %}
Background: {{ background }}

Paragraph: {{ situation }}

Given the paragraph above, please answer correctly the following question: {{ question }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text %}
Given the background: {{background}}

and the situation: {{situation}}

Answer the following question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text %}
{{ situation }}

{{ question }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text %}
{{ situation }}

{{ question }}

Hint: {{ background }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text %}
{{ background }}

{{ situation }}

{{ question }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text %}
I can use this background: {{background}}

Now, I have a new situation: {{situation}}

Answer this question please: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text %}
You are given a new situation: {{situation}}

and a hint : {{background}}

Please answer this question : {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text %}
I have a new situation: {{situation}}

But I can use this background: {{background}}

What is an answer for this question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text %}
{{ situation }}

Given the paragraph above, please answer correctly the following question: 

{{ question }}

Hint: {{ background }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text %}
I read this background article the other day: {{background}}

I am facing a new situation today: {{situation}}

Using the knowledge I acquired from the background article, how should I answer correctly the following question regarding my new situation: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{squad\_v2}
\noindent Dataset from \citet{2016arXiv160605250R}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ 56be85543aeaaa14008c9063 + \\
	 title & \verb+ Beyoncé + \\
	 context & \verb+ Beyoncé Giselle Knowles-Carter ... + \\
	 question & \verb+ When did Beyonce start becoming popular? + \\
	 answers & \verb+ {'text': ['in the late 1990s'], 'answer_start': [2... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set seq = [
'Answer the question depending on the context.',
'What is the answer?',
] %}

{{ seq | choice }}
Context: {{context}};
Question: {{question}};
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answers.text == [] %}
Answer not in context
{% else %}
{{answers.text[0]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text != [] %}
Determine the question that you might have asked to get back the following answer for the given context
Context: {{context}};
Answer: {{answers.text[0]}};
Question:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set seq = [
'What is this about? ',
'What is the paragraph about? ',
'Get the topic from: ',
'From the passage,  get the topic',
'I want to know the topic. ',
'Topic from the passage: ',
'Topic from the paragraph: ',
] %}
{{ seq | choice }}
{{context}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{title | replace("_", " ")}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set seq = [
'This is about ',
'What is this about? ',
'The paragraph is about ',
'What is the paragraph about? ',
'Get the topic: ',
'From the passage, the topic is',
'I want to know the topic. ',
'Topic from the passage: ',
'Topic from the paragraph: ',
] %}
{{context}}
{{ seq | choice }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{title | replace("_", " ")}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text != [] %}
What is a question that would give the following answer?
Answer: {{answers.text[0]}};
Question:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set seq = [
'Can you tell me ',
'Please tell me ',
'Tell me ',
'From the passage, ',
'I want to know ',
'I want to ask ',
'What is the answer to: ',
'Find the answer to: ',
'Answer: ',
'',
] %}
{{context}} {{ seq | choice }}{{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answers.text == [] %}
Answer not in context
{% else %}
{{answers.text[0]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if answers.text != [] %}
{{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text[0]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Context: {{context}}; 

Question: {{question}} 

Is this question answerable?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answers.text != [] %}
{{answer_choices[0]}}
{% else %}
{{answer_choices[1]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set seq = [
'Determine the topic of the question-answer pair. ',
'Find the topic. ',
'What is the topic from this? ',
] %}
{% if answers.text != [] %}
{{ seq | choice }}
Question: {{question}};  Answer: {{answers.text[0]}}; Topic:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{title}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
What is the following passage about?
{{context}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{title | replace("_", " ")}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{super\_glue record}
\noindent Dataset from \citet{zhang2018record}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ ['Nuria'] + \\
	 entities & \verb+ ['Afghanistan', 'Badam Bagh', 'Mariam', 'Nuria'] + \\
	 idx & \verb+ {'passage': 0, 'query': 0} + \\
	 passage & \verb+ The harrowing stories of women and children locked... + \\
	 query & \verb+ The baby she gave birth to is her husbands and he ... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ entities | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if ( answers | length ) > 0 %} 
{{ passage }} 
{{ query }} 
Which one is the "{{"@placeholder"}}"? {{ entities | join(", ") }}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ entities | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if ( answers | length ) > 0 %} 
The following document has been corrupted. Tell me what "{{"@placeholder"}}" is referring to.

Document: {{ passage }} 
{{ query }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ entities | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if ( answers | length ) > 0 %} 
{{ passage }} 
{{ query }} 

You should decide what "{{"@placeholder"}}" is referring to. Choose between:
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ entities | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if ( answers | length ) > 0 %} 
{{ passage }} 
{{ query }} 
In the question above, the "{{"@placeholder"}}" stands for
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ entities | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if ( answers | length ) > 0 %} 
{{ passage }} 
{{ query }} 
What could the "{{"@placeholder"}}" be? {{ entities | join(", ") }}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{entities | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if ( answers | length ) > 0 %}
{{ passage }}
{{ query }}

I am trying to decide what "{{"@placeholder"}}" means in the previous text.
Help by choosing an option between:
- {{ entities | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ entities | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if ( answers | length ) > 0 %} 
{{ passage }} 
{{ query }} 
Here, the placeholder refers to
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{entities | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if ( answers | length ) > 0 %}
Exercise: Extract from the text the correct entity that "{{"@placeholder"}}" is referring to.

{{ passage }}
{{ query }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{entities | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if ( answers | length ) > 0 %}
{{ passage }}
{{ query }}

Pick one option, "{{"@placeholder"}}" refers to:
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ entities | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if ( answers | length ) > 0 %} 
{{ passage }} 
{{ query }} 
Can you figure out what does the "{{"@placeholder"}}" mean? It means
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{qa\_srl}
\noindent 
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ ['four boat clubs', 'Aberdeen Boat Club', 'Aberdee... + \\
	 predicate & \verb+ row + \\
	 predicate\_idx & \verb+ 6 + \\
	 question & \verb+ ['what', '_', '_', 'rows', '_', '_', '_', '?'] + \\
	 sent\_id & \verb+ WIKI1_0 + \\
	 sentence & \verb+ There are four boat clubs that row on the River De... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Generate a plausible question that has the following answers based on the context:

Context: {{sentence}}

Answers: {{answers | join(", ")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question | join(" ") | replace("_ ", "")}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
The English teacher deconstructed an example sentence that contained the verb "{{predicate}}": {{sentence}}

{{question | join(" ") | replace("_ ", "")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Identify the predicate (the part of a sentence or clause containing a verb and stating something about the subject) in this sentence:

{{sentence}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{predicate}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{sentence}}
{{question|join(" ")|replace("_ ", "")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Here's a linguistic problem: you have to correctly identify the part of the sentence that answers the following {{"W"}} question.
Sentence: {{sentence}}
Question: {{question | join(" ") | replace("_ ", "")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Help me parse the structure of the following sentence constructed around the verb "{{predicate}}": {{sentence}}

{{question | join(" ") | replace("_ ", "")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{sentence}}

The previous sentence contains the verb "{{predicate}}". Answer this question about it: {{question|join(" ")|replace("_ ", "")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{quac}
\noindent Dataset from \citet{choi-etal-2018-quac}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ {'answer_starts': [[51], [640], [1862], [2024], [2... + \\
	 background & \verb+ The Malayali people or Keralite people (also spelt... + \\
	 context & \verb+ According to the Indian census of 2001, there were... + \\
	 dialogue\_id & \verb+ C_69758fcdfc1f46baba0e92c0f3b0919c_1 + \\
	 followups & \verb+ [2, 1, 1, 1, 1, 1, 1] + \\
	 orig\_answers & \verb+ {'texts': ['30,803,747 speakers of Malayalam in Ke... + \\
	 questions & \verb+ ['Where is Malayali located?', 'What other languag... + \\
	 section\_title & \verb+ Geographic distribution and population + \\
	 turn\_ids & \verb+ ['C_69758fcdfc1f46baba0e92c0f3b0919c_1_q#0', 'C_69... + \\
	 wikipedia\_page\_title & \verb+ Malayali + \\
	 yesnos & \verb+ [2, 2, 2, 2, 2, 0, 2] + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given the  partial dialogue : 

Student: {{questions[0]}}

Teacher: {{(answers.texts[0] | choice).replace("CANNOTANSWER","Cannot answer") }}

The context : {{context}}

Answer the question: {{questions[1] }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{(answers.texts[1] | choice).replace("CANNOTANSWER","Cannot answer")  }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given the dialogue: 
{% for i in range(0, questions | length - 1)%}
Student: {{questions[i]}}

Teacher: {{(answers.texts[i] | choice).replace("CANNOTANSWER","Cannot answer") }}
{% endfor %}

The context: {{context}}

Answer the question: {{questions | last }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{(answers.texts | last | choice).replace("CANNOTANSWER","Cannot answer") }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
This conversation happened between a teacher and a student:
{% for i in range(0, questions | length - 1) %}
Student: {{questions[i]}}

Teacher: {{(answers.texts[i] | choice).replace("CANNOTANSWER","Cannot answer") }}
{% endfor %}

Use the article : {{context}} to answer the question: {{questions | last }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{(answers.texts | last | choice).replace("CANNOTANSWER","Cannot answer") }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I read an article : {{context}} 

Then the following conversation occurred: 
{% for i in range(0, questions | length - 1) %}
Student: {{questions[i]}}

Teacher: {{(answers.texts[i] | choice).replace("CANNOTANSWER","Cannot answer") }}
{% endfor %}
Use both to answer the question:  {{questions | last }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{(answers.texts | last | choice).replace("CANNOTANSWER","Cannot answer") }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the article: {{context}} 

Then answer the question:  {{questions | last}}

You can use this dialogue to find the answer faster:
{% for i in range(0, questions | length - 1)%}
Student: {{questions[i]}}

Teacher: {{(answers.texts[i] | choice).replace("CANNOTANSWER","Cannot answer") }}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{(answers.texts | last | choice).replace("CANNOTANSWER","Cannot answer")  }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
A student is asking a teacher about the following article:
{{context}}

This is a summary of their conversation:
{% for i in range(0, questions | length - 1)%}
Student: {{questions[i]}}

Teacher: {{(answers.texts[i] | choice).replace("CANNOTANSWER","Cannot answer") }}
{% endfor %}

Use their conversation and the article to answer the question :  {{questions | last}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{(answers.texts | last | choice).replace("CANNOTANSWER","Cannot answer")  }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{quoref}
\noindent Dataset from \citet{allenai:quoref}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ {'answer_start': [250], 'text': ['Catherine']} + \\
	 context & \verb+ The earthquake swarm was noted on October 12, 2007... + \\
	 id & \verb+ ba3f052c7a557909526b59713430403dd134e01d + \\
	 question & \verb+ What is the first name of the person who doubted i... + \\
	 title & \verb+ 2007–2008 Nazko earthquakes 1 + \\
	 url & \verb+ https://en.wikipedia.org/wiki/2007%E2%80%932008_Na... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
The answer to the question: {{question}} is inside the article: {{context}}, can you guess it ?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given the following context:

{{context}}

answer the following question:

{{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
The following article contains an answer for the question: {{question}} , can you please find it? 

{{context}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
This article: {{context}} contains an answer for the question: {{question}}, what is it ?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{question}}

Answer the above question based on the context below:

{{context}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
What is the answer for the question: {{question}} from the following article ?

{{context}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I have a test where I am given the following article, what is an answer for the question: {{question}} ?

{{context}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given the below context:

{{context}}

Guess a valid title for it!
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{title}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Found the following article online, use it to answer the question: {{question}}

{{context}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
A friend asked me to answer this question: {{question}}, using the article: {{context}}, what would be the answer ?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the following paragraph and extract the answer for the question: {{question}}

{{context}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{QA Generative }
\subsubsection{drop}
\noindent Dataset from \citet{Dua2019DROP}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 section\_id & \verb+ nfl_2201 + \\
	 query\_id & \verb+ f16c0ee7-f131-4a8b-a6ac-4d275ea68066 + \\
	 passage & \verb+ To start the season, the Lions traveled south to T... + \\
	 question & \verb+ How many points did the buccaneers need to tie in ... + \\
	 answers\_spans & \verb+ {'spans': ['3'], 'types': ['number']} + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Question: {{question}}
Answer based on following passage.

{{passage}}

Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers_spans.spans | join(", ") }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I am trying to figure out the answer to the question, "{{question}}" I found the following text-snippet has the answer. Can you tell me the answer?

{{passage}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers_spans.spans | join(", ") }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Passage: {{passage}}
Question: {{question}}
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers_spans.spans | join(", ") }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Generate a question from the following passage that has the answer, {{ answers_spans.spans | join(", ") }}
Passage : {{passage}}
Question :
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Context: {{passage}}
I am trying to figure out the answer to the question from the above context.  Can you tell me the answer?
Question: {{question}}
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers_spans.spans | join(", ") }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{QA Multiple Choice }
\subsubsection{cos\_e v1.11}
\noindent 
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 abstractive\_explanation & \verb+ webmath is designed to help you solve + \\
	 answer & \verb+ math problem + \\
	 choices & \verb+ ['park', 'coloring book', 'garden center', 'math p... + \\
	 extractive\_explanation & \verb+ "there are 10 apples on an apple tree. three fall ... + \\
	 id & \verb+ 6b819727eb8a670df26a7ffad036c119 + \\
	 question & \verb+ "There are 10 apples on an apple tree.  Three fall... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ choices | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ question }}
Choose the most suitable option to answer the above question.
Options:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ question }}
Choose the most suitable option to answer the above question.
Options:
{% for k in range(choices | length) %}
{{'. '.join([answer_choices[k], choices[k]])}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[choices.index(answer)] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Question: {{question}}

Choices: 
- {{ choices | join("\n- ") }}

The rationale to choose "{{answer}}" as the answer is that:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{abstractive_explanation}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ choices | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ question }}
- {{ answer_choices | join("\n- ") }}

The best answer is
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Here's a question and a few possible answers: 

Q: {{ question }}
Possible A: {{ choices | join(", ") }}

Why is "{{answer}}" an answer aligned with human common sense?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ abstractive_explanation }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Pick the option in line with common sense to answer the question.
Question: {{ question }}
Options:
{% for k in range(choices | length) %}
{{'. '.join([answer_choices[k], choices[k]])}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[choices.index(answer)] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Question: {{ question }}
Options:
- {{ choices | join("\n- ") }}

Explain why a human would choose "{{answer}}" to answer the question above:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ abstractive_explanation }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Question: {{ question }}
Options:
- {{ choices | join("\n- ") }}

The answer is "{{ answer }}" because
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ abstractive_explanation }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ choices | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Pick the option in line with common sense to answer the question.
Questions: {{ question }}
Options:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Here's a question: {{ question }}

Here are possible answers to this question:
- {{ choices | join("\n- ") }}

I believe the correct choice is "{{answer}}", here's why:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ abstractive_explanation }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ question }}
{% for k in range(choices | length) %}
{{'. '.join([answer_choices[k], choices[k]])}}
{% endfor %}
The best answer is
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[choices.index(answer)] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{cosmos\_qa}
\noindent Dataset from \citet{cosmos}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer0 & \verb+ None of the above choices . + \\
	 answer1 & \verb+ This person likes music and likes to see the show ... + \\
	 answer2 & \verb+ This person only likes Good Old War and Person L ,... + \\
	 answer3 & \verb+ Other Bands is not on tour and this person can not... + \\
	 context & \verb+ Good Old War and person L : I saw both of these ba... + \\
	 id & \verb+ 3Q9SPIIRWJKVQ8244310E8TUS6YWAC##34V1S5K3GTZMDUBNBI... + \\
	 label & \verb+ 1 + \\
	 question & \verb+ In the future , will this person go to see other b... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Based on the context and the answer, generate a question. 

Context: {{context}}

Answer:
{% if label == 0 %}
{{answer0}}
{% elif label == 1 %}
{{answer1}}
{% elif label == 2 %}
{{answer2}}
{% elif label == 3 %}
{{answer3}}
{% endif %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the following context and choose the best option to answer the question.
Context: {{ context }}
Question: {{ question }}
Options: 
- {{ answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the following context and answer the question.
Context: {{ context }}
Question: {{ question }}
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the following context and choose the best option to answer the question.
Context: {{ context }}
Question: {{ question }}
Options: 
A. {{ answer0 }}
B. {{ answer1 }}
C. {{ answer2 }}
D. {{ answer3 }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
According to the above context, choose the best option to answer the following question.
Question: {{ question }}
Options:
- {{answer_choices | join("\n - ")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
{{ question }}
A. {{ answer0 }}
B. {{ answer1 }}
C. {{ answer2 }}
D. {{ answer3 }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
Question: {{ question }}
The answer to the above question:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
{{ question }}
- {{ answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
According to the above context, choose the best option to answer the following question.
Question: {{ question }}
Options:
A. {{ answer0 }}
B. {{ answer1 }}
C. {{ answer2 }}
D. {{ answer3 }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
{{ question }}
Pick the best answer from the following options:
A. {{ answer0 }}
B. {{ answer1 }}
C. {{ answer2 }}
D. {{ answer3 }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
According to the above context, answer the following question.
{{ question }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
{{ question }}
Pick the best answer from the following options:
- {{ answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{dream}
\noindent Dataset from \citet{sundream2018}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ Continue her dancing class. + \\
	 choice & \verb+ ['Consult her dancing teacher.', 'Take a more inte... + \\
	 dialogue & \verb+ ['M: I am considering dropping my dancing class. I... + \\
	 dialogue\_id & \verb+ 5-510 + \\
	 id & \verb+ 0 + \\
	 question & \verb+ What does the man suggest the woman do? + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the below conversation.

{{dialogue[:-1] | join("\n\n")}}

What would the listener say?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{dialogue[-1]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given the question "{{question}}" and the answer "{{answer}}", write a conversation that might have happened.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{dialogue | join("\n\n")}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{dialogue[1:] | join("\n\n")}}

What was said before this conversation?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{dialogue[0]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Dialogue:

{{dialogue | join("\n\n")}}

Question: {{question}} 

- {{answer_choices[0]}}

- {{answer_choices[1]}}

- {{answer_choices[2]}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the following conversation and answer the question.

{{dialogue | join("\n\n")}}

Question: {{question}} 

- {{answer_choices[0]}}

- {{answer_choices[1]}}

- {{answer_choices[2]}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{openbookqa main}
\noindent Dataset from \citet{OpenBookQA2018}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answerKey & \verb+ D + \\
	 choices & \verb+ {'label': ['puppies learning new tricks', 'childre... + \\
	 id & \verb+ 7-980 + \\
	 question\_stem & \verb+ The sun is responsible for + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{question_stem}}

Choose an answer from this list:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answerKey]]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{question_stem}}

Which is the correct answer?
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answerKey]]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{question_stem}}
{% for k in range(choices["text"] | length) %}
{{' -> '.join([["A", "B", "C", "D"][k], choices["text"][k]])}}
{% endfor %}
Is the right answer {{"A, B, C or D"}} ?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answerKey}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{question_stem}}

Choices:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answerKey]]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{question_stem}}
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answerKey]]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{question_stem}}
- {{ answer_choices | join("\n- ") }}

Which is the correct answer?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answerKey]]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{question_stem}}

Pick the right answer from the list:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answerKey]]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{qasc}
\noindent Dataset from \citet{allenai:qasc}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answerKey & \verb+ F + \\
	 choices & \verb+ {'label': ['A', 'B', 'C', 'D', 'E', 'F', 'G', 'H']... + \\
	 combinedfact & \verb+ Beads of water can be formed by clouds. + \\
	 fact1 & \verb+ beads of water are formed by water vapor condensin... + \\
	 fact2 & \verb+ Clouds are made of water vapor. + \\
	 formatted\_question & \verb+ What type of water formation is formed by clouds? ... + \\
	 id & \verb+ 3E7TUJ2EGCLQNOV1WEAJ2NN9ROPD9K + \\
	 question & \verb+ What type of water formation is formed by clouds? + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
If I tell you that {{combinedfact[0]|capitalize}}{{ combinedfact[1:]|trim('.') }}, and ask you the question "{{ question[0]|lower }}{{ question[1:] }}", is the correct answer "{{ choices.text[0][0]|lower}}{{ choices.text[0][1:]|trim('.') }}"?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answerKey == choices.label[0] %} Yes {% else %} No {% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ fact1[0]|capitalize }}{{ fact1[1:]|trim|trim('.') }}, and {{fact2[0]|lower }}{{ fact2[1:]|trim|trim('.') }}. Given these facts, {{ question[0]|lower }}{{question[1:]|trim('?') }} among the following options:
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for choice in choices.label %} {% if choice == answerKey %}{{ answer_choices[loop.index - 1] }}{% endif %}{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Fact 1: {{ fact1[0]|capitalize }}{{ fact1[1:]|trim|trim('.') }}.

Fact 2: {{fact2[0]|capitalize }}{{ fact2[1:]|trim|trim('.') }}.

Given the two facts above, {{ question[0]|lower }}{{question[1:]|trim('?') }}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for choice in choices.label %} {% if choice == answerKey %}{{ answer_choices[loop.index - 1] }}{% endif %}{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
You are presented with the question "{{ question }}" and the following answer choices: 
- {{answer_choices | join("\n - ") }}

Now knowing that {{ fact1[0]|lower }}{{ fact1[1:]|trim|trim('.') }} and {{fact2[0]|lower }}{{ fact2[1:]|trim|trim('.') }}, choose the best answer.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for choice in choices.label %} {% if choice == answerKey %}{{ answer_choices[loop.index - 1] }}{% endif %}{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
You are presented with the quiz "{{ question }}" 

But you don't know the answer, so you turn to your teacher to ask for hints. He says that "{{ fact1[0]|lower }}{{ fact1[1:]|trim|trim('.') }}" and "{{fact2[0]|lower }}{{ fact2[1:]|trim|trim('.') }}". 

So, what's the best answer to the question?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for choice in choices.label %} {% if choice == answerKey %}{{ answer_choices[loop.index - 1] }}{% endif %}{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
If {{ combinedfact[0]|lower }}{{ combinedfact[1:]|trim|trim('.') }}, then {{ question[0]|lower }}{{question[1:]|trim|trim('?') }}?

Answer choices:
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for choice in choices.label %} {% if choice == answerKey %}{{ answer_choices[loop.index - 1] }}{% endif %}{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Do you think the right answer to the question "{{ question[0]|lower }}{{ question[1:] }}" is "{{ choices.text[1][0]|lower}}{{ choices.text[1][1:]|trim('.') }}", given that
 {{combinedfact[0]|lower}}{{ combinedfact[1:]|trim('.') }}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answerKey == choices.label[0] %} Yes {% else %} No {% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Fact 1: {{ fact1[0]|capitalize }}{{ fact1[1:]|trim|trim('.') }}.

Fact 2: {{fact2[0]|capitalize }}{{ fact2[1:]|trim|trim('.') }}.

Given the two facts above, answer the question "{{ question }}" with the following options: 
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for choice in choices.label %} {% if choice == answerKey %}{{ answer_choices[loop.index - 1] }}{% endif %}{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{quail}
\noindent Dataset from \citet{DBLP:conf/aaai/RogersKDR20}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ ['not enough information', 'to visit family', 'par... + \\
	 context & \verb+ That fall came and I went back to Michigan and the... + \\
	 context\_id & \verb+ f001 + \\
	 correct\_answer\_id & \verb+ 3 + \\
	 domain & \verb+ fiction + \\
	 id & \verb+ f001_0 + \\
	 metadata & \verb+ {'author': 'Joseph Devon', 'title': 'Black Eyed Su... + \\
	 question & \verb+ Why was this character sent away after each school... + \\
	 question\_id & \verb+ 0 + \\
	 question\_type & \verb+ Causality + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
Question: {{ question }}
Options:
{% for k in range(answers | length) %}
{{'. '.join([answer_choices[k], answers[k]])}}
{% endfor %}
===
The correct answer is
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
Question: {{ question }}
Options:
- {{ answer_choices | join(" \n - ") }}
===
The correct answer is
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the following context and choose the correct option to answer the question.
Context: {{ context }}
Question: {{ question }}
Options:
{% for k in range(answers | length) %}
{{'. '.join([answer_choices[k], answers[k]])}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
{{ question }}
Pick the correct answer from the following options:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
Question: {{ question }}
===
The answer to the above question is
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
According to the above context, answer the following question.
{{ question }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
{{ question }}
Pick the correct answer from the following options:
{% for k in range(answers | length) %}
{{'. '.join([answer_choices[k], answers[k]])}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
{{ question }}
{% for k in range(answers | length) %}
{{'. '.join([answer_choices[k], answers[k]])}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
According to the above context, choose the correct option to answer the following question.
Question: {{ question }}
Options:
{% for k in range(answers | length) %}
{{'. '.join([answer_choices[k], answers[k]])}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the following context and answer the question.
Context: {{ context }}
Question: {{ question }}
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
{{ question }}
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ context }}
According to the above context, choose the correct option to answer the following question.
Question: {{ question }}
Options:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the following context and choose the correct option to answer the question.
Context: {{ context }}
Question: {{ question }}
Options:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{quarel}
\noindent Dataset from \citet{quarel_v1}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ QuaRel_V1_Fr_0223 + \\
	 answer\_index & \verb+ 1 + \\
	 logical\_forms & \verb+ ['(infer (speed higher world1) (smoothness higher ... + \\
	 logical\_form\_pretty & \verb+ qrel(speed, higher, world1) -> qrel(smoothness, hi... + \\
	 world\_literals & \verb+ {'world1': ['ice'], 'world2': ['snow']} + \\
	 question & \verb+ Mike was snowboarding on the snow and hit a piece ... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{world_literals.world1[0]}} ||| {{world_literals.world2[0]}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Question: {{question}}

Do not use {{"A"}} and {{"B"}} to answer the question but instead, choose between "{{answer_choices[0]}}" and  "{{answer_choices[1]}}".
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer_index]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{world_literals.world1[0]}} ||| {{world_literals.world2[0]}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Here's a logic test: {{question}}

Choose the answer between "{{answer_choices[0]}}" and "{{answer_choices[1]}}".
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer_index]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{world_literals.world1[0]}} ||| {{world_literals.world2[0]}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Here's a short story: {{question}}.

What is the most sensical answer between "{{answer_choices[0]}}" and  "{{answer_choices[1]}}"?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer_index]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{world_literals.world1[0]}} ||| {{world_literals.world2[0]}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Choose between "{{answer_choices[0]}}" and  "{{answer_choices[1]}}".
Question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer_index]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{world_literals.world1[0]}} ||| {{world_literals.world2[0]}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I am testing my students' logic.
What is the answer they should choose between "{{answer_choices[0]}}" and "{{answer_choices[1]}}"?
Logic test: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer_index]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{quartz}
\noindent Dataset from \citet{quartz}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answerKey & \verb+ A + \\
	 choices & \verb+ {'label': ['A', 'B'], 'text': ['scarce', 'plentifu... + \\
	 id & \verb+ QRQA-10385-4 + \\
	 para & \verb+ Many of the worlds people live with water scarcity... + \\
	 para\_anno & \verb+ {'effect_prop': 'population growth', 'cause_dir_st... + \\
	 para\_id & \verb+ QRSent-10385 + \\
	 question & \verb+ John's town used to have lots of water, back when ... + \\
	 question\_anno & \verb+ {'more_effect_dir': 'several thousand', 'less_effe... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Use information from the paragraph to answer the question.

Question:

{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!") }} {{ answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}

Paragraph :

{{ para }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ para }}
{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!")}} {{ answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Use information from the paragraph to answer the question.

Paragraph :

{{ para }}

Question:

{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!") }} {{ answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Answer the question based on the following text.

Question:

{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!") }} {{ answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}

Text:

{{ para }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Answer the question below:

{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!") }} {{  answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}

Assuming that:

{{ para }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the passage below and choose the right answer to the following question (choices are {{ answer_choices | join(" or ") }} ):

{{ para }}

{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!") }} {{ answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ para }}

Having read the above passage, choose the right answer to the following question (choices are {{ answer_choices | join(" or ") }} ):

{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!") }} {{ answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given the fact that:

{{ para }}

Answer the question:

{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!") }} {{ answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{race high}
\noindent Dataset from \citet{lai2017large}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ D + \\
	 article & \verb+ Studies show that you may be lied to every day any... + \\
	 example\_id & \verb+ high10001.txt + \\
	 options & \verb+ ['harmful', 'easy', 'interesting', 'common'] + \\
	 question & \verb+ From Para.1 we learn that lying is very   _  . + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set candidate = ["A", "B", "C", "D"] | choice %}
Article: {{article}}
Question: {{question}}
Yes or no, is the answer "{{ [options.0,options.1,options.2,options.3][{"A":0,"B":1,"C":2,"D":3}[answer]] }}"?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if candidate == answer %}
Yes
{% else %}
No
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Write a multi-choice question for the following article:
Article: {{article}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
Question: 
{{question}}
Options:
{{"A"}} {{options.0}}
{{"B"}} {{options.1}}
{{"C"}} {{options.2}}
{{"D"}} {{options.3}}
Answer:
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I'm taking a test and have to guess the right answer to the question after the article.
Article: {{article}}
Question: {{question}}
Options: {{"A"}}: {{options.0}}
{{"B"}}: {{options.1}}
{{"C"}}: {{options.2}}
{{"D"}}: {{options.3}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the article and select the best answer.
Article: {{article}}
Question: {{question}}
Options: {{"A"}}: {{options.0}}
{{"B"}}: {{options.1}}
{{"C"}}: {{options.2}}
{{"D"}}: {{options.3}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Write a multi-choice question for the following article, with the given choices and answer:
Article: {{article}}
Options:
{{"A"}} {{options.0}}
{{"B"}} {{options.1}}
{{"C"}} {{options.2}}
{{"D"}} {{options.3}}
Answer:
{{answer}} {{ [options.0,options.1,options.2,options.3][{"A":0,"B":1,"C":2,"D":3}[answer]] }}
Question:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ options | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the following article and select the best answer.
Article: {{article}}
Question: {{question}}
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answer]]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{article}}
{{question}}
{{"A)"}} {{options.0}}
{{"B)"}} {{options.1}}
{{"C)"}} {{options.2}}
{{"D)"}} {{options.3}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ options | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the following article and answer the question.
Article: {{article}}
Question: {{question}}
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[{"A":0,"B":1,"C":2,"D":3}[answer]] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{race middle}
\noindent Dataset from \citet{lai2017large}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ C + \\
	 article & \verb+ Take a class at Dulangkou School, and you'll see l... + \\
	 example\_id & \verb+ middle1.txt + \\
	 options & \verb+ ['take care of the whole group', 'make sure that e... + \\
	 question & \verb+ A discipline leader is supposed to  _  . + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the article and select the best answer.
Article: {{article}}
Question: {{question}}
Options: {{"A"}}: {{options.0}}
{{"B"}}: {{options.1}}
{{"C"}}: {{options.2}}
{{"D"}}: {{options.3}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ options | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the following article and answer the question.
Article: {{article}}
Question: {{question}}
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[{"A":0,"B":1,"C":2,"D":3}[answer]] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set candidate = ["A", "B", "C", "D"] | choice %}
Article: {{article}}
Question: {{question}}
Yes or no, is the answer "{{ [options.0,options.1,options.2,options.3][{"A":0,"B":1,"C":2,"D":3}[answer]] }}"?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if candidate == answer %}
Yes
{% else %}
No
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{article}}
{{question}}
{{"A)"}} {{options.0}}
{{"B)"}} {{options.1}}
{{"C)"}} {{options.2}}
{{"D)"}} {{options.3}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ options | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the following article and select the best answer.
Article: {{article}}
Question: {{question}}
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answer]]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Write a multi-choice question for the following article, with the given choices and answer:
Article: {{article}}
Options:
{{"A"}} {{options.0}}
{{"B"}} {{options.1}}
{{"C"}} {{options.2}}
{{"D"}} {{options.3}}
Answer:
{{answer}} {{ [options.0,options.1,options.2,options.3][{"A":0,"B":1,"C":2,"D":3}[answer]] }}
Question:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Write a multi-choice question for the following article:
Article: {{article}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
Question: 
{{question}}
Options:
{{"A"}} {{options.0}}
{{"B"}} {{options.1}}
{{"C"}} {{options.2}}
{{"D"}} {{options.3}}
Answer:
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I'm taking a test and have to guess the right answer to the question after the article.
Article: {{article}}
Question: {{question}}
Options: {{"A"}}: {{options.0}}
{{"B"}}: {{options.1}}
{{"C"}}: {{options.2}}
{{"D"}}: {{options.3}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{sciq}
\noindent Dataset from \citet{SciQ}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 question & \verb+ What type of organism is commonly used in preparat... + \\
	 distractor3 & \verb+ viruses + \\
	 distractor1 & \verb+ protozoa + \\
	 distractor2 & \verb+ gymnosperms + \\
	 correct\_answer & \verb+ mesophilic organisms + \\
	 support & \verb+ Mesophiles grow best in moderate temperature, typi... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{distractor1}} ||| {{distractor2}} ||| {{distractor3}} ||| {{correct_answer}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Q: {{question}}


A:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[3]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{distractor1}} ||| {{distractor2}} ||| {{distractor3}} ||| {{correct_answer}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set order = [[0, 1, 2, 3], [0, 1, 3, 2], [0, 2, 1, 3], [0, 2, 3, 1], [0, 3, 1, 2], [0, 3, 2, 1],
                             [1, 0, 2, 3], [1, 0, 3, 2], [1, 2, 0, 3], [1, 2, 3, 0], [1, 3, 0, 2], [1, 3, 2, 0],
                             [2, 1, 0, 3], [2, 1, 0, 2], [2, 0, 1, 3], [2, 0, 3, 1], [2, 3, 1, 0], [2, 3, 0, 1],
                             [3, 1, 2, 0], [3, 1, 0, 2], [3, 2, 1, 0], [3, 2, 0, 1], [3, 0, 1, 2], [3, 0, 2, 1]] | choice %}
Q: {{question}}


 Choices:

- {{ answer_choices[order[0]] }}

- {{ answer_choices[order[1]] }}

- {{ answer_choices[order[2]] }}

- {{ answer_choices[order[3]] }}

A:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[3]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{distractor1}} ||| {{distractor2}} ||| {{distractor3}} ||| {{correct_answer}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set order = [[0, 1, 2, 3], [0, 1, 3, 2], [0, 2, 1, 3], [0, 2, 3, 1], [0, 3, 1, 2], [0, 3, 2, 1],
                             [1, 0, 2, 3], [1, 0, 3, 2], [1, 2, 0, 3], [1, 2, 3, 0], [1, 3, 0, 2], [1, 3, 2, 0],
                             [2, 1, 0, 3], [2, 1, 0, 2], [2, 0, 1, 3], [2, 0, 3, 1], [2, 3, 1, 0], [2, 3, 0, 1],
                             [3, 1, 2, 0], [3, 1, 0, 2], [3, 2, 1, 0], [3, 2, 0, 1], [3, 0, 1, 2], [3, 0, 2, 1]] | choice %}
Q: {{question}}


Read this paragraph and choose the correct option from the provided answers:

{{support}}

 Choices:

- {{ answer_choices[order[0]] }}

- {{ answer_choices[order[1]] }}

- {{ answer_choices[order[2]] }}

- {{ answer_choices[order[3]] }}


A:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[3]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{distractor1}} ||| {{distractor2}} ||| {{distractor3}} ||| {{correct_answer}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set order = [[0, 1, 2, 3], [0, 1, 3, 2], [0, 2, 1, 3], [0, 2, 3, 1], [0, 3, 1, 2], [0, 3, 2, 1],
                             [1, 0, 2, 3], [1, 0, 3, 2], [1, 2, 0, 3], [1, 2, 3, 0], [1, 3, 0, 2], [1, 3, 2, 0],
                             [2, 1, 0, 3], [2, 1, 0, 2], [2, 0, 1, 3], [2, 0, 3, 1], [2, 3, 1, 0], [2, 3, 0, 1],
                             [3, 1, 2, 0], [3, 1, 0, 2], [3, 2, 1, 0], [3, 2, 0, 1], [3, 0, 1, 2], [3, 0, 2, 1]] | choice %}
Answer the following question given this paragraph: 

{{support}}


Q: {{question}}

 Choices:

- {{ answer_choices[order[0]] }}

- {{ answer_choices[order[1]] }}

- {{ answer_choices[order[2]] }}

- {{ answer_choices[order[3]] }}

A:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[3]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{distractor1}} ||| {{distractor2}} ||| {{distractor3}} ||| {{correct_answer}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Answer the following question given this paragraph: 

{{support}}


Q: {{question}}


A:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[3]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{social\_i\_qa}
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answerA & \verb+ like attending + \\
	 answerB & \verb+ like staying home + \\
	 answerC & \verb+ a good friend to have + \\
	 context & \verb+ Cameron decided to have a barbecue and gathered he... + \\
	 label & \verb+ 1 + \\
	 question & \verb+ How would Others feel as a result? + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answerA}} ||| {{answerB}} ||| {{answerC}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I heard that {{context}}

And I was wondering {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label | int - 1]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answerA}} ||| {{answerB}} ||| {{answerC}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{context}}

Given the context: {{question}}

Possible answers: {{answer_choices | join(", ")}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label | int - 1]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set random_answer_id = range(0,2) | choice%}
{% set answers = [answerA, answerB, answerC] %}
{{context}}

Given the question "{{question}}", is "{{answers[random_answer_id]}}" a valid answer?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if (label | int) - 1 == random_answer_id %}
    Yes
{% else %}
    No
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{context}}

Given that the answer to a question is "{{{"1": answerA, "2": answerB, "3": answerC}[label]}}", what is the question?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answerA}} ||| {{answerB}} ||| {{answerC}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{context}}

Given the context: {{question}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label | int - 1]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Context: {{context}}

Question: {{question}}

Which one of these answers best answers the question according to the context?

A: {{answerA}}

B: {{answerB}}

C: {{answerC}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{{"1": "A", "2": "B", "3": "C"}[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{super\_glue boolq}
\noindent Dataset from \citet{clark2019boolq}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 idx & \verb+ 0 + \\
	 label & \verb+ 1 + \\
	 passage & \verb+ Persian language -- Persian , al... + \\
	 question & \verb+ do iran and afghanistan speak the same language + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
False ||| True
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1 %}
Passage: {{passage}}

After reading this passage, I have a question: {{question}}? True or False?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1 %}
{{ passage }} 
Question: {{ question }}
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1 %}
{{ passage }} 

Having read that, I wonder {{ question }}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }} 
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1 %}
Text: {{passage}}

Answer the following yes/no question: {{question}}? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1 %}
{{ passage }} 

Having read that, could you tell me {{ question }}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1 %}
EXAM
1. Answer by yes or no.

Document: {{passage}}
Question: {{question}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1 %}
Based on the following passage, {{ question }}? {{ passage }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
False ||| True
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1 %}
Exercise: read the text and answer the question by True or False.

Text: {{passage}}
Question: {{question}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1 %}
{{ passage }}
Based on the previous passage, {{ question }}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
False ||| True
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1 %}
{{passage}}

Q: {{question}}? True or False?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{super\_glue copa}
\noindent Dataset from \citet{roemmele2011choice}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 choice1 & \verb+ The sun was rising. + \\
	 choice2 & \verb+ The grass was cut. + \\
	 idx & \verb+ 0 + \\
	 label & \verb+ 0 + \\
	 premise & \verb+ My body cast a shadow over the grass. + \\
	 question & \verb+ cause + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Exercise: choose the most plausible alternative.

{{ premise }} {% if question == "cause" %} because... {% else %} so... {% endif %}
- {{choice1}}
- {{choice2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if question == "effect" %} 
{{ premise }} What could happen next, "{{ answer_choices[0] }}" or "{{ answer_choices[1] }}"?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ premise }} 

I am hesitating between two options. Help me choose the more likely {% if question == "cause" %} cause: {% else %} effect: {% endif %}
- {{choice1}}
- {{choice2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ premise }} {% if question == "cause" %} This happened because... {% else %} As a consequence... {% endif %}
Help me pick the more plausible option:
- {{choice1}}
- {{choice2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1 }} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
"{{ answer_choices[0] }}" or "{{ answer_choices[1] }}"? {{ premise }} {% if question == "cause" %} because {% else %} so {% endif %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if question == "effect" %} 
{{ premise }} As a result, "{{ answer_choices[0] }}" or "{{ answer_choices[1] }}"?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ premise }} 

What's the best option?
- {{choice1}}
- {{choice2}}

We are looking for {% if question == "cause" %} a cause {% else %} an effect {% endif %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if question == "cause" %} 
{{ premise }} Which may be caused by "{{ answer_choices[0] }}" or "{{ answer_choices[1] }}"?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Pick the more likely continuation to the following sentence:
{{ premise }} {% if question == "cause" %} as a result of: {% else %} as a consequence: {% endif %}
- {{choice1}}
- {{choice2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ premise }}

Select the most plausible {% if question == "cause" %} cause: {% else %} effect: {% endif %}
- {{choice1}}
- {{choice2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if question == "cause" %} 
{{ premise }} Why? "{{ answer_choices[0] }}" or "{{ answer_choices[1] }}"?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ premise }} {% if question == "cause" %} because... {% else %} so... {% endif %}
Choose between:
- {{choice1}}
- {{choice2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{super\_glue multirc}
\noindent Dataset from \citet{MultiRC2018}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ Children, Gerd, or Dorian Popa + \\
	 idx & \verb+ {'paragraph': 0, 'question': 0, 'answer': 0} + \\
	 label & \verb+ 0 + \\
	 paragraph & \verb+ While this process moved along, diplomacy continue... + \\
	 question & \verb+ What did the high-level effort to persuade Pakista... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{paragraph}}

Question: {{question}}
I found this answer "{{answer}}". Is that correct? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ paragraph }}
Based on the previous passage, {{ question }} 
Is "{{ answer }}" a correct answer?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{paragraph}}
Question: {{question}}

I am grading my students' exercises. Is the answer "{{answer}}" correct?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ paragraph }}
{{ question }} 
Would it be good to answer "{{ answer }}"?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ paragraph }}
Question: {{ question }} 
Is it {{ answer }}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{paragraph}}

Decide whether "{{answer}}" is a valid answer to the following question: {{question}}
Answer yes or no.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ paragraph }}
Question: {{ question }} 
Is the correct answer {{ answer }}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Is "{{answer}}" a correct answer to the following question?
Question: {{question}}

Rely on the following text: {{paragraph}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{paragraph}}

Question: {{question}}
I think "{{answer}}" is a valid answer. Could you confirm? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ paragraph }}
{{ question }} 
I was going to say "{{ answer }}". Does that sound right?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{wiki\_hop original}
\noindent Dataset from \citet{welbl2018constructing}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 annotations & \verb+ [] + \\
	 answer & \verb+ 1996 summer olympics + \\
	 candidates & \verb+ ['1996 summer olympics', 'olympic games', 'sport'] + \\
	 id & \verb+ WH_train_0 + \\
	 question & \verb+ participant_of juan rossell + \\
	 supports & \verb+ ['The 2004 Summer Olympic Games, officially known ... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{candidates | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
What object entity has the relation of '{{ question_split[0] | replace("_", " ")}}' with the subject '{{ question_split[1:] | join(" ")}}'? 

Choices:
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
What is the relationship between '{{ question_split[1:] | join(" ")}}' and '{{answer}}'?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ question_split[0] | replace("_", " ") }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
What entity does '{{ question_split[1:] | join(" ")}}' has the relation '{{ question_split[0] | replace("_", " ") }}' with?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
Given the paragraphs above, decide what entity has the relation '{{ question_split[0] | replace("_", " ") }}' with '{{answer}}'.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ question_split[1:] | join(" ")}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{candidates | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
Given the information above, choose from the list below the object entity that exhibits the relation '{{ question_split[0] | replace("_", " ")}}' with the subject '{{ question_split[1:] | join(" ")}}'.

Choices:
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{candidates | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
After reading the paragraphs above, we are interested in knowing the entity with which '{{ question_split[1:] | join(" ")}}' exhibits the relationship of '{{ question_split[0] | replace("_", " ")}}'. Find the answer from the choices below.

Choices:
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
Given the information, choose the subject and object entities that have the relation of '{{ question_split[0] | replace("_", " ") }}'.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ question_split[1:] | join(" ") }} , {{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{candidates | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
After reading the paragraphs above, choose the best answer for the entity that related to '{{ question_split[1:] | join(" ")}}' with the relationship of '{{ question_split[0] | replace("_", " ")}}'.

Choices:
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{candidates | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
'{{ question_split[1:] | join(" ")}}' is related to which object entity through the relation of '{{ question_split[0] | replace("_", " ")}}'?

Choices:
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{wiqa}
\noindent Dataset from \citet{wiqa}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer\_label & \verb+ more + \\
	 answer\_label\_as\_choice & \verb+ A + \\
	 choices & \verb+ {'label': ['A', 'B', 'C'], 'text': ['more', 'less'... + \\
	 metadata\_graph\_id & \verb+ 144 + \\
	 metadata\_para\_id & \verb+ 1217 + \\
	 metadata\_path\_len & \verb+ 2 + \\
	 metadata\_question\_id & \verb+ influence_graph:1217:144:106#0 + \\
	 metadata\_question\_type & \verb+ INPARA_EFFECT + \\
	 question\_para\_step & \verb+ ['A tree produces seeds', 'The seeds are dispersed... + \\
	 question\_stem & \verb+ suppose there will be fewer new trees happens, how... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
-  {{ question_para_step[1:] | join("\n- ") }}

What might be the first step of the process?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ question_para_step | first }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set process_list = question_para_step[:-1] if question_para_step[-1] == "" else question_para_step %}
-  {{ process_list[:-1] | join("\n- ") }}

What might be the last step of the process?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ process_list | last }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
What is the missing first step of the following process:

-  {{ question_para_step[1:] | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ question_para_step | first }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set process_list = question_para_step[:-1] if question_para_step[-1] == "" else question_para_step %}
What is the final step of the following process:
-  {{ process_list[:-1] | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ process_list | last }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Process:
- {{ question_para_step | join("\n- ")}}

Question:
{{question_stem}}

How does the supposed perturbation influence the second effect mentioned. Answer by {{"more, less or no effect"}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_label|replace("_", " ")}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Process:

- {{ question_para_step | join("\n- ") }}

{{question_stem}}

Which of the following is the supposed perturbation?

- {{"directly impacting a step of the process"}}
- {{"indirectly impacting a step of the process"}}
- {{"not impacting any step of the process"}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{{"EXOGENOUS_EFFECT": "indirectly impacting a step of the process", "OUTOFPARA_DISTRACTOR": "not impacting any step of the process", "INPARA_EFFECT": "directly impacting a step of the process"}[metadata_question_type]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Process:
- {{ question_para_step | join("\n- ")}}

Question:
{{question_stem}}

- {{"A: more"}}
- {{"B: less"}}
- {{"C: no effect"}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_label_as_choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Process:

- {{ question_para_step | join("\n- ") }}

Perturbation hypothesis:
{{question_stem}}

Does the supposed perturbation have an effect (direct or indirect) on the process?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{{"EXOGENOUS_EFFECT": "yes", "OUTOFPARA_DISTRACTOR": "no", "INPARA_EFFECT": "yes"}[metadata_question_type]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{circa}
\noindent Dataset from \citet{louis_emnlp2020}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer-Y & \verb+ I'm a veterinary technician. + \\
	 canquestion-X & \verb+ I am employed . + \\
	 context & \verb+ Y has just travelled from a different city to meet... + \\
	 goldstandard1 & \verb+ 0 + \\
	 goldstandard2 & \verb+ 0 + \\
	 judgements & \verb+ Yes#Yes#Yes#Yes#Yes + \\
	 question-X & \verb+ Are you employed? + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Convert this question to a sentence declarative sentence asserting an affirmative answer:

{{question_X}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{canquestion_X}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if goldstandard2 != -1 %}

Given the question-answer pair of X and Y in the context of {{context}}, which of the following answers is Y implying: "{{"Yes"}}", "{{"No"}}", "{{"In the middle, neither yes nor no"}}", "{{"Probably yes / sometimes yes"}}", "{{"Probably no"}}", "{{"Yes, subject to some conditions"}}", "{{"Other"}}" or "{{"I am not sure how X will interpret Y’s answer"}}" ?

X: {{question_X}} 

Y: {{answer_Y}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{   answer_choices[goldstandard2]}}

{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
What is a possible question X could ask Y given the context of {{context}} that would cause Y to answer "{{answer_Y}}"?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question_X}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if goldstandard1 != -1 %}

Given the question-answer pair of X and Y in the context of {{context}}, what answer is Y implying?

X: {{question_X}} 

Y: {{answer_Y}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{   answer_choices[goldstandard1]}}

{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if goldstandard1 != -1 %}

Given the question-answer pair of X and Y in the context of {{context}}, which of the following answers is Y implying: "{{"Yes"}}", "{{"No"}}", "{{"In the middle, neither yes nor no"}}", "{{"Probably yes / sometimes yes"}}", "{{"Probably no"}}", "{{"Yes, subject to some conditions"}}", "{{"Other"}}" or "{{"I am not sure how X will interpret Y’s answer"}}" ?

X: {{question_X}} 

Y: {{answer_Y}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{   answer_choices[goldstandard1]}}

{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{mc\_taco}
\noindent Dataset from \citet{ZKNR19}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ she was ill for 30 seconds + \\
	 category & \verb+ 0 + \\
	 label & \verb+ 0 + \\
	 question & \verb+ How long was his mother ill? + \\
	 sentence & \verb+ Durer's father died in 1502, and his mother died i... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given the context,

{{sentence}}

observe the following QA pair and check if the answer is plausible:

Question: {{question}}

Answer: {{answer}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
I've been grappling with the temporal accuracy of this answer for a while:

Q: "{{question}}"

I have the following information: "{{sentence}}"

A: "{{answer}}" 

This answer is definitely not
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
There are five temporal categories: {{"Event Duration"}}, {{"Event Ordering"}}, {{"Frequency"}}, {{"Typical Time"}}, {{"Stationarity"}}.

Out of the above temporal categories, which one does the question "{{question}}" belong to?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[category]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label %}
I have the following passage:

{{sentence}}

My query is: "{{question}}"

I want an answer that is "temporally plausible".
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Here's what happened: {{sentence}}

I asked my friend {{question}}

and they said {{answer}}

Should I believe them?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given the context, the question, and the candidate answer, the task is to determine whether the candidate answer is plausible ("yes") or not ("no").

Context: {{sentence}}

Question: {{question}}

Candidate answer: {{answer}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given the context,

{{sentence}}

and the question,

{{question}}

is the following answer believable?

{{answer}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
True/False?

"{{answer}}" is a plausible answer to "{{question}}", given "{{sentence}}"
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Which temporal category does the question "{{question}}" belong to?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[category]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Here's what happened: {{sentence}}

I asked my friend {{question}}

and they said {{answer}}

Should I doubt them?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{piqa}
\noindent Dataset from \citet{Bisk2020}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 goal & \verb+ When boiling butter, when it's ready, you can + \\
	 label & \verb+ 1 + \\
	 sol1 & \verb+ Pour it onto a plate + \\
	 sol2 & \verb+ Pour it into a jar + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{sol1}} ||| {{sol2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Goal: {{goal}}

Which is the correct ending?
- {{sol1}}
- {{sol2}}

Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{sol1}} ||| {{sol2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{"Solution 1"}}: {{sol1}}
{{"Solution 2"}}: {{sol2}}

Goal: {{goal}}

Given the goal, what is the correct solution?

Answer by copying the correct solution
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Sentence: {{goal}}

Choice {{answer_choices[0]}}: {{sol1}}

Choice {{answer_choices[1]}}: {{sol2}}

What is the index of the correct choice for ending for the sentence?

Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given a goal and a wrong solution, rewrite it to give a correct solution.
Goal: {{goal}} 
Solution: {{[sol1, sol2][1 - label]}}
Corrected solution:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{[sol1, sol2][label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{sol1}} ||| {{sol2}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Finish the following sentence with the best choice: {{goal}}

Choices:
- {{sol1}}
- {{sol2}}

Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{goal}} {{sol2}}
Does this phrase make sense?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given a goal and 2 solutions, choose the most appropriate solution.
Goal: {{goal}}
- {{"Solution 1"}}: {{sol1}}
- {{"Solution 2"}}: {{sol2}}

Answer by returning either {{"Solution 1"}} or {{"Solution 2"}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given a sentence, correct it if it doesn't make sense. If it makes sense, just return it as the answer.
Input: {{goal}} {{sol2[0].lower() + sol2[1:]}}
Output:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{goal}} {{[sol1[0].lower() + sol1[1:], sol2[0].lower() + sol2[1:]][label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{goal}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{[sol1[0].lower() + sol1[1:], sol2[0].lower() + sol2[1:]][label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Does this phrase make sense?
{{goal}} {{sol1[0].lower() + sol1[1:]}}
Answer with {{answer_choices[0]}} or {{answer_choices[1]}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Sentence: {{goal}} {{sol1[0].lower() + sol1[1:]}}
If the sentence does not make sense, correct it so that it does make sense. Otherwise, just copy it.
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{goal}} {{[sol1[0].lower() + sol1[1:], sol2[0].lower() + sol2[1:]][label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Sentiment }
\subsubsection{amazon\_polarity}
\noindent Dataset from \citet{mcauley2013hidden}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 content & \verb+ This sound track was beautiful! It paints the sene... + \\
	 label & \verb+ 1 + \\
	 title & \verb+ Stuning even for the non-gamer + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Title: {{title}}
Review: {{content}}
Is the review positive or negative?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Based on this review, would the user recommend this product?
===
Review: {{content}}
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Is this product review positive?
Title: {{title}}
Review: {{content}}
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Title: {{title}}
Review: {{content}}
Is this product review negative?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Title: {{title}}
Review: {{content}}
Does this product review convey a negative or positive sentiment?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Is there a negative or positive tone to this product review?
===
Title: {{title}}
Review: {{content}}
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Title: {{title}}
Product review: {{content}}
Would you say this review depicts the product in a {{answer_choices[1]}} or {{answer_choices[0]}} light?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
You are considering whether to buy a product. You look at the reviews. Would the following review {{answer_choices[0]}} or {{answer_choices[1]}} the chances of you buying the product?
Review title: {{title}}
Product review: {{content}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Here is a review left by a customer on a product. Would you say he was {{answer_choices[1]}} or {{answer_choices[0]}}?
Title: {{title}}
Review: {{content}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{app\_reviews}
\noindent Dataset from Zurich Open Repository and
Archive.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 date & \verb+ October 12 2016 + \\
	 package\_name & \verb+ com.mantz_it.rfanalyzer + \\
	 review & \verb+ Great app! The new version now works on my Bravia ... + \\
	 star & \verb+ 4 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given this review: "{{review}}"
Would you recommend this app to a friend? {{answer_choices[0]}}, {{answer_choices[1]}}, {{answer_choices[2]}}, {{answer_choices[3]}}, or {{answer_choices[4]}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[star-1]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Generate a {{star}}-star review (1 being lowest and 5 being highest) about an app with package {{package_name}}.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{review}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
What would be the *-rating of this review (* being the lowest and ***** being the highest)? "{{review}}"
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[star-1]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
On a scale of 1-5 (with 1 being least favorable and 5 being most favorable), how would you rate this review? "{{review}}"
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{star}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{imdb}
\noindent Dataset from \citet{maas-EtAl:2011:ACL-HLT2011}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 text & \verb+ Bromwell High is a cartoon comedy. It ran at the s... + \\
	 label & \verb+ 1 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
The following movie review expresses what sentiment? {{text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} Did the reviewer find this movie {{"good or bad"}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} 
Is this review {{"positive or negative"}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} How does the viewer feel about the movie?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} What sentiment does the writer express for the movie?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} The sentiment expressed for the movie is
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} What is the sentiment expressed in this text?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} This is definitely not a
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [1-label]}} review.
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} Did the reviewer enjoy the movie?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} What is the sentiment expressed by the reviewer for the movie?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} How does the reviewer feel about the movie?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{rotten\_tomatoes}
\noindent Dataset from \citet{Pang+Lee:05a}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 text & \verb+ the rock is destined to be the 21st century's new ... + \\
	 label & \verb+ 1 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} Did the reviewer find this movie {{"good or bad"}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} What is the sentiment expressed in this text?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} 
Is this review {{"positive or negative"}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} Did the reviewer enjoy the movie?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} How does the reviewer feel about the movie?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} The sentiment expressed for the movie is
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} What sentiment does the writer express for the movie?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
The following movie review expresses what sentiment? {{text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} What is the sentiment expressed by the reviewer for the movie?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} How does the viewer feel about the movie?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{yelp\_review\_full}
\noindent Dataset from \citet{zhang2015character}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 label & \verb+ 4 + \\
	 text & \verb+ dr. goldberg offers everything i look for in a gen... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ text }}
So I would like to give it
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ text }}
===
Based on that, my rating is
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Review text:
{{ text }}

Stars:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ text }} My rating for this place is
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Review text:
{{ text }}

Review score (between 1 and 5):
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Review: {{text}}
On a scale of 1 to 5, I would give this product
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Review text:
{{ text }}

Review rating:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Story Completion }
\subsubsection{hellaswag}
\noindent Dataset from \citet{zellers2019hellaswag}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 activity\_label & \verb+ Removing ice from car + \\
	 ctx & \verb+ Then, the man writes over the snow covering the wi... + \\
	 ctx\_a & \verb+ Then, the man writes over the snow covering the wi... + \\
	 ctx\_b & \verb+ then + \\
	 endings & \verb+ [', the man adds wax to the windshield and cuts it... + \\
	 ind & \verb+ 4 + \\
	 label & \verb+ 3 + \\
	 source\_id & \verb+ activitynet~v_-1IBHYS3L-Y + \\
	 split & \verb+ train + \\
	 split\_type & \verb+ indomain + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{endings | join(" ||| ")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Complete the description with an appropriate ending:
First, {{ ctx_a.lower() }} Then, {{ ctx_b.lower() }} ...

(a) {{ answer_choices[0] }}

(b) {{ answer_choices[1] }}

(c) {{ answer_choices[2] }}

(d) {{ answer_choices[3] }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label | int()] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
What is the topic of the sentence: {{ctx}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{activity_label}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{endings | join(" ||| ")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Complete the sentence: {{ctx}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label | int()]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ctx}} {{endings[label | int()]}}
Can you identify the topic of the paragraph?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{activity_label}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{endings | join(" ||| ") }}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set prompts = [
'Can you pick the correct ending for the sentence: ',
'The task is to generate the ending for the sentence: ',
'How does this sentence end? ',
'From the list of endings described below, what ending makes the most sense for the sentence ',]
%}
{{prompts | choice}}
{{ctx}}

(a)  {{answer_choices[0]}}

(b)  {{answer_choices[1]}}

(c)  {{answer_choices[2]}}

(d)  {{answer_choices[3]}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices [label | int()]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set instance = [0, 1, 2, 3] | choice %}
Consider the following description: {{ ctx_a }}
Is the following an appropriate continuation?
{{ ctx_b }} {{ endings[instance] }}
Yes or No?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label  == instance | string() %}
{{answer_choices[0]}}
{% else %} 
{{answer_choices[1]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{endings | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
How does this sentence end?
{{ctx}}

(a)  {{answer_choices[0]}}

(b)  {{answer_choices[1]}}

(c)  {{answer_choices[2]}}

(d)  {{answer_choices[3]}}

Hint: the topic of the sentence is {{activity_label}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices [label | int()]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
How would you start the sentence:
{{endings[label | int()]}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ctx}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set instance = [0, 1, 2, 3] | choice %}
Consider the following text: {{ ctx_b }} {{ endings[instance] }}
Is it an appropriate continuation of the following text: 
{{ ctx_a }} ?
Yes or No?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label  == instance | string() %}
{{answer_choices[0]}}
{% else %} 
{{answer_choices[1]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{ ctx }}...
How does the description likely end?

Ending 1: {{ endings[0] }}

Ending 2: {{ endings[1] }}

Ending 3: {{ endings[2] }}

Ending 4: {{ endings[3] }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label | int()] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
If a description of a situation begins like this: {{ ctx }}... Then how
does it continue? 

Ending 1: {{ endings[0] }}

Ending 2: {{ endings[1] }}

Ending 3: {{ endings[2] }}

Ending 4: {{ endings[3] }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label | int()] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Structure To Text }
\subsubsection{common\_gen}
\noindent Dataset from \citet{lin-etal-2020-commongen}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 concept\_set\_idx & \verb+ 0 + \\
	 concepts & \verb+ ['ski', 'mountain', 'skier'] + \\
	 target & \verb+ Skier skis down the mountain + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Ignoring the order of the concepts: {{ concepts | join(", ") }}; 
Generate a sentence with all the concepts :
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Put the concepts together to form a sentence: {{ concepts | join(", ") }}.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Construct a sentence with the word {{ concepts | choice }}. 

Hint: Use {{concepts | join(", ")}} to restrict the output sentence.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set seq = [ 
'From the concepts mentioned below, generate a sentence:', 
'Convert the concepts to a sentence:', 
'Given the list of concepts, write a sentence:'
] %} 
{{ seq | choice }}
{{ concepts | join(", ") }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
What are the topics in the sentence: {{target}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ concepts | join(", ") }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
We have the sentence: {{target}}; 
Extract all the key concepts:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ concepts | join(", ") }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Can you write a sentence about the topic {{concepts | choice}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Humans can easily string together abstract concepts to form a coherent sentence. 
For example, with the concepts {{ concepts | join(", ") }}, a simple sentence can be
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Given the list of concepts: {{ concepts | join(", ") }}; 
Generate a sentence with all the concepts :
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{wiki\_bio}
\noindent Dataset from \citet{DBLP:journals/corr/LebretGA16}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 input\_text & \verb+ {'table': {'column_header': ['name', 'nationality'... + \\
	 target\_text & \verb+ walter extra is a german award-winning aerobatic p... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Facts:
{% for n in range (input_text["table"]["column_header"]|length) %}
{% if input_text["table"]["column_header"][n] != "article_title" %}
- {{input_text["table"]["column_header"][n].replace("_"," ") }}: {{input_text["table"]["content"][n] }}
{% endif %}
{% endfor %}
Based on these bullet points, write a short biography describing the life of {{input_text["context"]}}.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target_text}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Read the bio below and try to give details on {{input_text["context"]}}'s: 
{% for n in range (input_text["table"]["column_header"]|length) %} {% if input_text["table"]["column_header"][n] != "article_title" %}
- {{ input_text["table"]["column_header"][n].replace("_"," ") }} 
{% endif %} {% endfor %}

Bio: {{target_text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for n in range (input_text["table"]["column_header"]|length) %}
{% if input_text["table"]["column_header"][n] != "article_title" %}
- {{ input_text["table"]["column_header"][n].replace("_"," ") }} is {{ input_text["table"]["content"][n] }}
{% endif %}
{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
What type of details about {{input_text["context"]}} can be gathered from the following bio?

Bio: {{target_text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for n in range (input_text["table"]["column_header"]|length) %}
{% if input_text["table"]["column_header"][n] != "article_title" %}
- {{ input_text["table"]["column_header"][n].replace("_"," ") }} 
{% endif %}
{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% for n in range (input_text["table"]["column_header"]|length) %}
{% if input_text["table"]["column_header"][n] != "article_title" and input_text["table"]["column_header"][n] !="name" %}
- {{ input_text["table"]["column_header"][n].replace("_"," ") }} is {{ input_text["table"]["content"][n] }}
{% endif %}
{% endfor %}

Given the details above, guess who could this information be about.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{input_text["context"]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
What key details about {{input_text["context"]}} can be extracted from the following bio?

Bio: {{target_text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for n in range (input_text["table"]["column_header"]|length) %}
{% if input_text["table"]["column_header"][n] != "article_title" %}
- {{ input_text["table"]["column_header"][n].replace("_"," ") }} is {{ input_text["table"]["content"][n] }}
{% endif %}
{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Summarization }
\subsubsection{cnn\_dailymail 3.0.0}
\noindent Dataset from \citet{DBLP:journals/corr/SeeLM17}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 article & \verb+ It's official: U.S. President Barack Obama wants l... + \\
	 highlights & \verb+ Syrian official: Obama climbed to the top of the t... + \\
	 id & \verb+ 0001d1afc246a7964130f43ae940af6bc6c57f01 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Can you write an outline of the following article in a few points?

Article: {{article}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{highlights}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Summarise the article:

{{article}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{highlights}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
In 2 or 3 sentences, what are the main points one should remember from this news article?

Article: {{article}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{highlights}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Could you please generate a TLDR (Too Long Didn't Read) summary of the following news article?

Article: {{article}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{highlights}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Condense the article down to the essentials to present it in the form of short cards in mobile news apps:

{{article}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{highlights}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Generate a story from key plot points:

{{highlights}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{article}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Sum the following article in brief: {{article}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{highlights}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Extract key points from the article based on which the stock market could react:

{{article}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{highlights}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
What details would you include in a storyline to make it more engaging and informative?

{{highlights}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{article}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{gigaword}
\noindent Dataset from \citet{graff2003english}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 document & \verb+ australia 's current account deficit shrunk by a r... + \\
	 summary & \verb+ australian current account deficit narrows sharply + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{document}}

===

Generate a title for this article:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Title: {{summary}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{document}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Make a title for this article: {{document}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
First sentence of the article: {{document}}

Title:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{radford2019language}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{document}}

TL;DR:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{document}}

===

Given the above sentence, write its title:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Write a title for this sentence: {{document}} 

Title:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{document}} In a nutshell,
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Title: {{summary}}

===

Write an article with the given title:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{document}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{multi\_news}
\noindent Dataset from \citet{alex2019multinews}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 document & \verb+ National Archives  Yes, it’s that time again, ... + \\
	 summary & \verb+ – The unemployment rate dropped to 8.2% last month... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set docs = document.split("3ed2dface8203c4c9dfb1a5dc58e41e0||") | reject("equalto", "") | list %}
What are the key points across these news articles:
{% for doc in docs %}

Article: {{doc}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary[2:]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set docs = document.split("3ed2dface8203c4c9dfb1a5dc58e41e0||") | reject("equalto", "") | list %}
Synthesize these documents into a single one:
{% for doc in docs %}

- {{doc}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary[2:]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set docs = document.split("3ed2dface8203c4c9dfb1a5dc58e41e0||") | reject("equalto", "") | list %}
I want to edit the following articles into a more concise summary:
{% for doc in docs %}

Article: {{doc}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary[2:]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set docs = document.split("3ed2dface8203c4c9dfb1a5dc58e41e0||") | reject("equalto", "") | list %}
Write a summary of the following articles:
{% for doc in docs %}

Document: {{doc}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary[2:]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set docs = document.split("3ed2dface8203c4c9dfb1a5dc58e41e0||") | reject("equalto", "") | list%}
Write an expanded news article with plausible details from the following summary:
{{summary[2:]}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{docs | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set docs = document.split("3ed2dface8203c4c9dfb1a5dc58e41e0||") | reject("equalto", "") | list %}
I'm trying to distill these articles down into one:
{% for doc in docs %}

Article: {{doc}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary[2:]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{samsum}
\noindent Dataset from \citet{gliwa2019samsum}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 dialogue & \verb+ Amanda: I baked  cookies. Do you want some? Jerry... + \\
	 id & \verb+ 13818513 + \\
	 summary & \verb+ Amanda baked cookies and will bring Jerry some tom... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Summarize this dialogue: {{dialogue}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{dialogue}}
Given the above dialogue, write a summary.
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Summarize: {{dialogue}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{dialogue}}
To sum up this dialog:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Generate a summary for this dialogue:
{{dialogue}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Write a dialogue that matches this summary: {{summary}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{dialogue}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Sum up the following dialogue: 
{{dialogue}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{xsum}
\noindent Dataset from \citet{Narayan2018DontGM}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 document & \verb+ Recent reports have linked some France-based playe... + \\
	 id & \verb+ 29750031 + \\
	 summary & \verb+ New Welsh Rugby Union chairman Gareth Davies belie... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{document}}

===

Write a summary of the text above :
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Article: {{document}}

Summary:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{wikidotgpt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{document}}
How would you rephrase that in a few words?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{wikidotgpt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
My college roommate asked me what this article means:

{{document}}

So I recapped it in layman's terms:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{wikidotgpt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{document}}
This boils down to the simple idea that
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Summarize: {{document}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Summarize this document: {{document}}
Summary:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{document}}

===

Given the above document, write one sentence to summarize:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
First, please read the article below.

{{document}}

Now, can you write me an extremely short abstract for it?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{radford2019language}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{document}}

TL;DR:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Topic Classification }
\subsubsection{ag\_news}
\noindent Dataset from \citet{Zhang2015CharacterlevelCN}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 text & \verb+ Wall St. Bears Claw Back Into the Black (Reuters) ... + \\
	 label & \verb+ 2 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
What label best describes this news article?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Is this a piece of news regarding {{"world politics, sports, business, or science and technology"}}?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Would you recommend the following article to a {{"politician"}}, an {{"athlete"}}, a {{"business executive"}}, or a {{"scientist"}}?

{{ text }}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} 

Which of the following sections of a newspaper would this article likely appear in? {{"World News"}}, {{"Sports"}}, {{"Business"}}, or {{"Science and Technology"}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} 

Which section of a newspaper would this article likely appear in?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} 
Is this a piece of news regarding {{"world politics, sports, business, or science and technology"}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}} 
What label best describes this news article?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{dbpedia\_14}
\noindent Dataset from \citet{lehmann2015dbpedia}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 content & \verb+  Abbott of Farnham E D Abbott Limited was a Britis... + \\
	 label & \verb+ 0 + \\
	 title & \verb+ E. D. Abbott Ltd + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{content}} Given a list of categories: {{"company, educational institution, artist, athlete, office holder, mean of transportation, building, natural place, village, animal, plant, album, film or written work"}}, what category does the paragraph belong to?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Pick one category for the following text. The options are - {{"company, educational institution, artist, athlete, office holder, mean of transportation, building, natural place, village, animal, plant, album, film or written work"}}. {{title}} - {{content}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{title}} - {{content}} Given a choice of categories {{"company, educational institution, artist, athlete, office holder, mean of transportation, building, natural place, village, animal, plant, album, film or written work"}}, the text refers to which one?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
"{{title}}", given a list of categories: {{"company, educational institution, artist, athlete, office holder, mean of transportation, building, natural place, village, animal, plant, album, film or written work"}}, what category does the title belong to?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{trec}
\noindent Dataset from \citet{li-roth-2002-learning}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 label-coarse & \verb+ 0 + \\
	 label-fine & \verb+ 0 + \\
	 text & \verb+ How did serfdom develop in and then leave Russia ? + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Categories: {{', '.join(answer_choices)}}

What category best describes: {{text}} 
Answer:
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_coarse] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set label_mapping = {21:0, 18:1, 24:2, 11:3, 14:4} %}
{% if label_coarse == 5 %}
Is this question asking for {{', '.join(answer_choices)}}?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set label_mapping = {39:0, 13:1, 8:2, 40:3, 25:4, 43:5, 27:6, 38:7, 35:8, 41:9, 32:10, 45:11, 14:12} %}
{% if label_coarse == 4 %}
{{text}}

Is this question asking for {{', '.join(answer_choices)}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set label_mapping = {2:0, 22:1, 19:2, 1:3, 46:3, 23:4, 10:5, 17:6, 33:7, 37:8, 15:9, 30:10, 26:11, 16:12, 28:13, 42:14, 31:15, 20:16, 44:17, 36:18, 14:19} %}
{% if label_coarse == 1 %}
Is this question asking for {{', '.join(answer_choices)}}?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set label_mapping = {39:0, 13:1, 8:2, 40:3, 25:4, 43:5, 27:6, 38:7, 35:8, 41:9, 32:10, 45:11, 14:12} %}
{% if label_coarse == 4 %}
Is this question asking for {{', '.join(answer_choices)}}?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Question: {{text}}

Descriptors: {{', '.join(answer_choices)}}

Best Descriptor?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label_coarse]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}}

What is this question asking for?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label_fine] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set label_mapping = {21:0, 18:1, 24:2, 11:3, 14:4} %}
{% if label_coarse == 5 %}
{{text}}

Is this question asking for {{', '.join(answer_choices)}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Which category best describes the following question: {{text}} 

Choose from the following list: 
{{', '.join(answer_choices)}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_coarse] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set label_mapping={0:2, 7:1,  12:0, 9:3} %}
{% if label_coarse == 0 %}
Is this question asking for {{', '.join(answer_choices)}}?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{{text}}

Is this asking about {{(', ').join(answer_choices)}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_coarse] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set label_mapping={34:0, 3:1} %} 
{% if label_coarse == 2 %}
Is this question asking for an {{', '.join(answer_choices)}}?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set label_mapping = {34:0, 3:1} %} 
{% if label_coarse == 2 %}
{{text}}

Is this question asking for an {{', '.join(answer_choices)}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
Is the following question asking about {{', '.join(answer_choices)}}?

{{text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_coarse] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set label_mapping = {5:0, 4:1, 6:2, 12:3} %}
{% if label_coarse == 3 %}
Is this question asking for {{', '.join(answer_choices)}}?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
What is this question asking for?

{{text}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label_fine] }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set label_mapping = {5:0, 4:1, 6:2, 12:3} %}
{% if label_coarse == 3 %}
{{text}}

Is this question asking for {{', '.join(answer_choices)}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt not from the original task.}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% set label_mapping={0:2, 7:1,  12:0, 9:3} %}
{% if label_coarse == 0 %}
{{text}}

Is this question asking for {{', '.join(answer_choices)}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Word Sense Disambiguation }
\subsubsection{super\_glue wic}
\noindent Dataset from \citet{DBLP:journals/corr/abs-1808-09121}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 end1 & \verb+ 36 + \\
	 end2 & \verb+ 32 + \\
	 idx & \verb+ 0 + \\
	 label & \verb+ 0 + \\
	 sentence1 & \verb+ Do you want to come over to my place later? + \\
	 sentence2 & \verb+ A political system with no place for the less prom... + \\
	 start1 & \verb+ 31 + \\
	 start2 & \verb+ 27 + \\
	 word & \verb+ place + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1%}
Does the word "{{word}}" have the same meaning in these two sentences? Yes, No?
{{sentence1}}
{{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1%}
Does the word "{{word}}" have the same meaning in these two sentences?
{{sentence1}}
{{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1%}
Homework

Decide whether the word "{{word}}" is used with the same meaning in the two following sentences. Answer by yes or no.
{{sentence1}}
{{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1%}
Sentence A: {{sentence1}}
Sentence B: {{sentence2}}

"{{word}}" has a similar meaning in sentences A and B. True or False?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1%}
{{sentence1}}
{{sentence2}}
Question: Is the word '{{word}}' used in the same sense in the two sentences above?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1%}
Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}

Determine whether the word "{{word}}" is used in the same sense in both sentences. Yes or no?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1%}
Determine if the word '{{word}}' is used in the same way in the two sentences below. 
{{sentence1}}
{{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1%}
{{sentence1}}
{{sentence2}}
Question: Is the word '{{word}}' used in the same sense in the two sentences above? Yes, No?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1%}
The word "{{word}}" has multiple meanings. Does it have the same meaning in sentences 1 and 2? Yes or no?

Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small]{django}
{% if label != -1%}
{{sentence1}}
{{sentence2}}
Similar sense of {{word}}?
\end{minted}
\vspace*{-0.2cm}

\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}


==> promptgen2.tex <==
\subsection{Bias And Fairness }
\subsubsection{crows\_pairs}
\noindent Dataset from \citet{nangia2020crows}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ 0 + \\
	 sent\_more & \verb+ He couldn't figure out the issue with the rope, bu... + \\
	 sent\_less & \verb+ He couldn't figure out the issue with the rope, bu... + \\
	 stereo\_antistereo & \verb+ 0 + \\
	 bias\_type & \verb+ 0 + \\
	 annotations & \verb+ [[0], [0], [0], [0], [0]] + \\
	 anon\_writer & \verb+ a0 + \\
	 anon\_annotators & \verb+ ['a77', 'a78', 'a79', 'a80', 'a81'] + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
You are presented with two very similar sentences:
A: {{sent_more}}
B: {{sent_less}}
Sentence A is illustrating a stereotype. Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[stereo_antistereo]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Sentence A: {{sent_more}}
Sentence B: {{sent_less}}
Select the option that is the most plausible:
- {{answer_choices[0]}}
- {{answer_choices[1]}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[stereo_antistereo]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Sentence A demonstrates a stereotype ||| Sentence B violates a stereotype
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if stereo_antistereo == 0 %}
"{{sent_more}}"
The previous sentence illustrates a stereotype against a historically disadvantaged group in the US. Minimally modify the previous sentence to a less stereotypical sentence involving a contrasting advantaged group.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{sent_less}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
A: {{sent_more}}
B: {{sent_less}}
I believe sentence A is conveying a stereotype. Is that correct? Answer with yes or no.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[stereo_antistereo]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
You are presented with two very similar sentences:
A: {{sent_more}}
B: {{sent_less}}
Sentence B is illustrating an anti-stereotype. Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[stereo_antistereo]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if stereo_antistereo == 1 %}
"{{sent_less}}"
The previous sentence violates a stereotype against a historically disadvantaged group in the US. Minimally modify the previous sentence to a less stereotypical sentence involving a contrasting advantage group.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{sent_more}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Sentence 1: {{sent_more}}
Sentence 2: {{sent_less}}
I think that Sentence 2 conveys an anti-stereotype. Is that correct? Answer yes or no.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[stereo_antistereo]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Here are two sentences. One is more stereotypical than the other. What kind of stereotypes are these two sentences illustrating? Choose between {{answer_choices | join(", ") | lower}}.
Sentence 1: {{sent_more}}
Sentence 2: {{sent_less}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[bias_type]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Race and color ||| Socioeconomic status and occupation ||| Gender and gender identity ||| Disability ||| Nationality ||| Sexual orientation ||| Physical appearance ||| Religion ||| Age
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{super\_glue axg}
\noindent Dataset from \citet{rudinger-EtAl:2018:N18}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 premise & \verb+ The taxpayer met with the accountant to get help f... + \\
	 hypothesis & \verb+ The accountant sought help filing taxes. + \\
	 idx & \verb+ 0 + \\
	 label & \verb+ 1 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given {{premise}} Should we assume that "{{hypothesis}}" is true? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} 

Question: Does this imply that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} Based on the previous passage, is it true that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given that {{premise}} Therefore, it must be true that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}}
Question: {{hypothesis}} True or False?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
True ||| False
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given {{premise}} Is it guaranteed true that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given that {{premise}} Does it follow that {{hypothesis}} Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} Are we justified in saying that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Suppose {{premise}} Can we infer that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{N18-1101}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} Using only the above description and what you know about the world, is "{{hypothesis}}" definitely correct? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Coreference }
\subsubsection{super\_glue wsc.fixed}
\noindent Dataset from \citet{levesque2012winograd}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 idx & \verb+ 0 + \\
	 label & \verb+ 0 + \\
	 span1\_index & \verb+ 0 + \\
	 span1\_text & \verb+ Mark + \\
	 span2\_index & \verb+ 13 + \\
	 span2\_text & \verb+ He + \\
	 text & \verb+ Mark told Pete many lies about himself, which Pete... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ text }} In the previous sentence, does the pronoun "{{ span2_text.lower() }}" refer to {{ span1_text }}? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ text }} Here, by "{{ span2_text }}" they mean "{{ span1_text }}". Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ text }} 

In other words, {{ text.split(" ")[span2_index:] | join(" ") | replace(span2_text, span1_text) }} True or false?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
False ||| True
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ text }} I think they mean "{{ text.split(" ")[span2_index:] | join(" ") | replace(span2_text, span1_text) }}" Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ text }} Here, does "{{ span2_text.lower() }}" stand for {{ span1_text }}? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Passage: {{ text }} 

Question: In the passage above, does the pronoun "{{ span2_text }}" refer to {{ span1_text }}?

Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ text }} In the previous sentence, can the pronoun "{{ span2_text }}" be replaced with "{{ span1_text }}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Context: {{ text }} 

{% if span2_text.lower()  == "they" or span2_text.lower() == "them" %}
Question: "{{ span2_text }}" are {{ span1_text }}. True or false?
{% else %}
Question: "{{ span2_text }}" is {{ span1_text }}. True or false?
{% endif %}

Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
False ||| True
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ text }} 
In the passage above, the pronoun "{{ span2_text }}" refers to {{ span1_text }}. True or false?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
False ||| True
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ text }} 
{% if span2_text.lower()  == "they" or span2_text.lower() == "them" %}
Question: Who or what are "{{ span2_text.lower() }}"? {{ span1_text }}?
{% else %}
Question: Who or what is "{{ span2_text.lower() }}"? Is it {{ span1_text }}?
{% endif %}
Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{winogrande winogrande\_xl}
\noindent Dataset from \citet{ai2:winogrande}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ 2 + \\
	 option1 & \verb+ Ian + \\
	 option2 & \verb+ Dennis + \\
	 sentence & \verb+ Ian volunteered to eat Dennis's menudo after alrea... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ sentence }} In the previous sentence, does _ refer to {{ option1 }} or  {{ option2 }}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer == '1' %} {{option1}} {% else %} {{ option2 }} {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ option1 }} ||| {{ option2 }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
In the sentence below, does the _ stand for {{answer_choices[0]}} or {{answer_choices[1]}}?
{{sentence}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer | int - 1]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{option1}} ||| {{option2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{sentence}}
What does the _ in the above sentence refer to? {{ option1 }} or {{ option2 }}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer == '1' %} {{option1}} {% else %} {{ option2 }} {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{option1}} ||| {{option2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Fill in the _ in the below sentence:
{{sentence}}

Choices:
- {{ option1 }}
- {{ option2 }}

Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer == '1' %} {{option1}} {% else %} {{ option2 }} {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{option1}} ||| {{option2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
The _ in the sentence below refers to {{option1}}. True or False?
{{sentence}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer|int - 1]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
True ||| False
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{sentence}}
Replace the _ in the above sentence with the correct option: 
- {{option1}}
- {{option2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer == '1' %} {{option1}} {% else %} {{ option2 }} {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{option1}} ||| {{option2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{NLI }
\subsubsection{super\_glue cb}
\noindent Dataset from \citet{de marneff_simons_tonhauser_2019}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 hypothesis & \verb+ the language was peeled down + \\
	 idx & \verb+ 0 + \\
	 label & \verb+ 0 + \\
	 premise & \verb+ It was a complex language. Not written down but ha... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Suppose {{premise}} Can we infer that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No ||| Maybe
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} Based on the previous passage, is it true that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No ||| Maybe
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} Based on that information, is the claim: "{{hypothesis}}" {{"true"}}, {{"false"}}, or {{"inconclusive"}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
True ||| False ||| Inconclusive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given that {{premise}} Does it follow that {{hypothesis}} Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No ||| Maybe
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} Are we justified in saying that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No ||| Maybe
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Suppose it's true that {{premise}} Then, is "{{hypothesis}}" {{"always"}}, {{"sometimes"}}, or {{"never"}} true?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Always ||| Never ||| Sometimes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}}
Question: {{hypothesis}} True, False, or Neither?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
True ||| False ||| Neither
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} 

Keeping in mind the above text, consider: {{hypothesis}} Is this {{"always"}}, {{"sometimes"}}, or {{"never"}} correct?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Always ||| Never ||| Sometimes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given {{premise}} Is it guaranteed true that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No ||| Maybe
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given that {{premise}} Therefore, it must be true that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No ||| Maybe
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Assume it is true that {{premise}} 

Therefore, "{{hypothesis}}" is {{"guaranteed"}}, {{"possible"}}, or {{"impossible"}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Guaranteed ||| Impossible ||| Possible
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} 

Question: Does this imply that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{answer_choices[label]}}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No ||| Maybe
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{N18-1101}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} Using only the above description and what you know about the world, "{{hypothesis}}" is definitely correct, incorrect, or inconclusive?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Correct ||| Incorrect ||| Inconclusive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given {{premise}} Should we assume that "{{hypothesis}}" is true? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No ||| Maybe
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Take the following as truth: {{premise}}
Then the following statement: "{{hypothesis}}" is {{"true"}}, {{"false"}}, or {{"inconclusive"}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label !=-1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
True ||| False ||| Inconclusive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{super\_glue rte}
\noindent Dataset from \citet{dagan2005pascal}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 hypothesis & \verb+ Weapons of Mass Destruction Found in Iraq. + \\
	 idx & \verb+ 0 + \\
	 label & \verb+ 1 + \\
	 premise & \verb+ No Weapons of Mass Destruction Found in Iraq Yet. + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt from \cite{N18-1101}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} Using only the above description and what you know about the world, is "{{hypothesis}}" definitely correct? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given {{premise}} Is it guaranteed true that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Suppose {{premise}} Can we infer that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}}
Question: {{hypothesis}} True or False?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
True ||| False
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} 

Question: Does this imply that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{answer_choices[label]}}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given {{premise}} Should we assume that "{{hypothesis}}" is true? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given that {{premise}} Does it follow that {{hypothesis}} Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} Based on the previous passage, is it true that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} Are we justified in saying that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given that {{premise}} Therefore, it must be true that "{{hypothesis}}"? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{anli}
\noindent Dataset from \citet{nie2019adversarial}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 hypothesis & \verb+ The trolleybus system has over 2 urban routes + \\
	 label & \verb+ 0 + \\
	 premise & \verb+ The Parma trolleybus system (Italian: "Rete filovi... + \\
	 reason & \verb+  + \\
	 uid & \verb+ 0fd0abfb-659e-4453-b196-c3a64d2d8267 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small Prompt from \cite{N18-1101}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} Using only the above description and what you know about the world, "{{hypothesis}}" is definitely correct, incorrect, or inconclusive?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Correct ||| Inconclusive ||| Incorrect
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given {{premise}} Should we assume that "{{hypothesis}}" is true? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| Maybe ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given that {{premise}} Does it follow that {{hypothesis}} Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| Maybe ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}}
Question: {{hypothesis}} True, False, or Neither?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
True ||| Neither ||| False
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} Based on the previous passage, is it true that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| Maybe ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} Are we justified in saying that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| Maybe ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Take the following as truth: {{premise}}
Then the following statement: "{{hypothesis}}" is {{"true"}}, {{"false"}}, or {{"inconclusive"}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
True ||| Inconclusive ||| False
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given that {{premise}} Therefore, it must be true that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| Maybe ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Suppose {{premise}} Can we infer that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| Maybe ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Assume it is true that {{premise}} 

Therefore, "{{hypothesis}}" is {{"guaranteed"}}, {{"possible"}}, or {{"impossible"}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Guaranteed ||| Possible ||| Impossible
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Suppose it's true that {{premise}} Then, is "{{hypothesis}}" {{"always"}}, {{"sometimes"}}, or {{"never"}} true?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Always ||| Sometimes ||| Never
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} 

Question: Does this imply that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| Maybe ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} 

Keeping in mind the above text, consider: {{hypothesis}} Is this {{"always"}}, {{"sometimes"}}, or {{"never"}} correct?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Always ||| Sometimes ||| Never
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{premise}} Based on that information, is the claim: "{{hypothesis}}" {{"true"}}, {{"false"}}, or {{"inconclusive"}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
True ||| Inconclusive ||| False
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{webson-pavlick-2021}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given {{premise}} Is it guaranteed true that "{{hypothesis}}"? Yes, no, or maybe?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| Maybe ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Paraphrase }
\subsubsection{glue mrpc}
\noindent Dataset from \citet{dolan2005automatically}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 idx & \verb+ 0 + \\
	 label & \verb+ 1 + \\
	 sentence1 & \verb+ Amrozi accused his brother , whom he called " the ... + \\
	 sentence2 & \verb+ Referring to him as only " the witness " , Amrozi ... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if label == 1 %}
Paraphrase the following sentence: {{sentence1}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{sentence2}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I want to know whether the following two sentences mean the same thing.
{{sentence1}}
{{sentence2}}
Do they?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
no ||| yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Does the sentence
{{sentence1}}
paraphrase (that is, mean the same thing as) this sentence?
{{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
no ||| yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Are the following two sentences "{{"equivalent"}}" or "{{"not equivalent"}}"?
{{sentence1}}
{{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
not equivalent ||| equivalent
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if label == 1 %}
Generate a sentence that means the same thing as this one: {{sentence1}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{sentence2}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Can I replace the sentence
{{sentence1}}
with the sentence
{{sentence2}}
and have it mean the same thing?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
no ||| yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Do the following two sentences mean the same thing?
{{sentence1}}
{{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
no ||| yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{glue qqp}
\noindent Dataset from \citet{WinNT}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 idx & \verb+ 0 + \\
	 label & \verb+ 0 + \\
	 question1 & \verb+ How is the life of a math student? Could you descr... + \\
	 question2 & \verb+ Which level of prepration is enough for the exam j... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I'm an administrator on the website Quora. There are two posts, one that asks "{{question1}}" and another that asks "{{question2}}". I can merge questions if they are asking the same thing. Can I merge these two questions?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
no ||| yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{question1}}
{{question2}}
Pick one: These questions are "{{"duplicates"}}" or "{{"not duplicates"}}".
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
not duplicates ||| duplicates
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Are the questions "{{question1}}" and "{{question2}}" asking the same thing?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
no ||| yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Can an answer to "{{question1}}" also be used to answer "{{question2}}"?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
no ||| yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Question 1: {{question1}}
Question 2: {{question2}}

Do these two questions convey the same meaning? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I received the questions "{{question1}}" and "{{question2}}". Are they duplicates?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
no ||| yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{paws labeled\_final}
\noindent Dataset from \citet{paws2019naacl}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ 1 + \\
	 label & \verb+ 0 + \\
	 sentence1 & \verb+ In Paris , in October 1560 , he secretly met the E... + \\
	 sentence2 & \verb+ In October 1560 , he secretly met with the English... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Determine if the following two sentences paraphrase each other or not.
Sent 1: {{sentence1}}
Sent 2: {{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}
Question: Do Sentence 1 and Sentence 2 express the same meaning? Yes or No?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{sentence1}}
Is that a paraphrase of the following sentence?
{{sentence2}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}
Question: Can we rewrite Sentence 1 to Sentence 2?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{sentence1}}
Is that a paraphrase of the following sentence?
{{sentence2}}?
Yes or No.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}
Question: Does Sentence 1 paraphrase Sentence 2? Yes or No?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if label == 1 %} 
Paraphrase the sentence: {{sentence1}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{sentence2}} 
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}
Question: Does Sentence 1 paraphrase Sentence 2?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}
Question: Do Sentence 1 and Sentence 2 express the same meaning?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{sentence1}} Question: {{sentence2}} True or False?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
False ||| True
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}
Question: Can we rewrite Sentence 1 to Sentence 2? Yes or No?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{sentence1}} Question: {{sentence2}} Paraphrase or not?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{QA Closed Book }
\subsubsection{ai2\_arc ARC-Challenge}
\noindent Dataset from \citet{allenai:arc}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answerKey & \verb+ A + \\
	 choices & \verb+ {'label': ['A', 'B', 'C', 'D'], 'text': ['dry palm... + \\
	 id & \verb+ Mercury_SC_415702 + \\
	 question & \verb+ George wants to warm his hands quickly by rubbing ... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Pick and copy all the incorrect options for the following question:

{{question}}

Options:
- {{choices["text"] | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for i in range(choices["label"]|length) %}
{% if i != choices["label"].index(answerKey) %}
- {{choices["text"][i]}}
{% endif %}
{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Here's a problem to solve: {{question}}

Among the 4 following options, which is the correct answer?
{% for letter, t in zip(answer_choices, choices.text) %}
- {{letter}}: {{t}}
 {% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answerKey}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{question}}

Options:
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices["label"].index(answerKey)]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I am hesitating between 4 options to answer the following question, which option should I choose?
Question: {{question}}
Possibilities:
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices["label"].index(answerKey)]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I gave my students this multiple choice question: {{question}}

Only one answer is correct among these 4 choices:
- {{answer_choices | join("\n- ")}}

Could you tell me which one is correct?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices["label"].index(answerKey)]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Pick the most correct option to answer the following question.

{{question}}

Options:
{% for letter, t in zip(answer_choices, choices.text) %}
- {{letter}}: {{t}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answerKey}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{ai2\_arc ARC-Easy}
\noindent Dataset from \citet{allenai:arc}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answerKey & \verb+ B + \\
	 choices & \verb+ {'label': ['A', 'B', 'C', 'D'], 'text': ['a leg mu... + \\
	 id & \verb+ Mercury_7220990 + \\
	 question & \verb+ Which factor will most likely cause a person to de... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Pick the most correct option to answer the following question.

{{question}}

Options:
{% for letter, t in zip(answer_choices, choices.text) %}
- {{letter}}: {{t}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answerKey}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{question}}

Options:
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices["label"].index(answerKey)]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I am hesitating between 4 options to answer the following question, which option should I choose?
Question: {{question}}
Possibilities:
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices["label"].index(answerKey)]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I gave my students this multiple choice question: {{question}}

Only one answer is correct among these 4 choices:
- {{answer_choices | join("\n- ")}}

Could you tell me which one is correct?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices["label"].index(answerKey)]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Pick and copy all the incorrect options for the following question:

{{question}}

Options:
- {{choices["text"] | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for i in range(choices["label"]|length) %}
{% if i != choices["label"].index(answerKey) %}
- {{choices["text"][i]}}
{% endif %}
{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Here's a problem to solve: {{question}}

Among the 4 following options, which is the correct answer?
{% for letter, t in zip(answer_choices, choices.text) %}
- {{letter}}: {{t}}
 {% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answerKey}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{kilt\_tasks hotpotqa}
\noindent Dataset from \citet{fb_kilt}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ 5a7a06935542990198eaf050 + \\
	 input & \verb+ Which magazine was started first Arthur's Magazine... + \\
	 meta & \verb+ {'left_context': '', 'mention': '', 'right_context... + \\
	 output & \verb+ [{'answer': "Arthur's Magazine", 'meta': {'score':... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if output %}
Here's a complex question that requires someone to reason about the input, can you answer it?
{{input}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output | map(attribute="answer") | list | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if output %}
Combine facts and answer this: {{input}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output | map(attribute="answer") | list | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if output %}
Formulate an answer to this elaborate question: {{input}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output | map(attribute="answer") | list | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if output %}
FINAL EXAM

Question 1. {{input}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output | map(attribute="answer") | list | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if output %}
{{input}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{output | map(attribute="answer") | list | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{trivia\_qa unfiltered}
\noindent Dataset from \citet{2017arXivtriviaqa}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 question & \verb+ Who was President when the first Peanuts cartoon w... + \\
	 question\_id & \verb+ tc_0 + \\
	 question\_source & \verb+ http://www.triviacountry.com/ + \\
	 entity\_pages & \verb+ {'doc_source': ['TagMe'], 'filename': ['Peanuts.tx... + \\
	 search\_results & \verb+ {'description': ['Peanuts 1950s. The first Peanuts... + \\
	 answer & \verb+ {'aliases': ['Presidency of Harry S. Truman', 'Har... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answer.aliases %} 
    Guess a question that has the answer "{{answer.aliases|choice}}"
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}} 
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
The goal is to predict an English answer string for an input English question. 
Question : {{question}}
Answer :
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer.aliases %} 
{{answer.aliases|choice}} 
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Answer the following question.
{{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer.aliases %} 
{{answer.aliases|choice}} 
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I've always wondered: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer.aliases %} 
{{answer.aliases|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Question : {{question}}
Answer :
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answer.aliases %} 
{{answer.aliases|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{web\_questions}
\noindent Dataset from \citet{berant-etal-2013-semantic}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ ['Jazmyn Bieber', 'Jaxon Bieber'] + \\
	 question & \verb+ what is the name of justin bieber brother? + \\
	 url & \verb+ http://www.freebase.com/view/en/justin_bieber + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Give me the correct facts to answer this: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Give me a possible correct answer to the question "{{ question }}"
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers | choice }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
What's the answer to that question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Short general knowledge question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ question|capitalize }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers | choice }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{wiki\_qa}
\noindent Dataset from \citet{YangYihMeek:EMNLP2015:WikiQA}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ African immigration to the United States refers to... + \\
	 document\_title & \verb+ African immigration to the United States + \\
	 label & \verb+ 0 + \\
	 question & \verb+ HOW AFRICAN AMERICANS WERE IMMIGRATED TO THE US + \\
	 question\_id & \verb+ Q0 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Question: {{question}}?
Would "{{answer}}" be a reasonable answer?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I am verifying the answers generated by an automatic system to the following question: {{question}}
Suggested answer: {{answer}}
Should I validate this answer?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if label == 1 %}
What is the question to: "{{answer}}"? The topic is {{document_title}}.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
"{{question}}?"
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if label == 1 %}
Determine the topic of the question-answer pair.
Question: "{{question}}?";  Answer: "{{answer}}"? Topic:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{document_title}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if label == 1 %}
Generate a question about the topic "{{document_title}}" whose answer would be: {{answer}}.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}?
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Question: {{question}}
I found the following answer on Google: {{answer}}
Is that a correct answer? Yes or no.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if label == 1 %}
Determine the topic of the question.
Question: "{{question}}?"
Topic:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{document_title}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
The exercise is to decide whether the question accepts the proposed suggestion as a correct answer. If yes, write "{{answer_choices[1]}}", otherwise write "{{answer_choices[0]}}".
Question: {{question}}
Suggestion: {{answer}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
False ||| True
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
This is a correct answer to the following question about {{document_title}}. Yes or no?
Answer: {{answer}}
Question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if label == 1 %}
Determine the topic of the passage.
"{{answer}}"
Topic:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{document_title}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if label == 1 %}
Answer this question: {{question}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{QA Extractive }
\subsubsection{adversarial\_qa dbidaf}
\noindent Dataset from \citet{bartolo2020beat}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ 821607441c173838196c4d1500c2ab21a044e6b0 + \\
	 title & \verb+ Yale_University + \\
	 context & \verb+ Slack (2003) compares three groups that conducted ... + \\
	 question & \verb+ what year were the research groups compared + \\
	 answers & \verb+ {'text': ['2003'], 'answer_start': [7]} + \\
	 metadata & \verb+ {'split': 'train', 'model_in_the_loop': 'BiDAF'} + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if metadata.split != "test" %}
Extract the answer to the question from the following context.
Question: {{question}}
Context: {{context}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if metadata.split != "test" %}
Given the following passage

"{{context}}",

answer the following question. Note that the answer is present within the text.

Question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I want to test the ability of students to read a passage and answer questions about it. Could you please come up with a good question for the passage "{{context}}"?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if metadata.split != "test" %}
I know that the answer to the question "{{question}}" is in "{{context}}". Can you tell me what it is?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if metadata.split != "test" %}
Question: "{{question}}"

Context: "{{context}}"

Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{adversarial\_qa dbert}
\noindent Dataset from \citet{bartolo2020beat}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ dab017ed8a1c27c6afa2d8618abc3a477a4edffc + \\
	 title & \verb+ Empiricism + \\
	 context & \verb+ A generation later, the Irish Anglican bishop, Geo... + \\
	 question & \verb+ what concept is mentioned last? + \\
	 answers & \verb+ {'text': ['subjective idealism'], 'answer_start': ... + \\
	 metadata & \verb+ {'split': 'train', 'model_in_the_loop': 'BERT-Larg... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I want to test the ability of students to read a passage and answer questions about it. Could you please come up with a good question for the passage "{{context}}"?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if metadata.split != "test" %}
I know that the answer to the question "{{question}}" is in "{{context}}". Can you tell me what it is?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if metadata.split != "test" %}
Question: "{{question}}"

Context: "{{context}}"

Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if metadata.split != "test" %}
Extract the answer to the question from the following context.
Question: {{question}}
Context: {{context}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if metadata.split != "test" %}
Given the following passage

"{{context}}",

answer the following question. Note that the answer is present within the text.

Question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{adversarial\_qa droberta}
\noindent Dataset from \citet{bartolo2020beat}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ 12cf36866b656dc4f254081fe6796ea1be2f6d43 + \\
	 title & \verb+ Napoleon + \\
	 context & \verb+ When he became First Consul and later Emperor, Nap... + \\
	 question & \verb+ What jewelry like accessories did he wear? + \\
	 answers & \verb+ {'text': ["Légion d'honneur star, medal and ribbon... + \\
	 metadata & \verb+ {'split': 'train', 'model_in_the_loop': 'RoBERTa-L... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I want to test the ability of students to read a passage and answer questions about it. Could you please come up with a good question for the passage "{{context}}"?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if metadata.split != "test" %}
I know that the answer to the question "{{question}}" is in "{{context}}". Can you tell me what it is?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if metadata.split != "test" %}
Question: "{{question}}"

Context: "{{context}}"

Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if metadata.split != "test" %}
Extract the answer to the question from the following context.
Question: {{question}}
Context: {{context}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if metadata.split != "test" %}
Given the following passage

"{{context}}",

answer the following question. Note that the answer is present within the text.

Question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{duorc SelfRC}
\noindent Dataset from \citet{DuoRC}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ ['They arrived by train.'] + \\
	 no\_answer & \verb+ False + \\
	 plot & \verb+ 200 years in the future, Mars has been colonized b... + \\
	 plot\_id & \verb+ /m/03vyhn + \\
	 question & \verb+ How did the police arrive at the Mars mining camp? + \\
	 question\_id & \verb+ b440de7d-9c3f-841c-eaec-a14bdff950d1 + \\
	 title & \verb+ Ghosts of Mars + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if no_answer == false%}
Generate a question that has the following answer: 
{{answers|choice}} 
for the following movie plot: 
{{plot}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I am a movie director and I just received the following movie plot. Could you help me answer this question? If not, let me know by writing "{{"Not answerable"}}".

Plot title: {{title}}
Movie plot: {{plot}}
My question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
Not answerable
{% else %}
{{answers|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Extract the answer to the following question from the movie plot. If the question isn't answerable, please output "{{"Can't answer"}}".
Question: {{question}}
Title: {{title}}
Movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
Can't answer
{% else %}
{{answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Generate a question about the following movie plot: {{ plot }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ question }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Please answer the following question about this movie plot. If it's un-answerable, please output "{{"No answer"}}".

Question: {{question}}
Movie plot title: {{title}}
Movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
No answer
{% else %}
{{answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if no_answer == false%}
Build a movie plot around this: {{ question }} {{answers|choice}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ plot }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Question: {{question}}
If there is no answer, please output "{{"Insufficient information to provide an answer."}}".
Movie title: {{title}}
Context: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
Insufficient information to provide an answer.
{% else %}
{{answers|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Suggest a movie title for the following movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{title}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I am trying to decide whether it's worth it to invest in this film proposal. Can you help me answer a few questions? If you can't, please say "{{"No I can't"}}".

Question: {{question}}
Movie title: {{title}}
Movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
No I can't
{% else %}
{{answers|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{duorc ParaphraseRC}
\noindent Dataset from \citet{DuoRC}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ ['second in command Sergeant  Jericho and prisoner... + \\
	 no\_answer & \verb+ False + \\
	 plot & \verb+ Set in the second half of the 22nd century, Mars h... + \\
	 plot\_id & \verb+ /m/03vyhn + \\
	 question & \verb+ who is there with Melanie Ballard? + \\
	 question\_id & \verb+ 28ded42d-f6d5-aac6-cf6f-9e6e0820c5aa + \\
	 title & \verb+ Ghosts of Mars + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if no_answer == false%}
Build a movie plot around this: {{ question }} {{answers|choice}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ plot }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I am trying to decide whether it's worth it to invest in this film proposal. Can you help me answer a few questions? If you can't, please say "{{"No I can't"}}".

Question: {{question}}
Movie title: {{title}}
Movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
No I can't
{% else %}
{{answers|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Question: {{question}}
If there is no answer, please output "{{"Insufficient information to provide an answer."}}".
Movie title: {{title}}
Context: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
Insufficient information to provide an answer.
{% else %}
{{answers|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I am a movie director and I just received the following movie plot. Could you help me answer this question? If not, let me know by writing "{{"Not answerable"}}".

Plot title: {{title}}
Movie plot: {{plot}}
My question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
Not answerable
{% else %}
{{answers|choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Generate a question about the following movie plot: {{ plot }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ question }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Extract the answer to the following question from the movie plot. If the question isn't answerable, please output "{{"Can't answer"}}".
Question: {{question}}
Title: {{title}}
Movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
Can't answer
{% else %}
{{answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Suggest a movie title for the following movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{title}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Please answer the following question about this movie plot. If it's un-answerable, please output "{{"No answer"}}".

Question: {{question}}
Movie plot title: {{title}}
Movie plot: {{plot}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if no_answer %}
No answer
{% else %}
{{answers | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if no_answer == false%}
Generate a question that has the following answer: 
{{answers|choice}} 
for the following movie plot: 
{{plot}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{ropes}
\noindent Dataset from \citet{Lin2019ReasoningOP}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ {'text': ['cup B']} + \\
	 background & \verb+ Passive transport occurs when a substance passes t... + \\
	 id & \verb+ 1971664873 + \\
	 question & \verb+ Which cup has a higher concentration of sugar? + \\
	 situation & \verb+ A man put two cups, cup A and cup B, filled with e... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text %}
Please answer correctly the following question related to the paragraph below. 

{{ question }}

{{ situation }}

Hint: {{ background }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text %}
{{ situation }}

Given the paragraph above, please answer correctly the following question: 

{{ question }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text %}
Background: {{ background }}

Paragraph: {{ situation }}

Given the paragraph above, please answer correctly the following question: {{ question }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text %}
Given the background: {{background}}

and the situation: {{situation}}

Answer the following question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text %}
{{ situation }}

{{ question }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text %}
{{ situation }}

{{ question }}

Hint: {{ background }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text %}
{{ background }}

{{ situation }}

{{ question }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text %}
I can use this background: {{background}}

Now, I have a new situation: {{situation}}

Answer this question please: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text %}
You are given a new situation: {{situation}}

and a hint : {{background}}

Please answer this question : {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text %}
I have a new situation: {{situation}}

But I can use this background: {{background}}

What is an answer for this question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text %}
{{ situation }}

Given the paragraph above, please answer correctly the following question: 

{{ question }}

Hint: {{ background }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text %}
I read this background article the other day: {{background}}

I am facing a new situation today: {{situation}}

Using the knowledge I acquired from the background article, how should I answer correctly the following question regarding my new situation: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answers.text | choice }}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{squad\_v2}
\noindent Dataset from \citet{2016arXiv160605250R}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ 56be85543aeaaa14008c9063 + \\
	 title & \verb+ Beyoncé + \\
	 context & \verb+ Beyoncé Giselle Knowles-Carter (/biːˈjɒnseɪ/ bee-Y... + \\
	 question & \verb+ When did Beyonce start becoming popular? + \\
	 answers & \verb+ {'text': ['in the late 1990s'], 'answer_start': [2... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set seq = [
'Answer the question depending on the context.',
'What is the answer?',
] %}

{{ seq | choice }}
Context: {{context}};
Question: {{question}};
Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answers.text == [] %}
Answer not in context
{% else %}
{{answers.text[0]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text != [] %}
Determine the question that you might have asked to get back the following answer for the given context
Context: {{context}};
Answer: {{answers.text[0]}};
Question:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set seq = [
'What is this about? ',
'What is the paragraph about? ',
'Get the topic from: ',
'From the passage,  get the topic',
'I want to know the topic. ',
'Topic from the passage: ',
'Topic from the paragraph: ',
] %}
{{ seq | choice }}
{{context}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{title | replace("_", " ")}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set seq = [
'This is about ',
'What is this about? ',
'The paragraph is about ',
'What is the paragraph about? ',
'Get the topic: ',
'From the passage, the topic is',
'I want to know the topic. ',
'Topic from the passage: ',
'Topic from the paragraph: ',
] %}
{{context}}
{{ seq | choice }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{title | replace("_", " ")}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text != [] %}
What is a question that would give the following answer?
Answer: {{answers.text[0]}};
Question:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set seq = [
'Can you tell me ',
'Please tell me ',
'Tell me ',
'From the passage, ',
'I want to know ',
'I want to ask ',
'What is the answer to: ',
'Find the answer to: ',
'Answer: ',
'',
] %}
{{context}} {{ seq | choice }}{{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answers.text == [] %}
Answer not in context
{% else %}
{{answers.text[0]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set seq = [
'Answer the question depending on the context.',
'What is the answer?',
] %}

{{ seq | choice }}
Context: {{context}};
Question: {{question}};
If you can't find the answer, please respond "unanswerable".
Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answers.text == [] %}
unanswerable
{% else %}
{{answers.text[0]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if answers.text != [] %}
{{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text[0]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set seq = [
'Can you tell me ',
'Please tell me ',
'Tell me ',
'From the passage, ',
'I want to know ',
'I want to ask ',
'What is the answer to: ',
'Find the answer to: ',
'Answer: ',
'',
] %}
{{context}} {{ seq | choice }}{{question}} If you can't find the answer, please respond "unanswerable".
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answers.text == [] %}
unanswerable
{% else %}
{{answers.text[0]}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Context: {{context}}; 

Question: {{question}} 

Is this question answerable?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answers.text != [] %}
{{answer_choices[0]}}
{% else %}
{{answer_choices[1]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
yes ||| no
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set seq = [
'Determine the topic of the question-answer pair. ',
'Find the topic. ',
'What is the topic from this? ',
] %}
{% if answers.text != [] %}
{{ seq | choice }}
Question: {{question}};  Answer: {{answers.text[0]}}; Topic:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{title}}
{% endif %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
What is the following passage about?
{{context}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{title | replace("_", " ")}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{super\_glue record}
\noindent Dataset from \citet{zhang2018record}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ ['Nuria'] + \\
	 entities & \verb+ ['Afghanistan', 'Badam Bagh', 'Mariam', 'Nuria'] + \\
	 idx & \verb+ {'passage': 0, 'query': 0} + \\
	 passage & \verb+ The harrowing stories of women and children locked... + \\
	 query & \verb+ The baby she gave birth to is her husbands and he ... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage }} 
{{ query }} 
Which one is the "{{"@placeholder"}}"? {{ entities | join(", ") }}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %} {{ answers | choice }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ entities | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
The following document has been corrupted. Tell me what "{{"@placeholder"}}" is referring to.

Document: {{ passage }} 
{{ query }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}{{ answers | choice }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ entities | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Summary:

- {{ passage.split("@highlight")[1:] | join("\n- ") }} 

Article:

{{ passage.split("@highlight")[0] }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}{{ query | replace("@placeholder", answers | choice) }} {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{% for entity in entities[:-1] %} {{ query | replace("@placeholder", entity) }} ||| {% endfor %} {{ query | replace("@placeholder", entities[-1]) }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Summary:

- {{ passage.split("@highlight")[1:] | join("\n- ") }} 

Article:

{{ passage.split("@highlight")[0] }}

Now that you've read the article, please write a new sentence to add to it.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}{{ query | replace("@placeholder", answers | choice) }} {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{% for entity in entities[:-1] %} {{ query | replace("@placeholder", entity) }} ||| {% endfor %} {{ query | replace("@placeholder", entities[-1]) }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage }} 
{{ query }} 

You should decide what "{{"@placeholder"}}" is referring to. Choose between:
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}{{ answers | choice }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ entities | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage.split("@highlight")[0] }}

Summary:

- {{ passage.split("@highlight")[1:] | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}- {{ query | replace("@placeholder", answers | choice) }} {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{% for entity in entities[:-1] %} - {{ query | replace("@placeholder", entity) }} ||| {% endfor %} - {{ query | replace("@placeholder", entities[-1]) }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Article:

{{ passage.split("@highlight")[0] }}

Highlights:

{{ passage.split("@highlight")[1:] | join("\n") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}{{ query | replace("@placeholder", answers | choice) }} {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{% for entity in entities[:-1] %} {{ query | replace("@placeholder", entity) }} ||| {% endfor %} {{ query | replace("@placeholder", entities[-1]) }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage }} 
{{ query }} 
In the question above, the "{{"@placeholder"}}" stands for
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}{{ answers | choice }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ entities | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
After reading the article, write another sentence to add to it.
{{ passage | replace("@highlight", "\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}{{ query | replace("@placeholder", answers | choice) }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{% for entity in entities[:-1] %} {{ query | replace("@placeholder", entity) }} ||| {% endfor %} {{ query | replace("@placeholder", entities[-1]) }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Please read the following news article and write another sentence to add to it.

{{ passage | replace("@highlight", "\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}{{ query | replace("@placeholder", answers | choice) }} {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{% for entity in entities[:-1] %} {{ query | replace("@placeholder", entity) }} ||| {% endfor %} {{ query | replace("@placeholder", entities[-1]) }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage }} 
{{ query }} 
What could the "{{"@placeholder"}}" be? {{ entities | join(", ") }}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}{{ answers | choice }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ entities | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage }}
{{ query }}

I am trying to decide what "{{"@placeholder"}}" means in the previous text.
Help by choosing an option between:
- {{ entities | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}
{{ answers | choice }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{entities | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage }} 
{{ query }} 
Here, the placeholder refers to
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}{{ answers | choice }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ entities | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage.split("@highlight")[0] }}

Highlights:

- {{ passage.split("@highlight")[1:] | join("\n- ") }} 

Please write an additional highlight.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}- {{ query | replace("@placeholder", answers | choice) }} {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{% for entity in entities[:-1] %} - {{ query | replace("@placeholder", entity) }} ||| {% endfor %} - {{ query | replace("@placeholder", entities[-1]) }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Exercise: Extract from the text the correct entity that "{{"@placeholder"}}" is referring to.

{{ passage }}
{{ query }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}
{{ answers | choice }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{entities | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage }}
{{ query }}

Pick one option, "{{"@placeholder"}}" refers to:
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}
{{ answers | choice }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{entities | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage | replace("@highlight", "\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}- {{ query | replace("@placeholder", answers | choice) }} {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{% for entity in entities[:-1] %} - {{ query | replace("@placeholder", entity) }} ||| {% endfor %} - {{ query | replace("@placeholder", entities[-1]) }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Article:

{{ passage.split("@highlight")[0] }}

Highlights:

- {{ passage.split("@highlight")[1:] | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}- {{ query | replace("@placeholder", answers | choice) }} {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{% for entity in entities[:-1] %} - {{ query | replace("@placeholder", entity) }} ||| {% endfor %} - {{ query | replace("@placeholder", entities[-1]) }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage }} 
{{ query }} 
Can you figure out what does the "{{"@placeholder"}}" mean? It means
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}{{ answers | choice }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ entities | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage | replace("@highlight", "\n") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if ( answers | length ) > 0 %}{{ query | replace("@placeholder", answers | choice) }} {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{% for entity in entities[:-1] %} {{ query | replace("@placeholder", entity) }} ||| {% endfor %} {{ query | replace("@placeholder", entities[-1]) }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{quoref}
\noindent Dataset from \citet{allenai:quoref}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ {'answer_start': [250], 'text': ['Catherine']} + \\
	 context & \verb+ The earthquake swarm was noted on October 12, 2007... + \\
	 id & \verb+ ba3f052c7a557909526b59713430403dd134e01d + \\
	 question & \verb+ What is the first name of the person who doubted i... + \\
	 title & \verb+ 2007–2008 Nazko earthquakes 1 + \\
	 url & \verb+ https://en.wikipedia.org/wiki/2007%E2%80%932008_Na... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
The answer to the question: {{question}} is inside the article: {{context}}, can you guess it ?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given the following context:

{{context}}

answer the following question:

{{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
The following article contains an answer for the question: {{question}} , can you please find it? 

{{context}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
This article: {{context}} contains an answer for the question: {{question}}, what is it ?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{question}}

Answer the above question based on the context below:

{{context}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
What is the answer for the question: {{question}} from the following article ?

{{context}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I have a test where I am given the following article, what is an answer for the question: {{question}} ?

{{context}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given the below context:

{{context}}

Guess a valid title for it!
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{title}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Found the following article online, use it to answer the question: {{question}}

{{context}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
A friend asked me to answer this question: {{question}}, using the article: {{context}}, what would be the answer ?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the following paragraph and extract the answer for the question: {{question}}

{{context}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answers.text | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{QA Multiple Choice }
\subsubsection{cos\_e v1.11}
\noindent Dataset from \citet{rajani2019explain}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 abstractive\_explanation & \verb+ webmath is designed to help you solve + \\
	 answer & \verb+ math problem + \\
	 choices & \verb+ ['park', 'coloring book', 'garden center', 'math p... + \\
	 extractive\_explanation & \verb+ "there are 10 apples on an apple tree. three fall ... + \\
	 id & \verb+ 6b819727eb8a670df26a7ffad036c119 + \\
	 question & \verb+ "There are 10 apples on an apple tree.  Three fall... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ question }}
Choose the most suitable option to answer the above question.
Options:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ choices | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ question }}
Choose the most suitable option to answer the above question.
Options：
{% for k in range(choices | length) %}
{{'. '.join([answer_choices[k], choices[k]])}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[choices.index(answer)] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D ||| E
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Question: {{question}}

Choices: 
- {{ choices | join("\n- ") }}

The rationale to choose "{{answer}}" as the answer is that:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{abstractive_explanation}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ question }}
- {{ answer_choices | join("\n- ") }}

The best answer is
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ choices | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Here's a question and a few possible answers: 

Q: {{ question }}
Possible A: {{ choices | join(", ") }}

Why is "{{answer}}" an answer aligned with human common sense?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ abstractive_explanation }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Pick the option in line with common sense to answer the question.
Question: {{ question }}
Options:
{% for k in range(choices | length) %}
{{'. '.join([answer_choices[k], choices[k]])}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[choices.index(answer)] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D ||| E
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Question: {{ question }}
Options:
- {{ choices | join("\n- ") }}

Explain why a human would choose "{{answer}}" to answer the question above:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ abstractive_explanation }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Question: {{ question }}
Options:
- {{ choices | join("\n- ") }}

The answer is "{{ answer }}" because
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ abstractive_explanation }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Pick the option in line with common sense to answer the question.
Questions: {{ question }}
Options:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ choices | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Here's a question: {{ question }}

Here are possible answers to this question:
- {{ choices | join("\n- ") }}

I believe the correct choice is "{{answer}}", here's why:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ abstractive_explanation }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ question }}
{% for k in range(choices | length) %}
{{'. '.join([answer_choices[k], choices[k]])}}
{% endfor %}
The best answer is
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[choices.index(answer)] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D ||| E
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{cosmos\_qa}
\noindent Dataset from \citet{cosmos}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer0 & \verb+ None of the above choices . + \\
	 answer1 & \verb+ This person likes music and likes to see the show ... + \\
	 answer2 & \verb+ This person only likes Good Old War and Person L ,... + \\
	 answer3 & \verb+ Other Bands is not on tour and this person can not... + \\
	 context & \verb+ Good Old War and person L : I saw both of these ba... + \\
	 id & \verb+ 3Q9SPIIRWJKVQ8244310E8TUS6YWAC##34V1S5K3GTZMDUBNBI... + \\
	 label & \verb+ 1 + \\
	 question & \verb+ In the future , will this person go to see other b... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Based on the context and the answer, generate a question. 

Context: {{context}}

Answer:
{% if label == 0 %}
{{answer0}}
{% elif label == 1 %}
{{answer1}}
{% elif label == 2 %}
{{answer2}}
{% elif label == 3 %}
{{answer3}}
{% endif %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the following context and choose the best option to answer the question.
Context: {{ context }}
Question: {{ question }}
Options: 
- {{ answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the following context and answer the question.
Context: {{ context }}
Question: {{ question }}
Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the following context and choose the best option to answer the question.
Context: {{ context }}
Question: {{ question }}
Options: 
A. {{ answer0 }}
B. {{ answer1 }}
C. {{ answer2 }}
D. {{ answer3 }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
According to the above context, choose the best option to answer the following question.
Question: {{ question }}
Options:
- {{answer_choices | join("\n - ")}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
{{ question }}
A. {{ answer0 }}
B. {{ answer1 }}
C. {{ answer2 }}
D. {{ answer3 }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
Question: {{ question }}
The answer to the above question:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
{{ question }}
- {{ answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
According to the above context, choose the best option to answer the following question.
Question: {{ question }}
Options:
A. {{ answer0 }}
B. {{ answer1 }}
C. {{ answer2 }}
D. {{ answer3 }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
{{ question }}
Pick the best answer from the following options:
A. {{ answer0 }}
B. {{ answer1 }}
C. {{ answer2 }}
D. {{ answer3 }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
According to the above context, answer the following question.
{{ question }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
{{ question }}
Pick the best answer from the following options:
- {{ answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answer0}} ||| {{answer1}} ||| {{answer2}} ||| {{answer3}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{dream}
\noindent Dataset from \citet{sundream2018}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ Continue her dancing class. + \\
	 choice & \verb+ ['Consult her dancing teacher.', 'Take a more inte... + \\
	 dialogue & \verb+ ['M: I am considering dropping my dancing class. I... + \\
	 dialogue\_id & \verb+ 5-510 + \\
	 id & \verb+ 0 + \\
	 question & \verb+ What does the man suggest the woman do? + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the below conversation.

{{dialogue[:-1] | join("\n\n")}}

What would the listener say?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{dialogue[-1]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given the question "{{question}}" and the answer "{{answer}}", write a conversation that might have happened.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{dialogue | join("\n\n")}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{dialogue[1:] | join("\n\n")}}

What was said before this conversation?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{dialogue[0]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Dialogue:

{{dialogue | join("\n\n")}}

Question: {{question}} 

- {{answer_choices[0]}}

- {{answer_choices[1]}}

- {{answer_choices[2]}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the following conversation and answer the question.

{{dialogue | join("\n\n")}}

Question: {{question}} 

- {{answer_choices[0]}}

- {{answer_choices[1]}}

- {{answer_choices[2]}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{openbookqa main}
\noindent Dataset from \citet{OpenBookQA2018}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answerKey & \verb+ D + \\
	 choices & \verb+ {'label': ['puppies learning new tricks', 'childre... + \\
	 id & \verb+ 7-980 + \\
	 question\_stem & \verb+ The sun is responsible for + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{question_stem}}

Choose an answer from this list:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answerKey]]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{question_stem}}

Which is the correct answer?
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answerKey]]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{question_stem}}
{% for k in range(choices["text"] | length) %}
{{' -> '.join([["A", "B", "C", "D"][k], choices["text"][k]])}}
{% endfor %}
Is the right answer {{"A, B, C or D"}} ?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answerKey}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{question_stem}}

Choices:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answerKey]]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{question_stem}}
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answerKey]]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{question_stem}}
- {{ answer_choices | join("\n- ") }}

Which is the correct answer?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answerKey]]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{question_stem}}

Pick the right answer from the list:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answerKey]]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{qasc}
\noindent Dataset from \citet{allenai:qasc}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answerKey & \verb+ F + \\
	 choices & \verb+ {'label': ['A', 'B', 'C', 'D', 'E', 'F', 'G', 'H']... + \\
	 combinedfact & \verb+ Beads of water can be formed by clouds. + \\
	 fact1 & \verb+ beads of water are formed by water vapor condensin... + \\
	 fact2 & \verb+ Clouds are made of water vapor. + \\
	 formatted\_question & \verb+ What type of water formation is formed by clouds? ... + \\
	 id & \verb+ 3E7TUJ2EGCLQNOV1WEAJ2NN9ROPD9K + \\
	 question & \verb+ What type of water formation is formed by clouds? + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
If I tell you that {{combinedfact[0]|capitalize}}{{ combinedfact[1:]|trim('.') }}, and ask you the question "{{ question[0]|lower }}{{ question[1:] }}", is the correct answer "{{ choices.text[0][0]|lower}}{{ choices.text[0][1:]|trim('.') }}"?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answerKey == choices.label[0] %} Yes {% else %} No {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ fact1[0]|capitalize }}{{ fact1[1:]|trim|trim('.') }}, and {{fact2[0]|lower }}{{ fact2[1:]|trim|trim('.') }}. Given these facts, {{ question[0]|lower }}{{question[1:]|trim('?') }} among the following options:
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for choice in choices.label %} {% if choice == answerKey %}{{ answer_choices[loop.index - 1] }}{% endif %}{% endfor %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Fact 1: {{ fact1[0]|capitalize }}{{ fact1[1:]|trim|trim('.') }}.

Fact 2: {{fact2[0]|capitalize }}{{ fact2[1:]|trim|trim('.') }}.

Given the two facts above, {{ question[0]|lower }}{{question[1:]|trim('?') }}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for choice in choices.label %} {% if choice == answerKey %}{{ answer_choices[loop.index - 1] }}{% endif %}{% endfor %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
You are presented with the question "{{ question }}" and the following answer choices: 
- {{answer_choices | join("\n - ") }}

Now knowing that {{ fact1[0]|lower }}{{ fact1[1:]|trim|trim('.') }} and {{fact2[0]|lower }}{{ fact2[1:]|trim|trim('.') }}, choose the best answer.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for choice in choices.label %} {% if choice == answerKey %}{{ answer_choices[loop.index - 1] }}{% endif %}{% endfor %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
You are presented with the quiz "{{ question }}" 

But you don't know the answer, so you turn to your teacher to ask for hints. He says that "{{ fact1[0]|lower }}{{ fact1[1:]|trim|trim('.') }}" and "{{fact2[0]|lower }}{{ fact2[1:]|trim|trim('.') }}". 

So, what's the best answer to the question?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for choice in choices.label %} {% if choice == answerKey %}{{ answer_choices[loop.index - 1] }}{% endif %}{% endfor %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
If {{ combinedfact[0]|lower }}{{ combinedfact[1:]|trim|trim('.') }}, then {{ question[0]|lower }}{{question[1:]|trim|trim('?') }}?

Answer choices:
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for choice in choices.label %} {% if choice == answerKey %}{{ answer_choices[loop.index - 1] }}{% endif %}{% endfor %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Do you think the right answer to the question "{{ question[0]|lower }}{{ question[1:] }}" is "{{ choices.text[1][0]|lower}}{{ choices.text[1][1:]|trim('.') }}", given that
 {{combinedfact[0]|lower}}{{ combinedfact[1:]|trim('.') }}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if answerKey == choices.label[0] %} Yes {% else %} No {% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Fact 1: {{ fact1[0]|capitalize }}{{ fact1[1:]|trim|trim('.') }}.

Fact 2: {{fact2[0]|capitalize }}{{ fact2[1:]|trim|trim('.') }}.

Given the two facts above, answer the question "{{ question }}" with the following options: 
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for choice in choices.label %} {% if choice == answerKey %}{{ answer_choices[loop.index - 1] }}{% endif %}{% endfor %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{quail}
\noindent Dataset from \citet{DBLP:conf/aaai/RogersKDR20}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answers & \verb+ ['not enough information', 'to visit family', 'par... + \\
	 context & \verb+ That fall came and I went back to Michigan and the... + \\
	 context\_id & \verb+ f001 + \\
	 correct\_answer\_id & \verb+ 3 + \\
	 domain & \verb+ fiction + \\
	 id & \verb+ f001_0 + \\
	 metadata & \verb+ {'author': 'Joseph Devon', 'title': 'Black Eyed Su... + \\
	 question & \verb+ Why was this character sent away after each school... + \\
	 question\_id & \verb+ 0 + \\
	 question\_type & \verb+ Causality + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
Question: {{ question }}
Options:
{% for k in range(answers | length) %}
{{'. '.join([answer_choices[k], answers[k]])}}
{% endfor %}
===
The correct answer is
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
Question: {{ question }}
Options:
- {{ answer_choices | join(" \n - ") }}
===
The correct answer is
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the following context and choose the correct option to answer the question.
Context: {{ context }}
Question: {{ question }}
Options:
{% for k in range(answers | length) %}
{{'. '.join([answer_choices[k], answers[k]])}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
{{ question }}
Pick the correct answer from the following options:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
Question: {{ question }}
===
The answer to the above question is
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
According to the above context, answer the following question.
{{ question }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
{{ question }}
Pick the correct answer from the following options:
{% for k in range(answers | length) %}
{{'. '.join([answer_choices[k], answers[k]])}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
{{ question }}
{% for k in range(answers | length) %}
{{'. '.join([answer_choices[k], answers[k]])}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
According to the above context, choose the correct option to answer the following question.
Question: {{ question }}
Options:
{% for k in range(answers | length) %}
{{'. '.join([answer_choices[k], answers[k]])}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the following context and answer the question.
Context: {{ context }}
Question: {{ question }}
Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
{{ question }}
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ context }}
According to the above context, choose the correct option to answer the following question.
Question: {{ question }}
Options:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the following context and choose the correct option to answer the question.
Context: {{ context }}
Question: {{ question }}
Options:
- {{ answer_choices | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[correct_answer_id] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answers | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{quarel}
\noindent Dataset from \citet{quarel_v1}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 id & \verb+ QuaRel_V1_Fr_0223 + \\
	 answer\_index & \verb+ 1 + \\
	 logical\_forms & \verb+ ['(infer (speed higher world1) (smoothness higher ... + \\
	 logical\_form\_pretty & \verb+ qrel(speed, higher, world1) -> qrel(smoothness, hi... + \\
	 world\_literals & \verb+ {'world1': ['ice'], 'world2': ['snow']} + \\
	 question & \verb+ Mike was snowboarding on the snow and hit a piece ... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Question: {{question}}

Do not use {{"A"}} and {{"B"}} to answer the question but instead, choose between "{{answer_choices[0]}}" and  "{{answer_choices[1]}}".
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer_index]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{world_literals.world1[0]}} ||| {{world_literals.world2[0]}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Here's a logic test: {{question}}

Choose the answer between "{{answer_choices[0]}}" and "{{answer_choices[1]}}".
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer_index]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{world_literals.world1[0]}} ||| {{world_literals.world2[0]}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Here's a short story: {{question}}.

What is the most sensical answer between "{{answer_choices[0]}}" and  "{{answer_choices[1]}}"?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer_index]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{world_literals.world1[0]}} ||| {{world_literals.world2[0]}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Choose between "{{answer_choices[0]}}" and  "{{answer_choices[1]}}".
Question: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer_index]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{world_literals.world1[0]}} ||| {{world_literals.world2[0]}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I am testing my students' logic.
What is the answer they should choose between "{{answer_choices[0]}}" and "{{answer_choices[1]}}"?
Logic test: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[answer_index]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{world_literals.world1[0]}} ||| {{world_literals.world2[0]}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{quartz}
\noindent Dataset from \citet{quartz}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answerKey & \verb+ A + \\
	 choices & \verb+ {'label': ['A', 'B'], 'text': ['scarce', 'plentifu... + \\
	 id & \verb+ QRQA-10385-4 + \\
	 para & \verb+ Many of the worlds people live with water scarcity... + \\
	 para\_anno & \verb+ {'effect_prop': 'population growth', 'cause_dir_st... + \\
	 para\_id & \verb+ QRSent-10385 + \\
	 question & \verb+ John's town used to have lots of water, back when ... + \\
	 question\_anno & \verb+ {'more_effect_dir': 'several thousand', 'less_effe... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Use information from the paragraph to answer the question.

Question:

{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!") }} {{ answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}

Paragraph :

{{ para }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ para }}
{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!")}} {{ answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Use information from the paragraph to answer the question.

Paragraph :

{{ para }}

Question:

{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!") }} {{ answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Answer the question based on the following text.

Question:

{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!") }} {{ answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}

Text:

{{ para }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Answer the question below:

{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!") }} {{  answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}

Assuming that:

{{ para }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the passage below and choose the right answer to the following question (choices are {{ answer_choices | join(" or ") }} ):

{{ para }}

{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!") }} {{ answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ para }}

Having read the above passage, choose the right answer to the following question (choices are {{ answer_choices | join(" or ") }} ):

{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!") }} {{ answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given the fact that:

{{ para }}

Answer the question:

{% if '_____' in question %}
{{ question | trim(".?!") | replace("_____", answer_choices | join(" or ")) }}{{ "?" }} 
{% else %}
{{ question | trim(".?!") }} {{ answer_choices | join(" or ") }}{{ "?" }} 
{% endif %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[choices.label.index(answerKey)]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choices.text | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{race high}
\noindent Dataset from \citet{lai2017large}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ D + \\
	 article & \verb+ Studies show that you may be lied to every day any... + \\
	 example\_id & \verb+ high10001.txt + \\
	 options & \verb+ ['harmful', 'easy', 'interesting', 'common'] + \\
	 question & \verb+ From Para.1 we learn that lying is very   _  . + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set candidate = ["A", "B", "C", "D"] | choice %}
Article: {{article}}
Question: {{question}}
Yes or no, is the answer "{{ [options.0,options.1,options.2,options.3][{"A":0,"B":1,"C":2,"D":3}[answer]] }}"?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if candidate == answer %}
Yes
{% else %}
No
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Write a multi-choice question for the following article:
Article: {{article}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
Question: 
{{question}}
Options:
{{"A"}} {{options.0}}
{{"B"}} {{options.1}}
{{"C"}} {{options.2}}
{{"D"}} {{options.3}}
Answer:
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I'm taking a test and have to guess the right answer to the question after the article.
Article: {{article}}
Question: {{question}}
Options: {{"A"}}: {{options.0}}
{{"B"}}: {{options.1}}
{{"C"}}: {{options.2}}
{{"D"}}: {{options.3}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the article and select the best answer.
Article: {{article}}
Question: {{question}}
Options: {{"A"}}: {{options.0}}
{{"B"}}: {{options.1}}
{{"C"}}: {{options.2}}
{{"D"}}: {{options.3}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Write a multi-choice question for the following article, with the given choices and answer:
Article: {{article}}
Options:
{{"A"}} {{options.0}}
{{"B"}} {{options.1}}
{{"C"}} {{options.2}}
{{"D"}} {{options.3}}
Answer:
{{answer}} {{ [options.0,options.1,options.2,options.3][{"A":0,"B":1,"C":2,"D":3}[answer]] }}
Question:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the following article and select the best answer.
Article: {{article}}
Question: {{question}}
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answer]]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ options | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{article}}
{{question}}
{{"A)"}} {{options.0}}
{{"B)"}} {{options.1}}
{{"C)"}} {{options.2}}
{{"D)"}} {{options.3}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the following article and answer the question.
Article: {{article}}
Question: {{question}}
Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[{"A":0,"B":1,"C":2,"D":3}[answer]] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ options | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{race middle}
\noindent Dataset from \citet{lai2017large}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ C + \\
	 article & \verb+ Take a class at Dulangkou School, and you'll see l... + \\
	 example\_id & \verb+ middle1.txt + \\
	 options & \verb+ ['take care of the whole group', 'make sure that e... + \\
	 question & \verb+ A discipline leader is supposed to  _  . + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the article and select the best answer.
Article: {{article}}
Question: {{question}}
Options: {{"A"}}: {{options.0}}
{{"B"}}: {{options.1}}
{{"C"}}: {{options.2}}
{{"D"}}: {{options.3}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the following article and answer the question.
Article: {{article}}
Question: {{question}}
Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[{"A":0,"B":1,"C":2,"D":3}[answer]] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ options | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set candidate = ["A", "B", "C", "D"] | choice %}
Article: {{article}}
Question: {{question}}
Yes or no, is the answer "{{ [options.0,options.1,options.2,options.3][{"A":0,"B":1,"C":2,"D":3}[answer]] }}"?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if candidate == answer %}
Yes
{% else %}
No
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{article}}
{{question}}
{{"A)"}} {{options.0}}
{{"B)"}} {{options.1}}
{{"C)"}} {{options.2}}
{{"D)"}} {{options.3}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the following article and select the best answer.
Article: {{article}}
Question: {{question}}
- {{answer_choices | join("\n- ")}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[{"A":0,"B":1,"C":2,"D":3}[answer]]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{ options | join("|||") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Write a multi-choice question for the following article, with the given choices and answer:
Article: {{article}}
Options:
{{"A"}} {{options.0}}
{{"B"}} {{options.1}}
{{"C"}} {{options.2}}
{{"D"}} {{options.3}}
Answer:
{{answer}} {{ [options.0,options.1,options.2,options.3][{"A":0,"B":1,"C":2,"D":3}[answer]] }}
Question:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Write a multi-choice question for the following article:
Article: {{article}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
Question: 
{{question}}
Options:
{{"A"}} {{options.0}}
{{"B"}} {{options.1}}
{{"C"}} {{options.2}}
{{"D"}} {{options.3}}
Answer:
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I'm taking a test and have to guess the right answer to the question after the article.
Article: {{article}}
Question: {{question}}
Options: {{"A"}}: {{options.0}}
{{"B"}}: {{options.1}}
{{"C"}}: {{options.2}}
{{"D"}}: {{options.3}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C ||| D
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{sciq}
\noindent Dataset from \citet{SciQ}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 question & \verb+ What type of organism is commonly used in preparat... + \\
	 distractor3 & \verb+ viruses + \\
	 distractor1 & \verb+ protozoa + \\
	 distractor2 & \verb+ gymnosperms + \\
	 correct\_answer & \verb+ mesophilic organisms + \\
	 support & \verb+ Mesophiles grow best in moderate temperature, typi... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Q: {{question}}


A:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[3]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{distractor1}} ||| {{distractor2}} ||| {{distractor3}} ||| {{correct_answer}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set order = [[0, 1, 2, 3], [0, 1, 3, 2], [0, 2, 1, 3], [0, 2, 3, 1], [0, 3, 1, 2], [0, 3, 2, 1],
                             [1, 0, 2, 3], [1, 0, 3, 2], [1, 2, 0, 3], [1, 2, 3, 0], [1, 3, 0, 2], [1, 3, 2, 0],
                             [2, 1, 0, 3], [2, 1, 0, 2], [2, 0, 1, 3], [2, 0, 3, 1], [2, 3, 1, 0], [2, 3, 0, 1],
                             [3, 1, 2, 0], [3, 1, 0, 2], [3, 2, 1, 0], [3, 2, 0, 1], [3, 0, 1, 2], [3, 0, 2, 1]] | choice %}
Q: {{question}}


 Choices:

- {{ answer_choices[order[0]] }}

- {{ answer_choices[order[1]] }}

- {{ answer_choices[order[2]] }}

- {{ answer_choices[order[3]] }}

A:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[3]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{distractor1}} ||| {{distractor2}} ||| {{distractor3}} ||| {{correct_answer}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set order = [[0, 1, 2, 3], [0, 1, 3, 2], [0, 2, 1, 3], [0, 2, 3, 1], [0, 3, 1, 2], [0, 3, 2, 1],
                             [1, 0, 2, 3], [1, 0, 3, 2], [1, 2, 0, 3], [1, 2, 3, 0], [1, 3, 0, 2], [1, 3, 2, 0],
                             [2, 1, 0, 3], [2, 1, 0, 2], [2, 0, 1, 3], [2, 0, 3, 1], [2, 3, 1, 0], [2, 3, 0, 1],
                             [3, 1, 2, 0], [3, 1, 0, 2], [3, 2, 1, 0], [3, 2, 0, 1], [3, 0, 1, 2], [3, 0, 2, 1]] | choice %}
Q: {{question}}


Read this paragraph and choose the correct option from the provided answers:

{{support}}

 Choices:

- {{ answer_choices[order[0]] }}

- {{ answer_choices[order[1]] }}

- {{ answer_choices[order[2]] }}

- {{ answer_choices[order[3]] }}


A:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[3]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{distractor1}} ||| {{distractor2}} ||| {{distractor3}} ||| {{correct_answer}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set order = [[0, 1, 2, 3], [0, 1, 3, 2], [0, 2, 1, 3], [0, 2, 3, 1], [0, 3, 1, 2], [0, 3, 2, 1],
                             [1, 0, 2, 3], [1, 0, 3, 2], [1, 2, 0, 3], [1, 2, 3, 0], [1, 3, 0, 2], [1, 3, 2, 0],
                             [2, 1, 0, 3], [2, 1, 0, 2], [2, 0, 1, 3], [2, 0, 3, 1], [2, 3, 1, 0], [2, 3, 0, 1],
                             [3, 1, 2, 0], [3, 1, 0, 2], [3, 2, 1, 0], [3, 2, 0, 1], [3, 0, 1, 2], [3, 0, 2, 1]] | choice %}
Answer the following question given this paragraph: 

{{support}}


Q: {{question}}

 Choices:

- {{ answer_choices[order[0]] }}

- {{ answer_choices[order[1]] }}

- {{ answer_choices[order[2]] }}

- {{ answer_choices[order[3]] }}

A:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[3]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{distractor1}} ||| {{distractor2}} ||| {{distractor3}} ||| {{correct_answer}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Answer the following question given this paragraph: 

{{support}}


Q: {{question}}


A:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[3]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{distractor1}} ||| {{distractor2}} ||| {{distractor3}} ||| {{correct_answer}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{social\_i\_qa}
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answerA & \verb+ like attending + \\
	 answerB & \verb+ like staying home + \\
	 answerC & \verb+ a good friend to have + \\
	 context & \verb+ Cameron decided to have a barbecue and gathered he... + \\
	 label & \verb+ 1 + \\
	 question & \verb+ How would Others feel as a result? + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
I heard that {{context}}

And I was wondering {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label | int - 1]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answerA}} ||| {{answerB}} ||| {{answerC}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{context}}

Given the context: {{question}}

Possible answers: {{answer_choices | join(", ")}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label | int - 1]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answerA}} ||| {{answerB}} ||| {{answerC}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set random_answer_id = range(0,2) | choice%}
{% set answers = [answerA, answerB, answerC] %}
{{context}}

Given the question "{{question}}", is "{{answers[random_answer_id]}}" a valid answer?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if (label | int) - 1 == random_answer_id %}
    Yes
{% else %}
    No
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{context}}

Given that the answer to a question is "{{{"1": answerA, "2": answerB, "3": answerC}[label]}}", what is the question?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{question}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{context}}

Given the context: {{question}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label | int - 1]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{answerA}} ||| {{answerB}} ||| {{answerC}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Context: {{context}}

Question: {{question}}

Which one of these answers best answers the question according to the context?

A: {{answerA}}

B: {{answerB}}

C: {{answerC}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{{"1": "A", "2": "B", "3": "C"}[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
A ||| B ||| C
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{super\_glue boolq}
\noindent Dataset from \citet{clark2019boolq}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 idx & \verb+ 0 + \\
	 label & \verb+ 1 + \\
	 passage & \verb+ Persian language -- Persian (/ˈpɜːrʒən, -ʃən/), al... + \\
	 question & \verb+ do iran and afghanistan speak the same language + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Passage: {{passage}}

After reading this passage, I have a question: {{question}}? True or False?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
False ||| True
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage }} 
Question: {{ question }}
Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}
{{ answer_choices[label] }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage }} 

Having read that, I wonder {{ question }}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}
{{ answer_choices[label] }} 
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Text: {{passage}}

Answer the following yes/no question: {{question}}? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage }} 

Having read that, could you tell me {{ question }}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
EXAM
1. Answer by yes or no.

Document: {{passage}}
Question: {{question}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Based on the following passage, {{ question }}? {{ passage }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}
{{ answer_choices[label] }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Exercise: read the text and answer the question by True or False.

Text: {{passage}}
Question: {{question}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
False ||| True
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ passage }}
Based on the previous passage, {{ question }}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{passage}}

Q: {{question}}? True or False?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
False ||| True
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{super\_glue multirc}
\noindent Dataset from \citet{MultiRC2018}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer & \verb+ Children, Gerd, or Dorian Popa + \\
	 idx & \verb+ {'paragraph': 0, 'question': 0, 'answer': 0} + \\
	 label & \verb+ 0 + \\
	 paragraph & \verb+ While this process moved along, diplomacy continue... + \\
	 question & \verb+ What did the high-level effort to persuade Pakista... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{paragraph}}

Question: {{question}}
I found this answer "{{answer}}". Is that correct? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{answer_choices[label]}}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ paragraph }}
Based on the previous passage, {{ question }} 
Is "{{ answer }}" a correct answer?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{paragraph}}
Question: {{question}}

I am grading my students' exercises. Is the answer "{{answer}}" correct?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{answer_choices[label]}}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ paragraph }}
{{ question }} 
Would it be good to answer "{{ answer }}"?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ paragraph }}
Question: {{ question }} 
Is it {{ answer }}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{paragraph}}

Decide whether "{{answer}}" is a valid answer to the following question: {{question}}
Answer yes or no.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{answer_choices[label]}}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ paragraph }}
Question: {{ question }} 
Is the correct answer {{ answer }}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Is "{{answer}}" a correct answer to the following question?
Question: {{question}}

Rely on the following text: {{paragraph}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{answer_choices[label]}}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{paragraph}}

Question: {{question}}
I think "{{answer}}" is a valid answer. Could you confirm? Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{answer_choices[label]}}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ paragraph }}
{{ question }} 
I was going to say "{{ answer }}". Does that sound right?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{wiki\_hop original}
\noindent Dataset from \citet{welbl2018constructing}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 annotations & \verb+ [] + \\
	 answer & \verb+ 1996 summer olympics + \\
	 candidates & \verb+ ['1996 summer olympics', 'olympic games', 'sport'] + \\
	 id & \verb+ WH_train_0 + \\
	 question & \verb+ participant_of juan rossell + \\
	 supports & \verb+ ['The 2004 Summer Olympic Games, officially known ... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
What object entity has the relation of '{{ question_split[0] | replace("_", " ")}}' with the subject '{{ question_split[1:] | join(" ")}}'? 

Choices:
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{candidates | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
What is the relationship between '{{ question_split[1:] | join(" ")}}' and '{{answer}}'?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ question_split[0] | replace("_", " ") }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
What entity does '{{ question_split[1:] | join(" ")}}' has the relation '{{ question_split[0] | replace("_", " ") }}' with?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
Given the paragraphs above, decide what entity has the relation '{{ question_split[0] | replace("_", " ") }}' with '{{answer}}'.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ question_split[1:] | join(" ")}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
Given the information above, choose from the list below the object entity that exhibits the relation '{{ question_split[0] | replace("_", " ")}}' with the subject '{{ question_split[1:] | join(" ")}}'.

Choices:
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{candidates | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
After reading the paragraphs above, we are interested in knowing the entity with which '{{ question_split[1:] | join(" ")}}' exhibits the relationship of '{{ question_split[0] | replace("_", " ")}}'. Find the answer from the choices below.

Choices:
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{candidates | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
Given the information, choose the subject and object entities that have the relation of '{{ question_split[0] | replace("_", " ") }}'.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ question_split[1:] | join(" ") }} , {{answer}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
After reading the paragraphs above, choose the best answer for the entity that related to '{{ question_split[1:] | join(" ")}}' with the relationship of '{{ question_split[0] | replace("_", " ")}}'.

Choices:
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{candidates | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Information:
{% for support in supports %}
- {{ support }}
{% endfor %}

{% set question_split = question.split(' ') %}
'{{ question_split[1:] | join(" ")}}' is related to which object entity through the relation of '{{ question_split[0] | replace("_", " ")}}'?

Choices:
- {{answer_choices | join("\n - ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{candidates | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{wiqa}
\noindent Dataset from \citet{wiqa}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 answer\_label & \verb+ more + \\
	 answer\_label\_as\_choice & \verb+ A + \\
	 choices & \verb+ {'label': ['A', 'B', 'C'], 'text': ['more', 'less'... + \\
	 metadata\_graph\_id & \verb+ 144 + \\
	 metadata\_para\_id & \verb+ 1217 + \\
	 metadata\_path\_len & \verb+ 2 + \\
	 metadata\_question\_id & \verb+ influence_graph:1217:144:106#0 + \\
	 metadata\_question\_type & \verb+ INPARA_EFFECT + \\
	 question\_para\_step & \verb+ ['A tree produces seeds', 'The seeds are dispersed... + \\
	 question\_stem & \verb+ suppose there will be fewer new trees happens, how... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
-  {{ question_para_step[1:] | join("\n- ") }}

What might be the first step of the process?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ question_para_step | first }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set process_list = question_para_step[:-1] if question_para_step[-1] == "" else question_para_step %}
-  {{ process_list[:-1] | join("\n- ") }}

What might be the last step of the process?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ process_list | last }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
What is the missing first step of the following process:

-  {{ question_para_step[1:] | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ question_para_step | first }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set process_list = question_para_step[:-1] if question_para_step[-1] == "" else question_para_step %}
What is the final step of the following process:
-  {{ process_list[:-1] | join("\n- ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ process_list | last }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Process:
- {{ question_para_step | join("\n- ")}}

Question:
{{question_stem}}

How does the supposed perturbation influence the second effect mentioned. Answer by {{"more, less or no effect"}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_label|replace("_", " ")}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Process:

- {{ question_para_step | join("\n- ") }}

{{question_stem}}

Which of the following is the supposed perturbation?

- {{"directly impacting a step of the process"}}
- {{"indirectly impacting a step of the process"}}
- {{"not impacting any step of the process"}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{{"EXOGENOUS_EFFECT": "indirectly impacting a step of the process", "OUTOFPARA_DISTRACTOR": "not impacting any step of the process", "INPARA_EFFECT": "directly impacting a step of the process"}[metadata_question_type]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Process:
- {{ question_para_step | join("\n- ")}}

Question:
{{question_stem}}

- {{"A: more"}}
- {{"B: less"}}
- {{"C: no effect"}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_label_as_choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Process:

- {{ question_para_step | join("\n- ") }}

Perturbation hypothesis:
{{question_stem}}

Does the supposed perturbation have an effect (direct or indirect) on the process?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{{"EXOGENOUS_EFFECT": "yes", "OUTOFPARA_DISTRACTOR": "no", "INPARA_EFFECT": "yes"}[metadata_question_type]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{piqa}
\noindent Dataset from \citet{Bisk2020}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 goal & \verb+ When boiling butter, when it's ready, you can + \\
	 label & \verb+ 1 + \\
	 sol1 & \verb+ Pour it onto a plate + \\
	 sol2 & \verb+ Pour it into a jar + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Goal: {{goal}}

Which is the correct ending?
- {{sol1}}
- {{sol2}}

Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{sol1}} ||| {{sol2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{"Solution 1"}}: {{sol1}}
{{"Solution 2"}}: {{sol2}}

Goal: {{goal}}

Given the goal, what is the correct solution?

Answer by copying the correct solution
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{sol1}} ||| {{sol2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Sentence: {{goal}}

Choice {{answer_choices[0]}}: {{sol1}}

Choice {{answer_choices[1]}}: {{sol2}}

What is the index of the correct choice for ending for the sentence?

Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
1 ||| 2
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given a goal and a wrong solution, rewrite it to give a correct solution.
Goal: {{goal}} 
Solution: {{[sol1, sol2][1 - label]}}
Corrected solution:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{[sol1, sol2][label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Finish the following sentence with the best choice: {{goal}}

Choices:
- {{sol1}}
- {{sol2}}

Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{sol1}} ||| {{sol2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{goal}} {{sol2}}
Does this phrase make sense?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given a goal and 2 solutions, choose the most appropriate solution.
Goal: {{goal}}
- {{"Solution 1"}}: {{sol1}}
- {{"Solution 2"}}: {{sol2}}

Answer by returning either {{"Solution 1"}} or {{"Solution 2"}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Solution 1 ||| Solution 2
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given a sentence, correct it if it doesn't make sense. If it makes sense, just return it as the answer.
Input: {{goal}} {{sol2[0].lower() + sol2[1:]}}
Output:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{goal}} {{[sol1[0].lower() + sol1[1:], sol2[0].lower() + sol2[1:]][label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{goal}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{[sol1[0].lower() + sol1[1:], sol2[0].lower() + sol2[1:]][label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Does this phrase make sense?
{{goal}} {{sol1[0].lower() + sol1[1:]}}
Answer with {{answer_choices[0]}} or {{answer_choices[1]}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Sentence: {{goal}} {{sol1[0].lower() + sol1[1:]}}
If the sentence does not make sense, correct it so that it does make sense. Otherwise, just copy it.
Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{goal}} {{[sol1[0].lower() + sol1[1:], sol2[0].lower() + sol2[1:]][label]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Sentiment }
\subsubsection{amazon\_polarity}
\noindent Dataset from \citet{mcauley2013hidden}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 content & \verb+ This sound track was beautiful! It paints the sene... + \\
	 label & \verb+ 1 + \\
	 title & \verb+ Stuning even for the non-gamer + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Title: {{title}}
Review: {{content}}
Is the review positive or negative?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Negative ||| Positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Based on this review, would the user recommend this product?
===
Review: {{content}}
Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Is this product review positive?
Title: {{title}}
Review: {{content}}
Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Title: {{title}}
Review: {{content}}
Is this product review negative?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Title: {{title}}
Review: {{content}}
Does this product review convey a negative or positive sentiment?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Negative ||| Positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Is there a negative or positive tone to this product review?
===
Title: {{title}}
Review: {{content}}
Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Negative ||| Positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Here is a review left by a customer on a product. Would you say he was {{answer_choices[1]}} or {{answer_choices[0]}}?
Title: {{title}}
Review: {{content}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
dissatisfied ||| satisfied
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
You are considering whether to buy a product. You look at the reviews. Would the following review {{answer_choices[0]}} or {{answer_choices[1]}} the chances of you buying the product?
Review title: {{title}}
Product review: {{content}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
decrease ||| increase
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Title: {{title}}
Product review: {{content}}
Would you say this review depicts the product in a {{answer_choices[1]}} or {{answer_choices[0]}} light?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
unflattering ||| flattering
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{app\_reviews}
\noindent Dataset from \citet{Zurich Open Repository and
Archive:dataset}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 date & \verb+ October 12 2016 + \\
	 package\_name & \verb+ com.mantz_it.rfanalyzer + \\
	 review & \verb+ Great app! The new version now works on my Bravia ... + \\
	 star & \verb+ 4 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given this review: "{{review}}"
Would you recommend this app to a friend? {{answer_choices[0]}}, {{answer_choices[1]}}, {{answer_choices[2]}}, {{answer_choices[3]}}, or {{answer_choices[4]}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[star-1]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Not at all ||| No ||| Maybe ||| Yes ||| Definitely
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Generate a {{star}}-star review (1 being lowest and 5 being highest) about an app with package {{package_name}}.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{review}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
What would be the ★-rating of this review (★ being the lowest and ★★★★★ being the highest)? "{{review}}"
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[star-1]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
★ ||| ★★ ||| ★★★ ||| ★★★★ ||| ★★★★★
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
On a scale of 1-5 (with 1 being least favorable and 5 being most favorable), how would you rate this review? "{{review}}"
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{star}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{imdb}
\noindent Dataset from \citet{maas-EtAl:2011:ACL-HLT2011}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 text & \verb+ Bromwell High is a cartoon comedy. It ran at the s... + \\
	 label & \verb+ 1 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
The following movie review expresses what sentiment? {{text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} Did the reviewer find this movie {{"good or bad"}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
bad ||| good
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} 
Is this review {{"positive or negative"}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} How does the viewer feel about the movie?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} What sentiment does the writer express for the movie?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} The sentiment expressed for the movie is
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} What is the sentiment expressed in this text?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} This is definitely not a
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [1-label]}} review.
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} Did the reviewer enjoy the movie?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} What is the sentiment expressed by the reviewer for the movie?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} How does the reviewer feel about the movie?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
They didn't like it! ||| They loved it
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{rotten\_tomatoes}
\noindent Dataset from \citet{Pang+Lee:05a}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 text & \verb+ the rock is destined to be the 21st century's new ... + \\
	 label & \verb+ 1 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} Did the reviewer find this movie {{"good or bad"}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
bad ||| good
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} What is the sentiment expressed in this text?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} 
Is this review {{"positive or negative"}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} Did the reviewer enjoy the movie?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} How does the reviewer feel about the movie?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
They didn't like it ||| They loved it
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} The sentiment expressed for the movie is
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} What sentiment does the writer express for the movie?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
The following movie review expresses what sentiment? {{text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} What is the sentiment expressed by the reviewer for the movie?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} How does the viewer feel about the movie?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
negative ||| positive
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{yelp\_review\_full}
\noindent Dataset from \citet{zhang2015character}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 label & \verb+ 4 + \\
	 text & \verb+ dr. goldberg offers everything i look for in a gen... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ text }}
So I would like to give it
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
1 star ||| 2 stars ||| 3 stars ||| 4 stars ||| 5 stars
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ text }}
===
Based on that, my rating is
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
1 star ||| 2 stars ||| 3 stars ||| 4 stars ||| 5 stars
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Review text:
{{ text }}

Stars:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
1 star ||| 2 stars ||| 3 stars ||| 4 stars ||| 5 stars
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ text }} My rating for this place is
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
1 star ||| 2 stars ||| 3 stars ||| 4 stars ||| 5 stars
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Review text:
{{ text }}

Review score (between 1 and 5):
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
1 ||| 2 ||| 3 ||| 4 ||| 5
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Review: {{text}}
On a scale of 1 to 5, I would give this product
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
1 ||| 2 ||| 3 ||| 4 ||| 5
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Review text:
{{ text }}

Review rating:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
1 star ||| 2 stars ||| 3 stars ||| 4 stars ||| 5 stars
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Sentence Completion }
\subsubsection{super\_glue copa}
\noindent Dataset from \citet{roemmele2011choice}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 choice1 & \verb+ The sun was rising. + \\
	 choice2 & \verb+ The grass was cut. + \\
	 idx & \verb+ 0 + \\
	 label & \verb+ 0 + \\
	 premise & \verb+ My body cast a shadow over the grass. + \\
	 question & \verb+ cause + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Exercise: choose the most plausible alternative.

{{ premise }} {% if question == "cause" %} because... {% else %} so... {% endif %}
- {{choice1}}
- {{choice2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{%endif%}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if question == "effect" %} 
{{ premise }} What could happen next, "{{ answer_choices[0] }}" or "{{ answer_choices[1] }}"?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{%endif%}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ premise }} 

I am hesitating between two options. Help me choose the more likely {% if question == "cause" %} cause: {% else %} effect: {% endif %}
- {{choice1}}
- {{choice2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{%endif%}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ premise }} {% if question == "cause" %} This happened because... {% else %} As a consequence... {% endif %}
Help me pick the more plausible option:
- {{choice1}}
- {{choice2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{%endif%}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{schick-schutze-2021-just}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
"{{ answer_choices[0] }}" or "{{ answer_choices[1] }}"? {{ premise }} {% if question == "cause" %} because {% else %} so {% endif %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1 }} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if question == "effect" %} 
{{ premise }} As a result, "{{ answer_choices[0] }}" or "{{ answer_choices[1] }}"?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{%endif%}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ premise }} 

What's the best option?
- {{choice1}}
- {{choice2}}

We are looking for {% if question == "cause" %} a cause {% else %} an effect {% endif %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{answer_choices[label]}}{%endif%}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if question == "cause" %} 
{{ premise }} Which may be caused by "{{ answer_choices[0] }}" or "{{ answer_choices[1] }}"?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{%endif%}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Pick the more likely continuation to the following sentence:
{{ premise }} {% if question == "cause" %} as a result of: {% else %} as a consequence: {% endif %}
- {{choice1}}
- {{choice2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{%endif%}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ premise }}

Select the most plausible {% if question == "cause" %} cause: {% else %} effect: {% endif %}
- {{choice1}}
- {{choice2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{%endif%}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% if question == "cause" %} 
{{ premise }} Why? "{{ answer_choices[0] }}" or "{{ answer_choices[1] }}"?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{%endif%}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ premise }} {% if question == "cause" %} because... {% else %} so... {% endif %}
Choose between:
- {{choice1}}
- {{choice2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1 %}{{ answer_choices[label] }}{%endif%}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{choice1}} ||| {{choice2}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{hellaswag}
\noindent Dataset from \citet{zellers2019hellaswag}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 activity\_label & \verb+ Removing ice from car + \\
	 ctx & \verb+ Then, the man writes over the snow covering the wi... + \\
	 ctx\_a & \verb+ Then, the man writes over the snow covering the wi... + \\
	 ctx\_b & \verb+ then + \\
	 endings & \verb+ [', the man adds wax to the windshield and cuts it... + \\
	 ind & \verb+ 4 + \\
	 label & \verb+ 3 + \\
	 source\_id & \verb+ activitynet~v_-1IBHYS3L-Y + \\
	 split & \verb+ train + \\
	 split\_type & \verb+ indomain + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Complete the description with an appropriate ending:
First, {{ ctx_a.lower() }} Then, {{ ctx_b.lower() }} ...

(a) {{ answer_choices[0] }}

(b) {{ answer_choices[1] }}

(c) {{ answer_choices[2] }}

(d) {{ answer_choices[3] }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label | int()] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{endings | join(" ||| ")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
What is the topic of the sentence: {{ctx}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{activity_label}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Complete the sentence: {{ctx}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label | int()]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{endings | join(" ||| ")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ctx}} {{endings[label | int()]}}
Can you identify the topic of the paragraph?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{activity_label}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set prompts = [
'Can you pick the correct ending for the sentence: ',
'The task is to generate the ending for the sentence: ',
'How does this sentence end? ',
'From the list of endings described below, what ending makes the most sense for the sentence ',]
%}
{{prompts | choice}}
{{ctx}}

(a)  {{answer_choices[0]}}

(b)  {{answer_choices[1]}}

(c)  {{answer_choices[2]}}

(d)  {{answer_choices[3]}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices [label | int()]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{endings | join(" ||| ") }}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set instance = [0, 1, 2, 3] | choice %}
Consider the following description: {{ ctx_a }}
Is the following an appropriate continuation?
{{ ctx_b }} {{ endings[instance] }}
Yes or No?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label  == instance | string() %}
{{answer_choices[0]}}
{% else %} 
{{answer_choices[1]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
How does this sentence end?
{{ctx}}

(a)  {{answer_choices[0]}}

(b)  {{answer_choices[1]}}

(c)  {{answer_choices[2]}}

(d)  {{answer_choices[3]}}

Hint: the topic of the sentence is {{activity_label}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices [label | int()]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
{{endings | join("|||")}}
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
How would you start the sentence:
{{endings[label | int()]}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ctx}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set instance = [0, 1, 2, 3] | choice %}
Consider the following text: {{ ctx_b }} {{ endings[instance] }}
Is it an appropriate continuation of the following text: 
{{ ctx_a }} ?
Yes or No?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label  == instance | string() %}
{{answer_choices[0]}}
{% else %} 
{{answer_choices[1]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Yes ||| No
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{ ctx }}...
How does the description likely end?

Ending 1: {{ endings[0] }}

Ending 2: {{ endings[1] }}

Ending 3: {{ endings[2] }}

Ending 4: {{ endings[3] }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label | int()] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Ending 1 ||| Ending 2 ||| Ending 3 ||| Ending 4
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
If a description of a situation begins like this: {{ ctx }}... Then how
does it continue? 

Ending 1: {{ endings[0] }}

Ending 2: {{ endings[1] }}

Ending 3: {{ endings[2] }}

Ending 4: {{ endings[3] }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label | int()] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Ending 1 ||| Ending 2 ||| Ending 3 ||| Ending 4
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Structure To Text }
\subsubsection{common\_gen}
\noindent Dataset from \citet{lin-etal-2020-commongen}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 concept\_set\_idx & \verb+ 0 + \\
	 concepts & \verb+ ['ski', 'mountain', 'skier'] + \\
	 target & \verb+ Skier skis down the mountain + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Ignoring the order of the concepts: {{ concepts | join(", ") }}; 
Generate a sentence with all the concepts :
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Put the concepts together to form a sentence: {{ concepts | join(", ") }}.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Construct a sentence with the word {{ concepts | choice }}. 

Hint: Use {{concepts | join(", ")}} to restrict the output sentence.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set seq = [ 
'From the concepts mentioned below, generate a sentence:', 
'Convert the concepts to a sentence:', 
'Given the list of concepts, write a sentence:'
] %} 
{{ seq | choice }}
{{ concepts | join(", ") }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
What are the topics in the sentence: {{target}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ concepts | join(", ") }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
We have the sentence: {{target}}; 
Extract all the key concepts:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ concepts | join(", ") }}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Can you write a sentence about the topic {{concepts | choice}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Humans can easily string together abstract concepts to form a coherent sentence. 
For example, with the concepts {{ concepts | join(", ") }}, a simple sentence can be
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Given the list of concepts: {{ concepts | join(", ") }}; 
Generate a sentence with all the concepts :
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{wiki\_bio}
\noindent Dataset from \citet{DBLP:journals/corr/LebretGA16}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 input\_text & \verb+ {'table': {'column_header': ['name', 'nationality'... + \\
	 target\_text & \verb+ walter extra is a german award-winning aerobatic p... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Facts:
{% for n in range (input_text["table"]["column_header"]|length) %}
{% if input_text["table"]["column_header"][n] != "article_title" %}
- {{input_text["table"]["column_header"][n].replace("_"," ") }}: {{input_text["table"]["content"][n] }}
{% endif %}
{% endfor %}
Based on these bullet points, write a short biography describing the life of {{input_text["context"]}}.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{target_text}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Read the bio below and try to give details on {{input_text["context"]}}'s: 
{% for n in range (input_text["table"]["column_header"]|length) %} {% if input_text["table"]["column_header"][n] != "article_title" %}
- {{ input_text["table"]["column_header"][n].replace("_"," ") }} 
{% endif %} {% endfor %}

Bio: {{target_text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for n in range (input_text["table"]["column_header"]|length) %}
{% if input_text["table"]["column_header"][n] != "article_title" %}
- {{ input_text["table"]["column_header"][n].replace("_"," ") }} is {{ input_text["table"]["content"][n] }}
{% endif %}
{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
What type of details about {{input_text["context"]}} can be gathered from the following bio?

Bio: {{target_text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for n in range (input_text["table"]["column_header"]|length) %}
{% if input_text["table"]["column_header"][n] != "article_title" %}
- {{ input_text["table"]["column_header"][n].replace("_"," ") }} 
{% endif %}
{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% for n in range (input_text["table"]["column_header"]|length) %}
{% if input_text["table"]["column_header"][n] != "article_title" and input_text["table"]["column_header"][n] !="name" %}
- {{ input_text["table"]["column_header"][n].replace("_"," ") }} is {{ input_text["table"]["content"][n] }}
{% endif %}
{% endfor %}

Given the details above, guess who could this information be about.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{input_text["context"]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
What key details about {{input_text["context"]}} can be extracted from the following bio?

Bio: {{target_text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% for n in range (input_text["table"]["column_header"]|length) %}
{% if input_text["table"]["column_header"][n] != "article_title" %}
- {{ input_text["table"]["column_header"][n].replace("_"," ") }} is {{ input_text["table"]["content"][n] }}
{% endif %}
{% endfor %}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Summarization }
\subsubsection{cnn\_dailymail 3.0.0}
\noindent Dataset from \citet{DBLP:journals/corr/SeeLM17}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 article & \verb+ It's official: U.S. President Barack Obama wants l... + \\
	 highlights & \verb+ Syrian official: Obama climbed to the top of the t... + \\
	 id & \verb+ 0001d1afc246a7964130f43ae940af6bc6c57f01 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Can you write an outline of the following article in a few points?

Article: {{article}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{highlights}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Summarise the article:

{{article}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{highlights}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
In 2 or 3 sentences, what are the main points one should remember from this news article?

Article: {{article}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{highlights}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Could you please generate a TLDR (Too Long Didn't Read) summary of the following news article?

Article: {{article}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{highlights}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Condense the article down to the essentials to present it in the form of short cards in mobile news apps:

{{article}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{highlights}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Generate a story from key plot points:

{{highlights}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{article}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Sum the following article in brief: {{article}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{highlights}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Extract key points from the article based on which the stock market could react:

{{article}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{highlights}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
What details would you include in a storyline to make it more engaging and informative?

{{highlights}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{article}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{gigaword}
\noindent Dataset from \citet{graff2003english}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 document & \verb+ australia 's current account deficit shrunk by a r... + \\
	 summary & \verb+ australian current account deficit narrows sharply + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{document}}

===

Generate a title for this article:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Title: {{summary}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{document}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Make a title for this article: {{document}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
First sentence of the article: {{document}}

Title:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{radford2019language}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{document}}

TL;DR:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{document}}

===

Given the above sentence, write its title:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Write a title for this sentence: {{document}} 

Title:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{document}} In a nutshell,
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Title: {{summary}}

===

Write an article with the given title:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{document}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{multi\_news}
\noindent Dataset from \citet{alex2019multinews}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 document & \verb+ National Archives 
  
 Yes, it’s that time again, ... + \\
	 summary & \verb+ – The unemployment rate dropped to 8.2% last month... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set docs = document.split("3ed2dface8203c4c9dfb1a5dc58e41e0||") | reject("equalto", "") | list %}
What are the key points across these news articles:
{% for doc in docs %}

Article: {{doc}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary[2:]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set docs = document.split("3ed2dface8203c4c9dfb1a5dc58e41e0||") | reject("equalto", "") | list %}
Synthesize these documents into a single one:
{% for doc in docs %}

- {{doc}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary[2:]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set docs = document.split("3ed2dface8203c4c9dfb1a5dc58e41e0||") | reject("equalto", "") | list %}
I want to edit the following articles into a more concise summary:
{% for doc in docs %}

Article: {{doc}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary[2:]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set docs = document.split("3ed2dface8203c4c9dfb1a5dc58e41e0||") | reject("equalto", "") | list %}
Write a summary of the following articles:
{% for doc in docs %}

Document: {{doc}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary[2:]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set docs = document.split("3ed2dface8203c4c9dfb1a5dc58e41e0||") | reject("equalto", "") | list%}
Write an expanded news article with plausible details from the following summary:
{{summary[2:]}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{docs | choice}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set docs = document.split("3ed2dface8203c4c9dfb1a5dc58e41e0||") | reject("equalto", "") | list %}
I'm trying to distill these articles down into one:
{% for doc in docs %}

Article: {{doc}}
{% endfor %}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary[2:]}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{samsum}
\noindent Dataset from \citet{gliwa2019samsum}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 dialogue & \verb+ Amanda: I baked  cookies. Do you want some?
Jerry... + \\
	 id & \verb+ 13818513 + \\
	 summary & \verb+ Amanda baked cookies and will bring Jerry some tom... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Summarize this dialogue: {{dialogue}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{dialogue}}
Given the above dialogue, write a summary.
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Summarize: {{dialogue}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{dialogue}}
To sum up this dialog:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Generate a summary for this dialogue:
{{dialogue}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Write a dialogue that matches this summary: {{summary}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{dialogue}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Sum up the following dialogue: 
{{dialogue}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{xsum}
\noindent Dataset from \citet{Narayan2018DontGM}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 document & \verb+ Recent reports have linked some France-based playe... + \\
	 id & \verb+ 29750031 + \\
	 summary & \verb+ New Welsh Rugby Union chairman Gareth Davies belie... + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{document}}

===

Write a summary of the text above :
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Article: {{document}}

Summary:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{wikidotgpt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{document}}
How would you rephrase that in a few words?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{wikidotgpt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
My college roommate asked me what this article means:

{{document}}

So I recapped it in layman's terms:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{wikidotgpt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{document}}
This boils down to the simple idea that
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Summarize: {{document}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Summarize this document: {{document}}
Summary:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{document}}

===

Given the above document, write one sentence to summarize:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
First, please read the article below.

{{document}}

Now, can you write me an extremely short abstract for it?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{radford2019language}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{document}}

TL;DR:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{summary}}
\end{minted}
\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Topic Classification }
\subsubsection{ag\_news}
\noindent Dataset from \citet{Zhang2015CharacterlevelCN}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 text & \verb+ Wall St. Bears Claw Back Into the Black (Reuters) ... + \\
	 label & \verb+ 2 + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
What label best describes this news article?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
World politics ||| Sports ||| Business ||| Science and technology
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Is this a piece of news regarding {{"world politics, sports, business, or science and technology"}}?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
World politics ||| Sports ||| Business ||| Science and technology
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Would you recommend the following article to a {{"politician"}}, an {{"athlete"}}, a {{"business executive"}}, or a {{"scientist"}}?

{{ text }}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Politician ||| Athlete ||| Business executive ||| Scientist
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} 

Which of the following sections of a newspaper would this article likely appear in? {{"World News"}}, {{"Sports"}}, {{"Business"}}, or {{"Science and Technology"}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
World News ||| Sports ||| Business ||| Science and Technology
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} 

Which section of a newspaper would this article likely appear in?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
World News ||| Sports ||| Business ||| Science and Technology
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} 
Is this a piece of news regarding {{"world politics, sports, business, or science and technology"}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
World politics ||| Sports ||| Business ||| Science and technology
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}} 
What label best describes this news article?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
World politics ||| Sports ||| Business ||| Science and technology
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{dbpedia\_14}
\noindent Dataset from \citet{lehmann2015dbpedia}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 content & \verb+  Abbott of Farnham E D Abbott Limited was a Britis... + \\
	 label & \verb+ 0 + \\
	 title & \verb+ E. D. Abbott Ltd + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{content}} Given a list of categories: {{"company, educational institution, artist, athlete, office holder, mean of transportation, building, natural place, village, animal, plant, album, film or written work"}}, what category does the paragraph belong to?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Company ||| Educational Institution ||| Artist ||| Athlete ||| Office Holder ||| Mean Of Transportation ||| Building ||| Natural Place ||| Village ||| Animal ||| Plant ||| Album ||| Film ||| Written Work
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Pick one category for the following text. The options are - {{"company, educational institution, artist, athlete, office holder, mean of transportation, building, natural place, village, animal, plant, album, film or written work"}}. {{title}} - {{content}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Company ||| Educational Institution ||| Artist ||| Athlete ||| Office Holder ||| Mean Of Transportation ||| Building ||| Natural Place ||| Village ||| Animal ||| Plant ||| Album ||| Film ||| Written Work
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{title}} - {{content}} Given a choice of categories {{"company, educational institution, artist, athlete, office holder, mean of transportation, building, natural place, village, animal, plant, album, film or written work"}}, the text refers to which one?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Company ||| Educational Institution ||| Artist ||| Athlete ||| Office Holder ||| Mean Of Transportation ||| Building ||| Natural Place ||| Village ||| Animal ||| Plant ||| Album ||| Film ||| Written Work
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
"{{title}}", given a list of categories: {{"company, educational institution, artist, athlete, office holder, mean of transportation, building, natural place, village, animal, plant, album, film or written work"}}, what category does the title belong to?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Company ||| Educational Institution ||| Artist ||| Athlete ||| Office Holder ||| Mean Of Transportation ||| Building ||| Natural Place ||| Village ||| Animal ||| Plant ||| Album ||| Film ||| Written Work
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsubsection{trec}
\noindent Dataset from \citet{li-roth-2002-learning}.
Used in training.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 label-coarse & \verb+ 0 + \\
	 label-fine & \verb+ 0 + \\
	 text & \verb+ How did serfdom develop in and then leave Russia ? + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Categories: {{', '.join(answer_choices)}}

What category best describes: {{text}} 
Answer:
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_coarse] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Description ||| Entity ||| Abbreviation ||| Person ||| Quantity ||| Location
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set label_mapping = {21:0, 18:1, 24:2, 11:3, 14:4} %}
{% if label_coarse == 5 %}
Is this question asking for {{', '.join(answer_choices)}}?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
city ||| country ||| mountain ||| state ||| other location
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set label_mapping = {39:0, 13:1, 8:2, 40:3, 25:4, 43:5, 27:6, 38:7, 35:8, 41:9, 32:10, 45:11, 14:12} %}
{% if label_coarse == 4 %}
{{text}}

Is this question asking for {{', '.join(answer_choices)}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
code ||| count ||| date ||| distance ||| price ||| order ||| period of time ||| percentage ||| speed ||| temperature ||| size ||| weight ||| other number
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set label_mapping = {2:0, 22:1, 19:2, 1:3, 46:3, 23:4, 10:5, 17:6, 33:7, 37:8, 15:9, 30:10, 26:11, 16:12, 28:13, 42:14, 31:15, 20:16, 44:17, 36:18, 14:19} %}
{% if label_coarse == 1 %}
Is this question asking for {{', '.join(answer_choices)}}?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
an animal ||| an organ of the body ||| a color ||| creative piece ||| currency ||| disease or medicine ||| event ||| food ||| musical instrument ||| language ||| letter ||| plant ||| product ||| religion ||| sport ||| substance ||| symbol ||| technique ||| term ||| vehicle ||| word ||| other entity
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set label_mapping = {39:0, 13:1, 8:2, 40:3, 25:4, 43:5, 27:6, 38:7, 35:8, 41:9, 32:10, 45:11, 14:12} %}
{% if label_coarse == 4 %}
Is this question asking for {{', '.join(answer_choices)}}?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
code ||| count ||| date ||| distance ||| price ||| order ||| period of time ||| percentage ||| speed ||| temperature ||| size ||| weight ||| other number
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Question: {{text}}

Descriptors: {{', '.join(answer_choices)}}

Best Descriptor?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label_coarse]}}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Description ||| Entity ||| Abbreviation ||| Person ||| Quantity ||| Location
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}}

What is this question asking for?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label_fine] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Manner ||| Creative Piece ||| Animal ||| Expression abbreviated ||| Individual ||| Group ||| Title ||| Defintion ||| Date ||| Reason ||| Event ||| State ||| Description ||| Count ||| Other ||| Letter ||| Religion ||| Food ||| Country ||| Color ||| Term ||| City ||| Organ of the body ||| Disease or medicine ||| Mountain ||| Price ||| Product ||| Period ||| Substance ||| Sport ||| Plant ||| Technique ||| Size ||| Instrument ||| Abbreviation ||| Speed ||| Word ||| Language ||| Percentage ||| Code ||| Distance ||| Temperature ||| Symbol ||| Order ||| Vehicle ||| Weight ||| Currency
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set label_mapping = {21:0, 18:1, 24:2, 11:3, 14:4} %}
{% if label_coarse == 5 %}
{{text}}

Is this question asking for {{', '.join(answer_choices)}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
city ||| country ||| mountain ||| state ||| other location
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Which category best describes the following question: {{text}} 

Choose from the following list: 
{{', '.join(answer_choices)}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_coarse] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Description ||| Entity ||| Abbreviation ||| Person ||| Quantity ||| Location
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set label_mapping={0:2, 7:1,  12:0, 9:3} %}
{% if label_coarse == 0 %}
Is this question asking for {{', '.join(answer_choices)}}?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
definition ||| description ||| manner of action ||| reason
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{text}}

Is this asking about {{(', ').join(answer_choices)}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_coarse] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Description ||| Entity ||| Abbreviation ||| Person ||| Quantity ||| Location
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set label_mapping={34:0, 3:1} %} 
{% if label_coarse == 2 %}
Is this question asking for an {{', '.join(answer_choices)}}?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{answer_choices[label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
abbreviation ||| expression abbreviated
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set label_mapping = {34:0, 3:1} %} 
{% if label_coarse == 2 %}
{{text}}

Is this question asking for an {{', '.join(answer_choices)}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
abbreviation ||| expression abbreviated
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Is the following question asking about {{', '.join(answer_choices)}}?

{{text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_coarse] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Description ||| Entity ||| Abbreviation ||| Person ||| Quantity ||| Location
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set label_mapping = {5:0, 4:1, 6:2, 12:3} %}
{% if label_coarse == 3 %}
Is this question asking for {{', '.join(answer_choices)}}?
{{text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
group ||| individual ||| title ||| description
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
What is this question asking for?

{{text}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices[label_fine] }}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
Manner ||| Creative Piece ||| Animal ||| Expression abbreviated ||| Individual ||| Group ||| Title ||| Defintion ||| Date ||| Reason ||| Event ||| State ||| Description ||| Count ||| Other ||| Letter ||| Religion ||| Food ||| Country ||| Color ||| Term ||| City ||| Organ of the body ||| Disease or medicine ||| Mountain ||| Price ||| Product ||| Period ||| Substance ||| Sport ||| Plant ||| Technique ||| Size ||| Instrument ||| Abbreviation ||| Speed ||| Word ||| Language ||| Percentage ||| Code ||| Distance ||| Temperature ||| Symbol ||| Order ||| Vehicle ||| Weight ||| Currency
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set label_mapping = {5:0, 4:1, 6:2, 12:3} %}
{% if label_coarse == 3 %}
{{text}}

Is this question asking for {{', '.join(answer_choices)}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
group ||| individual ||| title ||| description
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small \nooriginal}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{% set label_mapping={0:2, 7:1,  12:0, 9:3} %}
{% if label_coarse == 0 %}
{{text}}

Is this question asking for {{', '.join(answer_choices)}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{{ answer_choices [label_mapping[label_fine]] }}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
definition ||| description ||| manner of action ||| reason
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\subsection{Word Sense Disambiguation }
\subsubsection{super\_glue wic}
\noindent Dataset from \citet{DBLP:journals/corr/abs-1808-09121}.
Used in evaluation.
\paragraph{Data Example}\mbox{}\\

\begin{table}[h]
\small
\begin{tabular}{ll}
\toprule 
Key & Value\\
\midrule 
	 end1 & \verb+ 36 + \\
	 end2 & \verb+ 32 + \\
	 idx & \verb+ 0 + \\
	 label & \verb+ 0 + \\
	 sentence1 & \verb+ Do you want to come over to my place later? + \\
	 sentence2 & \verb+ A political system with no place for the less prom... + \\
	 start1 & \verb+ 31 + \\
	 start2 & \verb+ 27 + \\
	 word & \verb+ place + \\
\bottomrule
\end{tabular}
\end{table}
\paragraph{Prompts}\mbox{}\\

\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Does the word "{{word}}" have the same meaning in these two sentences? Yes, No?
{{sentence1}}
{{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1%}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Does the word "{{word}}" have the same meaning in these two sentences?
{{sentence1}}
{{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1%}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Homework

Decide whether the word "{{word}}" is used with the same meaning in the two following sentences. Answer by yes or no.
{{sentence1}}
{{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1%}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Sentence A: {{sentence1}}
Sentence B: {{sentence2}}

"{{word}}" has a similar meaning in sentences A and B. True or False?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1%}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
False ||| True
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{sentence1}}
{{sentence2}}
Question: Is the word '{{word}}' used in the same sense in the two sentences above?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1%}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}

Determine whether the word "{{word}}" is used in the same sense in both sentences. Yes or no?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1%}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
Determine if the word '{{word}}' is used in the same way in the two sentences below. 
{{sentence1}}
{{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1%}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{gpt3}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{sentence1}}
{{sentence2}}
Question: Is the word '{{word}}' used in the same sense in the two sentences above? Yes, No?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1%}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
The word "{{word}}" has multiple meanings. Does it have the same meaning in sentences 1 and 2? Yes or no?

Sentence 1: {{sentence1}}
Sentence 2: {{sentence2}}
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1%}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}
\noindent{\small Prompt from \cite{DBLP:journals/corr/abs-2105-11447}}
\inputtemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bga]{django}
{{sentence1}}
{{sentence2}}
Similar sense of {{word}}?
\end{minted}
\vspace*{-0.2cm}

\targettemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small,bgcolor=bg]{django}
{% if label != -1%}
{{answer_choices[label]}}
{% endif %}
\end{minted}
\choicestemplate
\begin{minted}[breaklines, tabsize=2,breaksymbolleft=, fontsize=\small, bgcolor=bgb]{django}
No ||| Yes
\end{minted}
\vspace*{-0.3cm}

\textcolor[RGB]{220,220,220}{\rule{\linewidth}{0.2pt}}

